The Spitzer c2d Legacy Results: Star Formation Rates and Efficiencies; Evolution and Lifetimes

(Abridged) The c2d Spitzer Legacy project obtained images and photometry with both IRAC and MIPS instruments for five large, nearby molecular clouds. This paper combines information drawn from studies of individual clouds into a combined and updated statistical analysis of star formation rates and efficiencies, numbers and lifetimes for SED classes, and clustering properties. Current star formation efficiencies range from 3% to 6%. Taken together, the five clouds are producing about 260 solar masses of stars per Myr. The star formation surface density is more than an order of magnitude larger than would be predicted from the Kennicutt relation used in extragalactic studies. Measured against the dense gas probed by the maps of dust continuum emission, the efficiencies are much higher, and the current stock of dense cores would be exhausted in 1.8 Myr on average. The derived lifetime for the Class I phase is 0.44 to 0.54 Myr, considerably longer than some estimates. Similarly, the lifetime for the Class 0 SED class, 0.10 to 0.16 Myr, is longer than early estimates. The great majority (90%) of young stars lie within loose clusters with at least 35 members and a stellar density of 1 solar mass per cubic pc. Accretion at the sound speed from an isothermal sphere over the lifetime derived for the Class I phase could build a star of about 0.25 solar masses, given an efficiency of 0.3. Our data confirm and aggravate the "luminosity problem" for protostars. Our results strongly suggest that accretion is time variable, with prolonged periods of very low accretion. Based on a very simple model and this sample of sources, half the mass of a star would be accreted during only 7% of the Class I lifetime, as represented by the eight most luminous objects.

==> tab10.tex <==
\begin{landscape}
\begin{deluxetable}{rcccccccc}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\tablecaption{\label{tabysolist3}$3.4-100$ \um\ Flux Densities, in mJy, of YSOs in the c2d Clouds}
\tablehead{
                & \colhead{\emph{L}} & \colhead{\emph{M}} & \colhead{\emph{ISO}} & \colhead{\emph{IRAS}}    & \colhead{\emph{ISO}}    & \colhead{\emph{IRAS}}    & \colhead{\emph{IRAS}}    & \colhead{\emph{IRAS}}  \\
\colhead{Index} & \colhead{3.4 \um} & \colhead{5.0 \um} & \colhead{6.7 \um}       & \colhead{12 \um} & \colhead{14.3 \um} & \colhead{25 \um} & \colhead{60 \um} & \colhead{100 \um}}
\startdata
   1 &     3500 $\pm$      32 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
   2 &      540 $\pm$      5.0 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
   3 &    12000 $\pm$     230 &   21000 $\pm$ 590 &             ... &    44000 $\pm$    2200 &             ... &   100000 $\pm$    5100 &   110000 $\pm$   11000 &   100000 $\pm$   10000 \\
   4 &             ... &             ... &             ... &      110 $\pm$      20 &             ... &      900 $\pm$     180 &     3600 $\pm$     730 &     5100 $\pm$    1100 \\
   5 &       58 $\pm$      6.5 &             ... &             ... &             ... &             ... &       20 $\pm$      20 &             ... &             ... \\
   6 &       26 $\pm$      5.6 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
   7 &      290 $\pm$      2.7 &             ... &             ... &      520 $\pm$      50 &             ... &      500 $\pm$      50 &      460 $\pm$      90 &     4300 $\pm$    1100 \\
   8 &             ... &             ... &       6.7 $\pm$     0.60 &             ... &       6.0 $\pm$      1.2 &             ... &             ... &             ... \\
   9 &             ... &             ... &      790 $\pm$      26 &      700 $\pm$      70 &     1200 $\pm$      25 &     4400 $\pm$     220 &    11000 $\pm$     530 &    18000 $\pm$    5400 \\
  10 &      840 $\pm$      7.7 &             ... &             ... &      380 $\pm$      40 &             ... &      360 $\pm$      30 &             ... &             ... \\
  11 &      140 $\pm$      11 &             ... &      100 $\pm$      1.6 &      320 $\pm$      30 &      160 $\pm$      1.8 &      690 $\pm$      70 &      980 $\pm$     150 &             ... \\
  12 &             ... &             ... &      210 $\pm$      3.6 &             ... &      170 $\pm$      3.2 &             ... &             ... &             ... \\
  13 &      110 $\pm$      11 &             ... &             ... &             ... &             ... &      130 $\pm$      20 &      260 $\pm$      60 &             ... \\
  14 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  15 &             ... &             ... &             ... &      400 $\pm$      60 &             ... &      110 $\pm$      20 &             ... &             ... \\
  16 &      120 $\pm$      8.7 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  17 &       75 $\pm$      8.3 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  18 &       66 $\pm$      8.5 &             ... &             ... &      120 $\pm$      40 &             ... &       40 $\pm$      10 &             ... &             ... \\
  19 &      540 $\pm$      30 &             ... &             ... &      440 $\pm$      70 &             ... &      390 $\pm$      80 &      310 $\pm$      90 &             ... \\
  20 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  21 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  22 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  23 &       60 $\pm$      6.6 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  24 &      590 $\pm$      33 &             ... &             ... &      610 $\pm$      60 &             ... &      760 $\pm$      80 &      680 $\pm$     100 &             ... \\
  25 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  26 &      140 $\pm$      8.9 &             ... &             ... &      110 $\pm$      30 &             ... &      110 $\pm$      20 &             ... &             ... \\
  27 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  28 &             ... &             ... &             ... &             ... &             ... &      300 $\pm$      30 &     2600 $\pm$     260 &             ... \\
  29 &             ... &             ... &             ... &      550 $\pm$      55 &             ... &      760 $\pm$      76 &      690 $\pm$      69 &             ... \\
  30 &             ... &             ... &             ... &      550 $\pm$      55 &             ... &      760 $\pm$      76 &      690 $\pm$      69 &             ... \\
  31 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  32 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  33 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  34 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  35 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  36 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  37 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  38 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  39 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  40 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  41 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  42 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  43 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  44 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  45 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  46 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  47 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  48 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  49 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  50 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  51 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  52 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  53 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  54 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  55 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  56 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  57 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  58 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  59 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  60 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  61 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  62 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  63 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  64 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  65 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  66 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  67 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  68 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  69 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  70 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  71 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  72 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  73 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  74 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  75 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  76 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  77 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  78 &             ... &             ... &             ... &             ... &             ... &             ... &     1700 $\pm$     220 &             ... \\
  79 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  80 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  81 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  82 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  83 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  84 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  85 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  86 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  87 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  88 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  89 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  90 &             ... &             ... &             ... &      290 $\pm$      29 &             ... &             ... &             ... &    22000 $\pm$    2200 \\
  91 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  92 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  93 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  94 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  95 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  96 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  97 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  98 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  99 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 100 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 101 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 102 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 103 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 104 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 105 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 106 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 107 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 108 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 109 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 110 &             ... &             ... &             ... &     2600 $\pm$     260 &             ... &     1400 $\pm$     140 &      480 $\pm$      48 &     4500 $\pm$     450 \\
 111 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 112 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 113 &             ... &             ... &             ... &      290 $\pm$      29 &             ... &      780 $\pm$      78 &     1200 $\pm$     120 &     4600 $\pm$     460 \\
 114 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 115 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 116 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 117 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 118 &             ... &             ... &             ... &      970 $\pm$      97 &             ... &      400 $\pm$      40 &      450 $\pm$      45 &     4600 $\pm$     460 \\
 119 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 120 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 121 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 122 &             ... &             ... &             ... &             ... &             ... &      650 $\pm$      78 &    14000 $\pm$    1700 &             ... \\
 123 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 124 &             ... &             ... &             ... &      610 $\pm$      49 &             ... &     5200 $\pm$     370 &    25000 $\pm$    5500 &   170000 $\pm$   24000 \\
 125 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 126 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 127 &             ... &             ... &             ... &             ... &             ... &      550 $\pm$      76 &     4200 $\pm$     380 &     7000 $\pm$     700 \\
 128 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 129 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 130 &             ... &             ... &             ... &             ... &             ... &     3400 $\pm$     200 &    47000 $\pm$    5200 &    94000 $\pm$   22000 \\
 131 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 132 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 133 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 134 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 135 &             ... &             ... &             ... &             ... &             ... &             ... &      690 $\pm$      55 &             ... \\
 136 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 137 &             ... &             ... &             ... &      420 $\pm$      63 &             ... &     1800 $\pm$     260 &     4400 $\pm$     440 &     7400 $\pm$    1600 \\
 138 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 139 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 140 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 141 &             ... &             ... &             ... &      560 $\pm$      39 &             ... &    16000 $\pm$    1200 &             ... &             ... \\
 142 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 143 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 144 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 145 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 146 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 147 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 148 &             ... &             ... &             ... &     1100 $\pm$      77 &             ... &     3000 $\pm$     210 &             ... &             ... \\
 149 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 150 &             ... &             ... &             ... &       20 $\pm$      4.0 &             ... &      150 $\pm$      30 &     1400 $\pm$     130 &     6000 $\pm$    1200 \\
 151 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 152 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 153 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 154 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 155 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 156 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 157 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 158 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 159 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 160 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 161 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 162 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 163 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 164 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 165 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 166 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 167 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 168 &             ... &             ... &             ... &             ... &             ... &             ... &   150000 $\pm$   20000 &   360000 $\pm$   51000 \\
 169 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 170 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 171 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 172 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 173 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 174 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 175 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 176 &             ... &             ... &             ... &             ... &             ... &             ... &    33000 $\pm$    4300 &    78000 $\pm$   11000 \\
 177 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 178 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 179 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 180 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 181 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 182 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 183 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 184 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 185 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 186 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 187 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 188 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 189 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 190 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 191 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 192 &             ... &             ... &             ... &    11000 $\pm$     560 &             ... &    43000 $\pm$    2100 &   230000 $\pm$   28000 &             ... \\
 193 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 194 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 195 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 196 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 197 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 198 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 199 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 200 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 201 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 202 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 203 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 204 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 205 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 206 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 207 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 208 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 209 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 210 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 211 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 212 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 213 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 214 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 215 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 216 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 217 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 218 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 219 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 220 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 221 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 222 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 223 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 224 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 225 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 226 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 227 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 228 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 229 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 230 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 231 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 232 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 233 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 234 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 235 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 236 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 237 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 238 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 239 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 240 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 241 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 242 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 243 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 244 &             ... &             ... &             ... &             ... &             ... &             ... &     1100 $\pm$      96 &             ... \\
 245 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 246 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 247 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 248 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 249 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 250 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 251 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 252 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 253 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 254 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 255 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 256 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 257 &             ... &             ... &             ... &             ... &             ... &             ... &     1900 $\pm$     150 &             ... \\
 258 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 259 &             ... &             ... &             ... &             ... &             ... &     1700 $\pm$     140 &     7500 $\pm$     730 &     8200 $\pm$    1100 \\
 260 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 261 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 262 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 263 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 264 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 265 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 266 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 267 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 268 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 269 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 270 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 271 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 272 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 273 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 274 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 275 &             ... &             ... &             ... &             ... &             ... &             ... &     2300 $\pm$     210 &    14000 $\pm$    1500 \\
 276 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 277 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 278 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 279 &             ... &             ... &             ... &             ... &             ... &             ... &     1600 $\pm$     130 &     9100 $\pm$    1300 \\
 280 &             ... &             ... &             ... &             ... &             ... &             ... &     1400 $\pm$     120 &             ... \\
 281 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 282 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 283 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 284 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 285 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 286 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 287 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 288 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 289 &             ... &             ... &             ... &     1600 $\pm$      94 &             ... &     3700 $\pm$     220 &     5300 $\pm$     470 &             ... \\
 290 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 291 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 292 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 293 &             ... &             ... &             ... &             ... &             ... &     1400 $\pm$     140 &             ... &    35000 $\pm$    5300 \\
 294 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 295 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 296 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 297 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 298 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 299 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 300 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 301 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 302 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 303 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 304 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 305 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 306 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 307 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 308 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 309 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 310 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 311 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 312 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 313 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 314 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 315 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 316 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 317 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 318 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 319 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 320 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 321 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 322 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 323 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 324 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 325 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 326 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 327 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 328 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 329 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 330 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 331 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 332 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 333 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 334 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 335 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 336 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 337 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 338 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 339 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 340 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 341 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 342 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 343 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 344 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 345 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 346 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 347 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 348 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 349 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 350 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 351 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 352 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 353 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 354 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 355 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 356 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 357 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 358 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 359 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 360 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 361 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 362 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 363 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 364 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 365 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 366 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 367 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 368 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 369 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 370 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 371 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 372 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 373 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 374 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 375 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 376 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 377 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 378 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 379 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 380 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 381 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 382 &             ... &             ... &             ... &             ... &             ... &     1500 $\pm$     150 &             ... &             ... \\
 383 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 384 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 385 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 386 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 387 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 388 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 389 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 390 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 391 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 392 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 393 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 394 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 395 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 396 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 397 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 398 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 399 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 400 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 401 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 402 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 403 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 404 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 405 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 406 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 407 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 408 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 409 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 410 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 411 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 412 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 413 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 414 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 415 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 416 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 417 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 418 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 419 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 420 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 421 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 422 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 423 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 424 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 425 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 426 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 427 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 428 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 429 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 430 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 431 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 432 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 433 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 434 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 435 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 436 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 437 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 438 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 439 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 440 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 441 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 442 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 443 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 444 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 445 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 446 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 447 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 448 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 449 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 450 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 451 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 452 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 453 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 454 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 455 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 456 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 457 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 458 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 459 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 460 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 461 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 462 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 463 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 464 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 465 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 466 &             ... &             ... &             ... &      510 $\pm$      46 &             ... &     2100 $\pm$     150 &             ... &             ... \\
 467 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 468 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 469 &             ... &             ... &             ... &       38 $\pm$      3.4 &             ... &      160 $\pm$      11 &             ... &             ... \\
 470 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 471 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 472 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 473 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 474 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 475 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 476 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 477 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 478 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 479 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 480 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 481 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 482 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 483 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 484 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 485 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 486 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 487 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 488 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 489 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 490 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 491 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 492 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 493 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 494 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 495 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 496 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 497 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 498 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 499 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 500 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 501 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 502 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 503 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 504 &             ... &             ... &             ... &             ... &             ... &      750 $\pm$      45 &     1200 $\pm$      85 &             ... \\
 505 &             ... &             ... &             ... &     1600 $\pm$      65 &             ... &     5200 $\pm$     210 &    16000 $\pm$     930 &    15000 $\pm$    1400 \\
 506 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 507 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 508 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 509 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 510 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 511 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 512 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 513 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 514 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 515 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 516 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 517 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 518 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 519 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 520 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 521 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 522 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 523 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 524 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 525 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 526 &             ... &             ... &             ... &             ... &             ... &      240 $\pm$      24 &      940 $\pm$     100 &             ... \\
 527 &             ... &             ... &             ... &             ... &             ... &       35 $\pm$      3.5 &      140 $\pm$      15 &             ... \\
 528 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 529 &             ... &             ... &             ... &             ... &             ... &      510 $\pm$      51 &     2000 $\pm$     220 &             ... \\
 530 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 531 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 532 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 533 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 534 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 535 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 536 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 537 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 538 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 539 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 540 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 541 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 542 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 543 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 544 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 545 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 546 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 547 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 548 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 549 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 550 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 551 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 552 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 553 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 554 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 555 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 556 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 557 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 558 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 559 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 560 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 561 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 562 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 563 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 564 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 565 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 566 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 567 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 568 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 569 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 570 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 571 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 572 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 573 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 574 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 575 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 576 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 577 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 578 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 579 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 580 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 581 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 582 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 583 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 584 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 585 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 586 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 587 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 588 &             ... &             ... &             ... &             ... &             ... &      750 $\pm$      67 &     2100 $\pm$     310 &             ... \\
 589 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 590 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 591 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 592 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 593 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 594 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 595 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 596 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 597 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 598 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 599 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 600 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 601 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 602 &             ... &             ... &             ... &     3300 $\pm$     160 &             ... &     6300 $\pm$     440 &     9300 $\pm$    1300 &             ... \\
 603 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 604 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 605 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 606 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 607 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 608 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 609 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 610 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 611 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 612 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 613 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 614 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 615 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 616 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 617 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 618 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 619 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 620 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 621 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 622 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 623 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 624 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 625 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 626 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 627 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 628 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 629 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 630 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 631 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 632 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 633 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 634 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 635 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 636 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 637 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 638 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 639 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 640 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 641 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 642 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 643 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 644 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 645 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 646 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 647 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 648 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 649 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 650 &             ... &             ... &             ... &             ... &             ... &      120 $\pm$      16 &     1600 $\pm$     200 &     7300 $\pm$    1100 \\
 651 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 652 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 653 &             ... &             ... &             ... &             ... &             ... &      400 $\pm$      52 &             ... &             ... \\
 654 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 655 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 656 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 657 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 658 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 659 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 660 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 661 &             ... &             ... &             ... &             ... &             ... &       19 $\pm$      2.5 &     1100 $\pm$     130 &     6500 $\pm$     980 \\
 662 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 663 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 664 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 665 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 666 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 667 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 668 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 669 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 670 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 671 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 672 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 673 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 674 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 675 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 676 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 677 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 678 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 679 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 680 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 681 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 682 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 683 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 684 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 685 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 686 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 687 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 688 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 689 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 690 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 691 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 692 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 693 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 694 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 695 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 696 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 697 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 698 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 699 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 700 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 701 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 702 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 703 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 704 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 705 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 706 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 707 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 708 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 709 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 710 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 711 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 712 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 713 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 714 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 715 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 716 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 717 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 718 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 719 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 720 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 721 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 722 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 723 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 724 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 725 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 726 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 727 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 728 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 729 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 730 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 731 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 732 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 733 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 734 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 735 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 736 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 737 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 738 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 739 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 740 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 741 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 742 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 743 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 744 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 745 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 746 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 747 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 748 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 749 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 750 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 751 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 752 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 753 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 754 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 755 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 756 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 757 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 758 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 759 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 760 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 761 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 762 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 763 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 764 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 765 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 766 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 767 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 768 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 769 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 770 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 771 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 772 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 773 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 774 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 775 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 776 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 777 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 778 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 779 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 780 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 781 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 782 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 783 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 784 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 785 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 786 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 787 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 788 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 789 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 790 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 791 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 792 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 793 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 794 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 795 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 796 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 797 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 798 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 799 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 800 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 801 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 802 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 803 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 804 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 805 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 806 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 807 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 808 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 809 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 810 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 811 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 812 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 813 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 814 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 815 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 816 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 817 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 818 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 819 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 820 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 821 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 822 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 823 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 824 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 825 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 826 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 827 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 828 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 829 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 830 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 831 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 832 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 833 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 834 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 835 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 836 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 837 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 838 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 839 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 840 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 841 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 842 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 843 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 844 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 845 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 846 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 847 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 848 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 849 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 850 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 851 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 852 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 853 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 854 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 855 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 856 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 857 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 858 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 859 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 860 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 861 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 862 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 863 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 864 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 865 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 866 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 867 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 868 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 869 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 870 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 871 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 872 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 873 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 874 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 875 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 876 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 877 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 878 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 879 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 880 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 881 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 882 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 883 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 884 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 885 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &   220000 $\pm$   48000 \\
 886 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 887 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 888 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 889 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 890 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 891 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 892 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 893 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 894 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 895 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 896 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 897 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 898 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 899 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 900 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 901 &             ... &             ... &             ... &     9900 $\pm$     990 &             ... &    68000 $\pm$    6800 &             ... &   350000 $\pm$   88000 \\
 902 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 903 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 904 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 905 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 906 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 907 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 908 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 909 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 910 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 911 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 912 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 913 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 914 &             ... &             ... &             ... &      280 $\pm$      28 &             ... &      500 $\pm$      50 &      940 $\pm$      94 &             ... \\
 915 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 916 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 917 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 918 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 919 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 920 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 921 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 922 &             ... &             ... &             ... &     1400 $\pm$     140 &             ... &     2400 $\pm$     240 &     3600 $\pm$     360 &             ... \\
 923 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 924 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 925 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 926 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 927 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 928 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 929 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 930 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 931 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 932 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 933 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 934 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 935 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 936 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 937 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 938 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 939 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 940 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 941 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 942 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 943 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 944 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 945 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 946 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 947 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 948 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 949 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 950 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 951 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 952 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 953 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 954 &             ... &             ... &             ... &             ... &             ... &             ... &     2900 $\pm$     380 &    16000 $\pm$    2800 \\
 955 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 956 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 957 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 958 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 959 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 960 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 961 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 962 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 963 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 964 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 965 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 966 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 967 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 968 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 969 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 970 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 971 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 972 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 973 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 974 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 975 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 976 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 977 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 978 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 979 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 980 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 981 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 982 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 983 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 984 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 985 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 986 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 987 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 988 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 989 &             ... &             ... &             ... &     1200 $\pm$      59 &             ... &     3700 $\pm$     220 &     9400 $\pm$     760 &             ... \\
 990 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 991 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 992 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 993 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 994 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 995 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 996 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 997 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 998 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 999 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1000 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1001 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1002 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1003 &             ... &             ... &             ... &     3600 $\pm$     180 &             ... &    15000 $\pm$    1200 &    66000 $\pm$    9300 &   130000 $\pm$   25000 \\
1004 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1005 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1006 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1007 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1008 &             ... &             ... &             ... &             ... &             ... &     1800 $\pm$     130 &   250000 $\pm$   31000 &  1000000 $\pm$   93000 \\
1009 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1010 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1011 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1012 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1013 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1014 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1015 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1016 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1017 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1018 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1019 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1020 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1021 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1022 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1023 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1024 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
\enddata \\
\end{deluxetable}
\end{landscape}


==> tab11.tex <==
\begin{landscape}
\begin{deluxetable}{rccccccc}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\tablecaption{\label{tabysolist3}$160-1300$ \um\ Flux Densities, in mJy, of YSOs in the c2d Clouds}
\tablehead{
                & \colhead{\emph{MIPS}} &  &  &     &     &     &    \\
\colhead{Index} & \colhead{160 \um} & \colhead{350 \um} & \colhead{450 \um}       & \colhead{850 \um} & \colhead{1100 \um} & \colhead{1200 \um} & \colhead{1300 \um}}
\startdata
   1 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
   2 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
   3 &             ... &             ... &             ... &             ... &             ... &     1500 $\pm$     120 &      680 $\pm$      22 \\
   4 &    12000 $\pm$    2400 &             ... &             ... &             ... &             ... &             ... &       60 $\pm$      15 \\
   5 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
   6 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
   7 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
   8 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
   9 &    27000 $\pm$    2700 &             ... &             ... &             ... &             ... &     1900 $\pm$     130 &             ... \\
  10 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  11 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  12 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  13 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  14 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  15 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  16 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  17 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  18 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  19 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  20 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  21 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  22 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  23 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  24 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  25 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  26 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  27 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  28 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  29 &             ... &             ... &             ... &             ... &             ... &             ... &       56 $\pm$      5.6 \\
  30 &             ... &             ... &             ... &             ... &             ... &             ... &       47 $\pm$      4.7 \\
  31 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  32 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  33 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  34 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  35 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  36 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  37 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  38 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  39 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  40 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  41 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  42 &             ... &             ... &             ... &             ... &             ... &             ... &       26 $\pm$      2.6 \\
  43 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  44 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  45 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  46 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  47 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  48 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  49 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  50 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  51 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  52 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  53 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  54 &             ... &             ... &             ... &             ... &             ... &             ... &       28 $\pm$      2.8 \\
  55 &             ... &             ... &             ... &             ... &             ... &             ... &       84 $\pm$      8.4 \\
  56 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  57 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  58 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  59 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  60 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  61 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  62 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  63 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  64 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  65 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  66 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  67 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  68 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  69 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  70 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  71 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  72 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  73 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  74 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  75 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  76 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  77 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  78 &     8700 $\pm$    2500 &             ... &             ... &             ... &             ... &      990 $\pm$     130 &             ... \\
  79 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  80 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  81 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  82 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  83 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  84 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  85 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  86 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  87 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  88 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  89 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  90 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  91 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  92 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  93 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  94 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  95 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  96 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  97 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  98 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  99 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 100 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 101 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 102 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 103 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 104 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 105 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 106 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 107 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 108 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 109 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 110 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 111 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 112 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 113 &     2300 $\pm$     230 &             ... &             ... &             ... &             ... &             ... &             ... \\
 114 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 115 &     5400 $\pm$    1600 &             ... &             ... &             ... &             ... &             ... &             ... \\
 116 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 117 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 118 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 119 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 120 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 121 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 122 &             ... &             ... &             ... &             ... &     1200 $\pm$     120 &             ... &             ... \\
 123 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 124 &             ... &             ... &             ... &             ... &     3700 $\pm$     370 &             ... &             ... \\
 125 &             ... &             ... &             ... &             ... &     1500 $\pm$     150 &             ... &             ... \\
 126 &             ... &             ... &             ... &             ... &     1500 $\pm$     150 &             ... &             ... \\
 127 &     9000 $\pm$    2600 &     4000 $\pm$     900 &    12000 $\pm$    2400 &      860 $\pm$     170 &      410 $\pm$      41 &             ... &             ... \\
 128 &     9500 $\pm$    1900 &     4000 $\pm$     800 &     1600 $\pm$     320 &      720 $\pm$     140 &      280 $\pm$      28 &             ... &             ... \\
 129 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 130 &             ... &    11000 $\pm$    2300 &             ... &             ... &      420 $\pm$      42 &             ... &             ... \\
 131 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 132 &    17000 $\pm$    3500 &     4300 $\pm$     900 &             ... &             ... &      410 $\pm$      41 &             ... &             ... \\
 133 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 134 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 135 &     1200 $\pm$     260 &             ... &             ... &             ... &      140 $\pm$      14 &             ... &             ... \\
 136 &     3300 $\pm$     100 &     1900 $\pm$     400 &             ... &      240 $\pm$      48 &      160 $\pm$      16 &             ... &             ... \\
 137 &     6400 $\pm$    1300 &             ... &             ... &             ... &       98 $\pm$      9.8 &             ... &             ... \\
 138 &             ... &     1600 $\pm$     300 &             ... &             ... &      200 $\pm$      20 &             ... &             ... \\
 139 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 140 &             ... &             ... &             ... &             ... &      110 $\pm$      11 &             ... &             ... \\
 141 &             ... &             ... &             ... &             ... &      360 $\pm$      36 &             ... &             ... \\
 142 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 143 &     4900 $\pm$    1400 &     2300 $\pm$     500 &             ... &      750 $\pm$     150 &      290 $\pm$      29 &             ... &             ... \\
 144 &     1100 $\pm$     220 &             ... &             ... &             ... &      400 $\pm$      40 &             ... &             ... \\
 145 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 146 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 147 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 148 &     6400 $\pm$    1300 &             ... &             ... &             ... &      200 $\pm$      20 &             ... &             ... \\
 149 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 150 &     5000 $\pm$    1600 &     2300 $\pm$     500 &      550 $\pm$     140 &      100 $\pm$      12 &      160 $\pm$      16 &             ... &             ... \\
 151 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 152 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 153 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 154 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 155 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 156 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 157 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 158 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 159 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 160 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 161 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 162 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 163 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 164 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 165 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 166 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 167 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 168 &             ... &             ... &             ... &             ... &     2300 $\pm$     230 &             ... &             ... \\
 169 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 170 &             ... &             ... &             ... &             ... &      200 $\pm$      20 &             ... &             ... \\
 171 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 172 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 173 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 174 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 175 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 176 &             ... &             ... &             ... &             ... &      600 $\pm$      60 &             ... &             ... \\
 177 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 178 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 179 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 180 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 181 &             ... &             ... &             ... &             ... &      580 $\pm$      58 &             ... &             ... \\
 182 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 183 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 184 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 185 &    14000 $\pm$    1400 &             ... &     2100 $\pm$     420 &      720 $\pm$     140 &      240 $\pm$      24 &             ... &             ... \\
 186 &             ... &             ... &             ... &             ... &     1500 $\pm$     150 &             ... &             ... \\
 187 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 188 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 189 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 190 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 191 &             ... &             ... &             ... &             ... &       90 $\pm$      9.0 &             ... &             ... \\
 192 &             ... &             ... &             ... &             ... &     2700 $\pm$     270 &             ... &             ... \\
 193 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 194 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 195 &             ... &             ... &             ... &             ... &      950 $\pm$      95 &             ... &             ... \\
 196 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 197 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 198 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 199 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 200 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 201 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 202 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 203 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 204 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 205 &             ... &             ... &             ... &             ... &     1300 $\pm$     130 &             ... &             ... \\
 206 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 207 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 208 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 209 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 210 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 211 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 212 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 213 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 214 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 215 &             ... &    39000 $\pm$    7800 &             ... &             ... &     6300 $\pm$     630 &             ... &             ... \\
 216 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 217 &             ... &             ... &             ... &             ... &     2000 $\pm$     200 &             ... &             ... \\
 218 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 219 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 220 &             ... &             ... &             ... &             ... &     2000 $\pm$     200 &             ... &             ... \\
 221 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 222 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 223 &             ... &    22000 $\pm$    4400 &             ... &             ... &     3000 $\pm$     300 &             ... &             ... \\
 224 &             ... &             ... &             ... &             ... &      630 $\pm$      63 &             ... &             ... \\
 225 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 226 &             ... &     6400 $\pm$    1400 &    21000 $\pm$    4200 &     2900 $\pm$     580 &      410 $\pm$      41 &             ... &             ... \\
 227 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 228 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 229 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 230 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 231 &             ... &     3500 $\pm$     400 &     2500 $\pm$     500 &     1400 $\pm$     280 &      410 $\pm$      41 &             ... &             ... \\
 232 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 233 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 234 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 235 &             ... &             ... &             ... &             ... &      360 $\pm$      36 &             ... &             ... \\
 236 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 237 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 238 &             ... &             ... &             ... &             ... &      420 $\pm$      42 &             ... &             ... \\
 239 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 240 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 241 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 242 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 243 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 244 &     4400 $\pm$    1300 &     1300 $\pm$     300 &             ... &     1600 $\pm$     310 &      520 $\pm$      52 &             ... &             ... \\
 245 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 246 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 247 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 248 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 249 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 250 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 251 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 252 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 253 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 254 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 255 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 256 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 257 &     6000 $\pm$    1700 &     4700 $\pm$    1000 &    12000 $\pm$    6400 &     4900 $\pm$    1200 &      520 $\pm$      52 &             ... &             ... \\
 258 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 259 &     9500 $\pm$    1900 &             ... &             ... &             ... &      380 $\pm$      38 &             ... &             ... \\
 260 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 261 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 262 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 263 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 264 &     2600 $\pm$     870 &     1600 $\pm$     300 &             ... &             ... &      810 $\pm$      81 &             ... &             ... \\
 265 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 266 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 267 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 268 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 269 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 270 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 271 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 272 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 273 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 274 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 275 &    16000 $\pm$    5700 &    12000 $\pm$    2100 &     3300 $\pm$     660 &     2300 $\pm$     450 &      780 $\pm$      78 &             ... &             ... \\
 276 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 277 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 278 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 279 &    24000 $\pm$    8400 &    18000 $\pm$    2800 &    22000 $\pm$    4300 &     5600 $\pm$    1100 &     2400 $\pm$     240 &             ... &             ... \\
 280 &     8300 $\pm$    2400 &     2900 $\pm$     400 &             ... &             ... &      370 $\pm$      37 &             ... &             ... \\
 281 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 282 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 283 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 284 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 285 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 286 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 287 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 288 &             ... &             ... &             ... &             ... &      170 $\pm$      17 &             ... &             ... \\
 289 &     8000 $\pm$    1600 &             ... &             ... &             ... &      430 $\pm$      43 &             ... &             ... \\
 290 &             ... &     1700 $\pm$     400 &             ... &             ... &      340 $\pm$      34 &             ... &             ... \\
 291 &    13000 $\pm$    1300 &     4500 $\pm$     900 &             ... &             ... &      850 $\pm$      85 &             ... &             ... \\
 292 &    14000 $\pm$    3900 &    16000 $\pm$    3200 &    50000 $\pm$   10000 &     5400 $\pm$    1100 &     1300 $\pm$     130 &             ... &             ... \\
 293 &             ... &             ... &             ... &             ... &      920 $\pm$      92 &             ... &             ... \\
 294 &             ... &             ... &             ... &             ... &     3100 $\pm$     310 &             ... &             ... \\
 295 &             ... &             ... &             ... &             ... &     1200 $\pm$     120 &             ... &             ... \\
 296 &    14000 $\pm$    2900 &             ... &             ... &             ... &      480 $\pm$      48 &             ... &             ... \\
 297 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 298 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 299 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 300 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 301 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 302 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 303 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 304 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 305 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 306 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 307 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 308 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 309 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 310 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 311 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 312 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 313 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 314 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 315 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 316 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 317 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 318 &             ... &             ... &             ... &             ... &       57 $\pm$      5.7 &             ... &             ... \\
 319 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 320 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 321 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 322 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 323 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 324 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 325 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 326 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 327 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 328 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 329 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 330 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 331 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 332 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 333 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 334 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 335 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 336 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 337 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 338 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 339 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 340 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 341 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 342 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 343 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 344 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 345 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 346 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 347 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 348 &             ... &             ... &             ... &             ... &      200 $\pm$      20 &             ... &             ... \\
 349 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 350 &             ... &     3400 $\pm$     700 &             ... &             ... &      940 $\pm$      94 &             ... &             ... \\
 351 &             ... &     2300 $\pm$     500 &             ... &     1500 $\pm$     290 &      510 $\pm$      51 &             ... &             ... \\
 352 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 353 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 354 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 355 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 356 &             ... &    25000 $\pm$    4100 &    83000 $\pm$   17000 &     8200 $\pm$    1600 &     2500 $\pm$     250 &             ... &             ... \\
 357 &             ... &             ... &    18000 $\pm$    3500 &     3600 $\pm$     720 &     1500 $\pm$     150 &             ... &             ... \\
 358 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 359 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 360 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 361 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 362 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 363 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 364 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 365 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 366 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 367 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 368 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 369 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 370 &             ... &             ... &             ... &      940 $\pm$     190 &      510 $\pm$      51 &             ... &             ... \\
 371 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 372 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 373 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 374 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 375 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 376 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 377 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 378 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 379 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 380 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 381 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 382 &             ... &             ... &             ... &             ... &       98 $\pm$      9.8 &             ... &             ... \\
 383 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 384 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 385 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 386 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 387 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 388 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 389 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 390 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 391 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 392 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 393 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 394 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 395 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 396 &             ... &      400 $\pm$     100 &             ... &             ... &      140 $\pm$      14 &             ... &             ... \\
 397 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 398 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 399 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 400 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 401 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 402 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 403 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 404 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 405 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 406 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 407 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 408 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 409 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 410 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 411 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 412 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 413 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 414 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 415 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 416 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 417 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 418 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 419 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 420 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 421 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 422 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 423 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 424 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 425 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 426 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 427 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 428 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 429 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 430 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 431 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 432 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 433 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 434 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 435 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 436 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 437 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 438 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 439 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 440 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 441 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 442 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 443 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 444 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 445 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 446 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 447 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 448 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 449 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 450 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 451 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 452 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 453 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 454 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 455 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 456 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 457 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 458 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 459 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 460 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 461 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 462 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 463 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 464 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 465 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 466 &             ... &             ... &             ... &             ... &      260 $\pm$      26 &             ... &             ... \\
 467 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 468 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 469 &    46000 $\pm$    4600 &             ... &             ... &             ... &      510 $\pm$      51 &             ... &             ... \\
 470 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 471 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 472 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 473 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 474 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 475 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 476 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 477 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 478 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 479 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 480 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 481 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 482 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 483 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 484 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 485 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 486 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 487 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 488 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 489 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 490 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 491 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 492 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 493 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 494 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 495 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 496 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 497 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 498 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 499 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 500 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 501 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 502 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 503 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 504 &     2300 $\pm$     480 &             ... &             ... &             ... &      110 $\pm$      11 &             ... &             ... \\
 505 &    20000 $\pm$    4100 &    12000 $\pm$    1700 &             ... &             ... &     1400 $\pm$     140 &             ... &             ... \\
 506 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 507 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 508 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 509 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 510 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 511 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 512 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 513 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 514 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 515 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 516 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 517 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 518 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 519 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 520 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 521 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 522 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 523 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 524 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 525 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 526 &             ... &             ... &             ... &             ... &      210 $\pm$      21 &             ... &             ... \\
 527 &             ... &             ... &             ... &             ... &      200 $\pm$      20 &             ... &             ... \\
 528 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 529 &     9300 $\pm$     930 &             ... &             ... &             ... &      240 $\pm$      24 &             ... &             ... \\
 530 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 531 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 532 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 533 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 534 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 535 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 536 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 537 &             ... &             ... &             ... &             ... &      130 $\pm$      13 &             ... &             ... \\
 538 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 539 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 540 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 541 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 542 &    35000 $\pm$    3500 &             ... &             ... &             ... &     1400 $\pm$     140 &             ... &             ... \\
 543 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 544 &    35000 $\pm$    3500 &             ... &             ... &             ... &     1300 $\pm$     130 &             ... &             ... \\
 545 &             ... &             ... &             ... &             ... &      200 $\pm$      20 &             ... &             ... \\
 546 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 547 &             ... &             ... &             ... &             ... &      970 $\pm$      97 &             ... &             ... \\
 548 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 549 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 550 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 551 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 552 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 553 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 554 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 555 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 556 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 557 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 558 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 559 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 560 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 561 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 562 &             ... &             ... &             ... &             ... &      140 $\pm$      14 &             ... &             ... \\
 563 &             ... &             ... &             ... &             ... &      180 $\pm$      18 &             ... &             ... \\
 564 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 565 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 566 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 567 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 568 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 569 &             ... &             ... &             ... &             ... &     1100 $\pm$     110 &             ... &             ... \\
 570 &             ... &             ... &             ... &             ... &     1100 $\pm$     110 &             ... &             ... \\
 571 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 572 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 573 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 574 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 575 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 576 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 577 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 578 &             ... &             ... &             ... &             ... &      950 $\pm$      95 &             ... &             ... \\
 579 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 580 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 581 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 582 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 583 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 584 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 585 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 586 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 587 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 588 &    10000 $\pm$    2100 &             ... &             ... &             ... &      440 $\pm$     440 &             ... &             ... \\
 589 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 590 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 591 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 592 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 593 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 594 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 595 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 596 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 597 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 598 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 599 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 600 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 601 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 602 &    24000 $\pm$    5000 &             ... &             ... &             ... &     1700 $\pm$    1700 &             ... &             ... \\
 603 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 604 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 605 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 606 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 607 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 608 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 609 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 610 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 611 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 612 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 613 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 614 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 615 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 616 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 617 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 618 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 619 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 620 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 621 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 622 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 623 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 624 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 625 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 626 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 627 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 628 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 629 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 630 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 631 &             ... &             ... &             ... &             ... &     3000 $\pm$     300 &             ... &             ... \\
 632 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 633 &             ... &             ... &             ... &             ... &     1300 $\pm$     130 &             ... &             ... \\
 634 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 635 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 636 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 637 &             ... &             ... &             ... &             ... &     6500 $\pm$     650 &             ... &             ... \\
 638 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 639 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 640 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 641 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 642 &             ... &             ... &             ... &             ... &     1500 $\pm$     150 &             ... &             ... \\
 643 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 644 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 645 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 646 &             ... &             ... &             ... &             ... &     1000 $\pm$     100 &             ... &             ... \\
 647 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 648 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 649 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 650 &     9600 $\pm$    1900 &             ... &             ... &             ... &      440 $\pm$      44 &             ... &             ... \\
 651 &             ... &             ... &             ... &             ... &      600 $\pm$      60 &             ... &             ... \\
 652 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 653 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 654 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 655 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 656 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 657 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 658 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 659 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 660 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 661 &     8600 $\pm$    1700 &             ... &             ... &             ... &      390 $\pm$      39 &             ... &             ... \\
 662 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 663 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 664 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 665 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 666 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 667 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 668 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 669 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 670 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 671 &             ... &             ... &             ... &             ... &      560 $\pm$      56 &             ... &             ... \\
 672 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 673 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 674 &             ... &             ... &             ... &             ... &     1900 $\pm$     190 &             ... &             ... \\
 675 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 676 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 677 &             ... &             ... &             ... &             ... &     1600 $\pm$     160 &             ... &             ... \\
 678 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 679 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 680 &             ... &             ... &             ... &             ... &      870 $\pm$      87 &             ... &             ... \\
 681 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 682 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 683 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 684 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 685 &             ... &             ... &             ... &             ... &     1600 $\pm$     160 &             ... &             ... \\
 686 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 687 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 688 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 689 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 690 &             ... &             ... &             ... &             ... &     2100 $\pm$     210 &             ... &             ... \\
 691 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 692 &             ... &             ... &             ... &             ... &      930 $\pm$      93 &             ... &             ... \\
 693 &             ... &             ... &             ... &             ... &     2100 $\pm$     210 &             ... &             ... \\
 694 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 695 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 696 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 697 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 698 &             ... &             ... &             ... &             ... &     2100 $\pm$     210 &             ... &             ... \\
 699 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 700 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 701 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 702 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 703 &             ... &             ... &             ... &             ... &     1100 $\pm$     110 &             ... &             ... \\
 704 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 705 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 706 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 707 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 708 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 709 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 710 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 711 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 712 &             ... &             ... &             ... &             ... &      160 $\pm$      16 &             ... &             ... \\
 713 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 714 &             ... &             ... &             ... &             ... &      160 $\pm$      16 &             ... &             ... \\
 715 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 716 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 717 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 718 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 719 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 720 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 721 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 722 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 723 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 724 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 725 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 726 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 727 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 728 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 729 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 730 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 731 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 732 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 733 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 734 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 735 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 736 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 737 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 738 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 739 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 740 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 741 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 742 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 743 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 744 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 745 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 746 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 747 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 748 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 749 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 750 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 751 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 752 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 753 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 754 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 755 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 756 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 757 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 758 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 759 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 760 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 761 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 762 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 763 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 764 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 765 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 766 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 767 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 768 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 769 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 770 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 771 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 772 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 773 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 774 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 775 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 776 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 777 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 778 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 779 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 780 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 781 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 782 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 783 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 784 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 785 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 786 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 787 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 788 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 789 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 790 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 791 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 792 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 793 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 794 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 795 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 796 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 797 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 798 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 799 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 800 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 801 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 802 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 803 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 804 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 805 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 806 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 807 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 808 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 809 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 810 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 811 &             ... &             ... &             ... &             ... &      720 $\pm$      72 &             ... &             ... \\
 812 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 813 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 814 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 815 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 816 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 817 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 818 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 819 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 820 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 821 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 822 &             ... &             ... &             ... &             ... &     1700 $\pm$     170 &             ... &             ... \\
 823 &             ... &             ... &             ... &             ... &      780 $\pm$      78 &             ... &             ... \\
 824 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 825 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 826 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 827 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 828 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 829 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 830 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 831 &             ... &             ... &             ... &             ... &      200 $\pm$      20 &             ... &             ... \\
 832 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 833 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 834 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 835 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 836 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 837 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 838 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 839 &             ... &             ... &             ... &             ... &       98 $\pm$      9.8 &             ... &             ... \\
 840 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 841 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 842 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 843 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 844 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 845 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 846 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 847 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 848 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 849 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 850 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 851 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 852 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 853 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 854 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 855 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 856 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 857 &             ... &             ... &             ... &             ... &      260 $\pm$      26 &             ... &             ... \\
 858 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 859 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 860 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 861 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 862 &             ... &             ... &             ... &      440 $\pm$      44 &      290 $\pm$      29 &             ... &             ... \\
 863 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 864 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 865 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 866 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 867 &             ... &             ... &             ... &             ... &      160 $\pm$      16 &             ... &             ... \\
 868 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 869 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 870 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 871 &             ... &             ... &             ... &             ... &       57 $\pm$      5.7 &             ... &             ... \\
 872 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 873 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 874 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 875 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 876 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 877 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 878 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 879 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 880 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 881 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 882 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 883 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 884 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 885 &             ... &             ... &             ... &             ... &      230 $\pm$      23 &             ... &             ... \\
 886 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 887 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 888 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 889 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 890 &             ... &             ... &             ... &             ... &      130 $\pm$      13 &             ... &             ... \\
 891 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 892 &             ... &             ... &             ... &             ... &      390 $\pm$      39 &             ... &             ... \\
 893 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 894 &             ... &             ... &             ... &             ... &      390 $\pm$      39 &             ... &             ... \\
 895 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 896 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 897 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 898 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 899 &             ... &             ... &             ... &             ... &     1200 $\pm$     120 &             ... &             ... \\
 900 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 901 &             ... &             ... &             ... &             ... &      360 $\pm$      36 &             ... &             ... \\
 902 &             ... &             ... &             ... &             ... &      950 $\pm$      95 &             ... &             ... \\
 903 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 904 &             ... &             ... &             ... &             ... &      620 $\pm$      62 &             ... &             ... \\
 905 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 906 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 907 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 908 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 909 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 910 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 911 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 912 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 913 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 914 &             ... &             ... &             ... &             ... &      130 $\pm$      13 &             ... &             ... \\
 915 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 916 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 917 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 918 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 919 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 920 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 921 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 922 &             ... &             ... &             ... &             ... &      130 $\pm$      13 &             ... &             ... \\
 923 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 924 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 925 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 926 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 927 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 928 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 929 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 930 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 931 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 932 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 933 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 934 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 935 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 936 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 937 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 938 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 939 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 940 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 941 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 942 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 943 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 944 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 945 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 946 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 947 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 948 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 949 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 950 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 951 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 952 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 953 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 954 &    19000 $\pm$    5300 &     5300 $\pm$    1100 &             ... &             ... &     1700 $\pm$     170 &      410 $\pm$      41 &             ... \\
 955 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 956 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 957 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 958 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 959 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 960 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 961 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 962 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 963 &             ... &             ... &             ... &             ... &      130 $\pm$      13 &             ... &             ... \\
 964 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 965 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 966 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 967 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 968 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 969 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 970 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 971 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 972 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 973 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 974 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 975 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 976 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 977 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 978 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 979 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 980 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 981 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 982 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 983 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 984 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 985 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 986 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 987 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 988 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 989 &    51000 $\pm$   15000 &             ... &             ... &             ... &      460 $\pm$      46 &             ... &             ... \\
 990 &    14000 $\pm$    3900 &             ... &             ... &             ... &       98 $\pm$      9.8 &             ... &             ... \\
 991 &             ... &             ... &             ... &             ... &      130 $\pm$      13 &             ... &             ... \\
 992 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 993 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 994 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 995 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 996 &             ... &             ... &             ... &             ... &      160 $\pm$      16 &             ... &             ... \\
 997 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 998 &             ... &             ... &             ... &             ... &      260 $\pm$      26 &             ... &             ... \\
 999 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1000 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1001 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1002 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1003 &             ... &             ... &             ... &             ... &      160 $\pm$      16 &             ... &             ... \\
1004 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1005 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1006 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1007 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1008 &             ... &             ... &             ... &             ... &     3800 $\pm$     380 &             ... &             ... \\
1009 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1010 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1011 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1012 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1013 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1014 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1015 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1016 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1017 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1018 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1019 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1020 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1021 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1022 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1023 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1024 &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
\enddata \\
\end{deluxetable}
\end{landscape}


==> tab12.tex <==
\begin{landscape}
\begin{deluxetable}{rlclrrrrrrrcr}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\tablecaption{\label{tabysoprops}Properties of YSOs in the c2d Clouds}
\tablehead{
                &                 & \colhead{Spitzer}      &                          &         & \multicolumn{3}{c}{Observed}  & \multicolumn{3}{c}{Extinction Corrected}  &                                     &                   \\
                &                 & \colhead{Source Name}  & \colhead{c2d}            &         &          & \colhead{\tbol} & \colhead{\lbol}    &          & \colhead{\tbol$^{\prime}$} & \colhead{\lbol$^{\prime}$}      &                                     &                   \\
\colhead{Index} & \colhead{Cloud} & \colhead{(SSTc2d $+$)} & \colhead{Classification} & \colhead{A$_{\rm V}$\tablenotemark{a}} & \colhead{$\alpha$} & \colhead{(K)}    & \colhead{(\lsun)}   & \colhead{$\alpha^{\prime}$} & \colhead{(K)}    & \colhead{(\lsun)}     & \colhead{Envelope\tablenotemark{b}} & \colhead{Quality\tablenotemark{c}}}
\startdata
   1 & Cham II & J124825.74$-$770636.5 & YSOc\_star$+$dust(MP1) &  4.4 &   $-$2.19 &       2200 &       11 &   $-$2.59 &       3000 &       28 & N &    G \\
   2 & Cham II & J125230.66$-$771513.0 & YSOc\_star$+$dust(MP1) &  4.3 &   $-$2.38 &       2100 &       1.4 &   $-$2.71 &       2700 &       3.2 & N &    G \\
   3 & Cham II & J125317.23$-$770710.7 &              rising & 10.5 &   $-$0.72 &        550 &       38 &   $-$0.14 &       1400 &       72 & N &    G \\
   4 & Cham II & J125342.86$-$771511.5 &            YSOc\_red &  4.0 &    0.65 &        120 &       0.49 &    0.21 &        190 &       0.59 & Y &    G \\
   5 & Cham II & J125633.66$-$764545.3 & YSOc\_star$+$dust(IR2) &  2.4 &   $-$1.22 &       2200 &       0.21 &   $-$1.35 &       2900 &       0.36 & N &    G \\
   6 & Cham II & J125658.68$-$764706.6 & YSOc\_star$+$dust(IR2) &  0.0 &   $-$1.84 & $\geq$4500 & $\geq$0.067 &   $-$1.84 & $\geq$4500 & $\geq$0.067 & N & L\_II \\
   7 & Cham II & J125711.77$-$764011.3 & YSOc\_star$+$dust(IR1) &  3.3 &   $-$0.85 &       1800 &       0.86 &   $-$1.06 &       3100 &       1.8 & N &    G \\
   8 & Cham II & J125806.78$-$770909.4 & YSOc\_star$+$dust(IR1) &  5.0 &   $-$0.93 &       1400 &       0.013 &   $-$1.09 &       1900 &       0.020 & N &    G \\
   9 & Cham II & J125906.58$-$770739.9 &            YSOc\_red &  4.0 &    0.68 &        220 &       1.9 &    0.49 &        270 &       2.4 & Y &    G \\
  10 & Cham II & J125926.45$-$774708.4 & YSOc\_star$+$dust(IR4) &  3.9 &   $-$1.78 &       2400 &       3.7 &   $-$2.01 &       3300 &       9.8 & N &    G \\
  11 & Cham II & J130055.36$-$771022.1 & YSOc\_star$+$dust(IR2) &  3.8 &   $-$0.65 &       1800 &       0.55 &   $-$0.90 &       3000 &       1.2 & N &    G \\
  12 & Cham II & J130059.29$-$771402.7 & YSOc\_star$+$dust(IR3) &  9.0 &   $-$1.14 &       1300 &       0.75 &   $-$1.82 &       1900 &       1.9 & N &    G \\
  13 & Cham II & J130158.94$-$775121.7 & YSOc\_star$+$dust(IR1) &  1.5 &   $-$1.19 &       2300 &       0.40 &   $-$1.10 &       3100 &       0.59 & N &    G \\
  14 & Cham II & J130222.85$-$773449.3 & YSOc\_star$+$dust(IR4) &  2.9 &   $-$1.46 &       2200 &       0.040 &   $-$1.54 &       2800 &       0.070 & N &    G \\
  15 & Cham II & J130424.92$-$775230.1 & YSOc\_star$+$dust(IR3) &  4.2 &   $-$0.97 &       1300 &       0.13 &   $-$1.19 &       2300 &       0.25 & N &    G \\
  16 & Cham II & J130455.75$-$773949.5 & YSOc\_star$+$dust(IR4) &  2.7 &   $-$0.85 &       2400 &       0.51 &   $-$1.22 &       3800 &       1.2 & N &    G \\
  17 & Cham II & J130508.53$-$773342.4 & YSOc\_star$+$dust(IR1) &  4.1 &   $-$1.05 &       1700 &       0.18 &   $-$1.19 &       3100 &       0.41 & N &    G \\
  18 & Cham II & J130512.69$-$773052.3 & YSOc\_star$+$dust(IR1) &  3.7 &   $-$0.98 &       1700 &       0.19 &   $-$1.10 &       3000 &       0.40 & N &    G \\
  19 & Cham II & J130520.68$-$773901.4 & YSOc\_star$+$dust(IR2) &  1.6 &   $-$1.35 &       2500 &       1.6 &   $-$1.48 &       3300 &       2.5 & N &    G \\
  20 & Cham II & J130521.66$-$773810.0 & YSOc\_star$+$dust(IR2) &  4.0 &   $-$0.05 &       2000 &       0.010 &   $-$0.47 &       5800 &       0.14 & N &    G \\
  21 & Cham II & J130529.04$-$774140.1 &                YSOc &  0.0 &   $-$0.37 & $\geq$540 & $\geq$0.0030 &   $-$0.37 & $\geq$540 & $\geq$0.0030 & N & L\_II \\
  22 & Cham II & J130718.05$-$774052.9 & YSOc\_star$+$dust(IR3) &  4.8 &   $-$1.11 &       1900 &       0.033 &   $-$1.23 &       2700 &       0.080 & N &    G \\
  23 & Cham II & J130748.51$-$774121.4 & YSOc\_star$+$dust(IR2) &  3.5 &   $-$0.90 &       1800 &       0.16 &   $-$1.10 &       2800 &       0.32 & N &    G \\
  24 & Cham II & J130806.28$-$775505.2 & YSOc\_star$+$dust(IR1) &  3.1 &   $-$0.90 &       1600 &       1.2 &   $-$1.00 &       2500 &       2.0 & N &    G \\
  25 & Cham II & J130827.17$-$774323.2 & YSOc\_star$+$dust(IR2) &  4.3 &   $-$1.23 &       2100 &       0.018 &   $-$1.35 &       3200 &       0.050 & N &    G \\
  26 & Cham II & J130950.38$-$775723.9 & YSOc\_star$+$dust(IR2) &  0.8 &   $-$1.10 &       2200 &       0.040 &   $-$1.26 &       2400 &       0.47 & N &    G \\
  27 &     Lup & J153803.10$-$331357.7 & YSOc\_star$+$dust(MP1) &  3.0 &   $-$2.21 &       2200 &       0.90 &   $-$2.30 &       2700 &       1.7 & N &    G \\
  28 &     Lup & J153848.36$-$344038.2 &         YSOc\_PAH$-$em &  2.9 &    0.58 &        190 &       0.11 &    0.31 &        260 &       0.13 & N &    G \\
  29 &     Lup & J153927.78$-$344617.4 & YSOc\_star$+$dust(IR3) &  1.0 &   $-$0.84 &       2600 &       0.98 &   $-$0.81 &       3200 &       1.3 & N &    G \\
  30 &     Lup & J153928.29$-$344618.3 & YSOc\_star$+$dust(IR3) &  2.0 &   $-$0.84 &       1600 &       0.32 &   $-$0.64 &       2100 &       0.45 & N &    G \\
  31 &     Lup & J154214.57$-$341025.8 &         YSOc\_PAH$-$em &  2.9 &    0.78 &        270 &       0.029 &    0.42 &        400 &       0.036 & N &    G \\
  32 &     Lup & J154240.32$-$341343.0 & YSOc\_star$+$dust(MP1) &  9.0 &   $-$2.28 &       1900 &       0.32 &   $-$2.59 &       4700 &       2.8 & N &    G \\
  33 &     Lup & J154301.29$-$340915.4 & YSOc\_star$+$dust(IR2) &  2.9 &   $-$0.21 &        770 &       0.0047 &   $-$0.36 &        900 &       0.0071 & N &    G \\
  34 &     Lup & J154302.29$-$344406.2 & YSOc\_star$+$dust(IR1) &  2.9 &    0.18 &        750 &       0.0086 &    0.14 &       3100 &       0.017 & N &    G \\
  35 &     Lup & J154457.90$-$342339.5 & Galc\_star$+$dust(IR4) &  0.0 &   $-$1.41 & $\geq$2600 & $\geq$0.020 &   $-$1.41 & $\geq$2600 & $\geq$0.020 & N & L\_II \\
  36 &     Lup & J154506.34$-$341738.1 &            YSOc\_red &  2.9 &   $-$0.29 &        650 &       0.029 &   $-$0.47 &        780 &       0.041 & N &    G \\
  37 &     Lup & J154508.88$-$341733.7 & YSOc\_star$+$dust(IR1) & 10.0 &   $-$0.89 &       1300 &       0.17 &   $-$1.13 &       3000 &       0.84 & N &    G \\
  38 &     Lup & J154517.42$-$341828.5 & YSOc\_star$+$dust(IR1) &  4.0 &   $-$1.16 &       1900 &       0.22 &   $-$1.21 &       3100 &       0.51 & N &    G \\
  39 &     Lup & J154518.53$-$342124.8 & YSOc\_star$+$dust(IR1) &  2.0 &   $-$1.00 &       2100 &       0.093 &   $-$1.08 &       2400 &       0.13 & N &    G \\
  40 &     Lup & J160703.85$-$391111.6 & YSOc\_star$+$dust(IR1) &  2.9 &    0.09 &        970 &       0.026 &   $-$0.14 &       1500 &       0.045 & N &    G \\
  41 &     Lup & J160708.56$-$391407.7 &                YSOc &  2.9 &    0.05 &        640 &       0.12 &   $-$0.01 &        770 &       0.18 & N &    G \\
  42 &     Lup & J160710.08$-$391103.5 & YSOc\_star$+$dust(IR2) &  3.0 &   $-$1.04 &       2100 &       0.70 &   $-$1.02 &       3700 &       1.6 & N &    G \\
  43 &     Lup & J160711.60$-$390347.7 & YSOc\_star$+$dust(MP1) &  1.0 &   $-$2.04 &       2500 &       0.27 &   $-$1.89 &       2900 &       0.35 & N &    G \\
  44 &     Lup & J160737.72$-$392138.8 & YSOc\_star$+$dust(IR2) &  0.0 &   $-$1.09 & $\geq$2300 & $\geq$0.032 &   $-$1.09 & $\geq$2300 & $\geq$0.032 & N & L\_II \\
  45 &     Lup & J160752.32$-$385806.3 & YSOc\_star$+$dust(IR4) &  1.0 &   $-$1.29 &       2700 &       0.25 &   $-$1.31 &       3100 &       0.33 & N &    G \\
  46 &     Lup & J160754.09$-$392046.2 & YSOc\_star$+$dust(MP1) &  5.0 &   $-$2.28 &       2400 &       1.0 &   $-$2.43 &       3700 &       4.0 & N &    G \\
  47 &     Lup & J160754.73$-$391544.5 &            YSOc\_red &  2.9 &   $-$0.13 &        480 &       0.013 &   $-$0.15 &        670 &       0.018 & N &    G \\
  48 &     Lup & J160755.29$-$390717.8 & YSOc\_star$+$dust(IR4) & 10.0 &   $-$1.86 &       1700 &       1.1 &   $-$2.16 &       2600 &       5.3 & N &    G \\
  49 &     Lup & J160800.16$-$390259.5 & YSOc\_star$+$dust(IR2) &  1.0 &   $-$1.12 &       2400 &       0.086 &   $-$1.15 &       2700 &       0.11 & N &    G \\
  50 &     Lup & J160803.02$-$385229.3 & YSOc\_star$+$dust(MP1) &  4.0 &   $-$2.32 &       2400 &       1.0 &   $-$2.43 &       4100 &       3.6 & N &    G \\
  51 &     Lup & J160806.17$-$391222.5 & YSOc\_star$+$dust(IR4) &  7.0 &   $-$1.55 &       1800 &       1.1 &   $-$1.84 &       2600 &       3.7 & N &    G \\
  52 &     Lup & J160812.62$-$390833.5 & YSOc\_star$+$dust(IR1) &  0.0 &   $-$0.83 & $\geq$2200 & $\geq$0.68 &   $-$0.83 & $\geq$2200 & $\geq$0.68 & N & L\_II \\
  53 &     Lup & J160814.96$-$385714.5 &                YSOc &  1.0 &   $-$0.71 &       1500 &       0.012 &   $-$0.73 &       1600 &       0.014 & N &    G \\
  54 &     Lup & J160821.79$-$390421.5 & YSOc\_star$+$dust(IR2) &  1.0 &   $-$1.13 &       2700 &       0.21 &   $-$1.18 &       3100 &       0.28 & N &    G \\
  55 &     Lup & J160822.48$-$390446.3 & YSOc\_star$+$dust(IR1) &  0.0 &   $-$0.48 & $\geq$1900 & $\geq$1.8 &   $-$0.48 & $\geq$1900 & $\geq$1.8 & N & L\_II \\
  56 &     Lup & J160824.03$-$390549.4 & YSOc\_star$+$dust(IR2) &  0.0 &   $-$1.08 & $\geq$250 & $\geq$0.11 &   $-$1.08 & $\geq$2500 & $\geq$0.11 & N & L\_II \\
  57 &     Lup & J160825.75$-$390601.2 & YSOc\_star$+$dust(IR2) &  1.0 &   $-$0.71 &       2100 &       0.29 &   $-$0.73 &       2400 &       0.36 & N &    G \\
  58 &     Lup & J160828.41$-$390532.3 & YSOc\_star$+$dust(IR4) &  2.0 &   $-$1.76 &       2500 &       0.40 &   $-$1.73 &       2900 &       0.66 & N &    G \\
  59 &     Lup & J160829.73$-$390311.0 &            YSOc\_red &  2.9 &    0.72 &        740 &       0.14 &    0.58 &       3000 &       0.29 & N &    G \\
  60 &     Lup & J160830.26$-$390611.1 & YSOc\_star$+$dust(IR3) &  1.0 &   $-$0.76 &       2100 &       0.21 &   $-$0.78 &       2300 &       0.26 & N &    G \\
  61 &     Lup & J160830.80$-$390548.8 & YSOc\_star$+$dust(IR2) &  0.0 &   $-$0.91 & $\geq$2200 & $\geq$0.17 &   $-$0.91 & $\geq$2200 & $\geq$0.17 & N & L\_II \\
  62 &     Lup & J160839.76$-$390625.3 & YSOc\_star$+$dust(IR1) &  0.0 &   $-$0.94 & $\geq$1700 & $\geq$0.20 &   $-$0.94 & $\geq$1700 & $\geq$0.20 & N & L\_II \\
  63 &     Lup & J160841.79$-$390137.0 & YSOc\_star$+$dust(MP1) &  1.0 &   $-$1.79 &       2700 &       0.17 &   $-$1.67 &       2900 &       0.23 & N &    G \\
  64 &     Lup & J160842.87$-$390614.6 & YSOc\_star$+$dust(IR4) &  4.0 &   $-$0.85 &       1700 &       0.100 &   $-$0.75 &       3000 &       0.26 & N &    G \\
  65 &     Lup & J160849.40$-$390539.3 & YSOc\_star$+$dust(IR2) &  0.0 &   $-$0.57 & $\geq$1700 & $\geq$0.29 &   $-$0.57 & $\geq$1700 & $\geq$0.29 & N & L\_II \\
  66 &     Lup & J160851.43$-$390530.4 & YSOc\_star$+$dust(IR2) &  0.0 &   $-$0.35 & $\geq$390 & $\geq$0.038 &   $-$0.35 & $\geq$390 & $\geq$0.038 & N & L\_II \\
  67 &     Lup & J160851.56$-$390317.7 & YSOc\_star$+$dust(IR2) &  0.0 &   $-$0.74 & $\geq$2500 & $\geq$0.34 &   $-$0.74 & $\geq$2500 & $\geq$0.34 & N & L\_II \\
  68 &     Lup & J160853.23$-$391440.3 & YSOc\_star$+$dust(IR3) &  2.0 &   $-$1.14 &       2100 &       0.24 &   $-$1.18 &       2600 &       0.36 & N &    G \\
  69 &     Lup & J160853.73$-$391436.8 & YSOc\_star$+$dust(IR2) &  8.0 &   $-$1.22 &       1500 &       0.016 &   $-$1.32 &       2700 &       0.059 & N &    G \\
  70 &     Lup & J160855.28$-$384848.2 & YSOc\_star$+$dust(IR2) &  3.0 &   $-$1.14 &       2500 &       0.038 &   $-$1.22 &       4000 &       0.098 & N &    G \\
  71 &     Lup & J160855.52$-$390233.9 & YSOc\_star$+$dust(IR4) &  1.0 &   $-$0.94 &       2300 &       0.27 &   $-$0.79 &       2600 &       0.34 & N &    G \\
  72 &     Lup & J160857.79$-$390222.8 & YSOc\_star$+$dust(IR2) &  2.0 &   $-$0.53 &       1900 &       0.086 &   $-$0.58 &       2700 &       0.13 & N &    G \\
  73 &     Lup & J160858.27$-$390735.5 &                YSOc &  0.0 &   $-$1.26 & $\geq$880 & $\geq$0.042 &   $-$1.26 & $\geq$880 & $\geq$0.042 & N & L\_II \\
  74 &     Lup & J160859.53$-$385627.6 & YSOc\_star$+$dust(IR2) &  0.0 &   $-$0.90 & $\geq$2000 & $\geq$0.017 &   $-$0.90 & $\geq$2000 & $\geq$0.017 & N & L\_II \\
  75 &     Lup & J160901.40$-$392511.9 & YSOc\_star$+$dust(IR2) &  0.0 &   $-$1.17 & $\geq$2200 & $\geq$0.18 &   $-$1.17 & $\geq$2200 & $\geq$0.18 & N & L\_II \\
  76 &     Lup & J160901.84$-$390512.5 & YSOc\_star$+$dust(IR2) &  2.0 &   $-$0.55 &       2100 &       0.54 &   $-$0.58 &       3000 &       0.88 & N &    G \\
  77 &     Lup & J160906.21$-$390851.8 & YSOc\_star$+$dust(IR3) &  1.0 &   $-$1.58 &       2800 &       0.17 &   $-$1.58 &       3100 &       0.22 & N &    G \\
  78 &     Lup & J160918.07$-$390453.4 &            YSOc\_red &  2.9 &    1.10 &         39 &       0.37 &    1.17 &         41 &       0.39 & Y &    G \\
  79 &     Lup & J160934.11$-$391342.1 &                YSOc &  6.0 &   $-$2.26 &       2100 &       2.7 &   $-$2.47 &       3100 &       9.5 & N &    G \\
  80 &     Lup & J160944.35$-$391330.3 & YSOc\_star$+$dust(IR2) &  1.0 &   $-$1.05 &       2400 &       0.38 &   $-$1.06 &       2800 &       0.49 & N &    G \\
  81 &     Lup & J160948.64$-$391116.9 & YSOc\_star$+$dust(IR2) &  6.0 &   $-$0.77 &       1500 &       0.72 &   $-$0.96 &       3200 &       2.1 & N &    G \\
  82 &     Lup & J160956.29$-$385951.7 & YSOc\_star$+$dust(IR2) &  1.0 &   $-$0.90 &       2200 &       0.045 &   $-$0.93 &       2600 &       0.057 & N &    G \\
  83 &     Lup & J161000.11$-$385401.1 & YSOc\_star$+$dust(IR3) & 12.0 &   $-$1.69 &       2000 &       1.2 &   $-$2.03 &       3900 &       30 & N &    G \\
  84 &     Lup & J161001.32$-$390644.9 & YSOc\_star$+$dust(IR3) &  7.0 &   $-$1.24 &       2000 &       0.100 &   $-$1.41 &       5800 &       1.2 & N &    G \\
  85 &     Lup & J161013.06$-$384616.8 &            YSOc\_red &  2.9 &   $-$0.28 &       1400 &       0.0074 &   $-$0.49 &       2000 &       0.015 & N &    G \\
  86 &     Lup & J161018.56$-$383613.0 & YSOc\_star$+$dust(IR2) &  2.0 &   $-$1.46 &       2700 &       0.048 &   $-$1.50 &       3400 &       0.087 & N &    G \\
  87 &     Lup & J161019.84$-$383606.8 & YSOc\_star$+$dust(IR2) &  2.0 &   $-$1.14 &       2600 &       0.029 &   $-$1.19 &       3600 &       0.053 & N &    G \\
  88 &     Lup & J161027.43$-$390230.2 & YSOc\_star$+$dust(IR4) &  2.9 &   $-$0.01 &       1300 &       0.0034 &   $-$0.19 &       1700 &       0.0063 & N &    G \\
  89 &     Lup & J161029.57$-$392214.7 & YSOc\_star$+$dust(IR4) &  1.0 &   $-$1.07 &       2300 &       0.11 &   $-$0.94 &       2600 &       0.14 & N &    G \\
  90 &     Lup & J161032.59$-$374614.9 & YSOc\_star$+$dust(MP1) &  6.0 &   $-$2.22 &       1600 &       5.7 &   $-$2.35 &       2700 &       16 & N &    G \\
  91 &     Lup & J161034.51$-$381450.3 & YSOc\_star$+$dust(IR4) &  5.0 &   $-$2.18 &       2100 &       4.4 &   $-$2.34 &       2800 &       12 & N &    G \\
  92 &     Lup & J161034.97$-$390654.6 & YSOc\_star$+$dust(MP1) &  6.0 &   $-$2.25 &       1900 &       0.71 &   $-$2.42 &       3200 &       2.4 & N &    G \\
  93 &     Lup & J161045.38$-$385454.9 & YSOc\_star$+$dust(IR1) &  0.0 &   $-$0.94 & $\geq$2300 & $\geq$0.018 &   $-$0.94 & $\geq$2300 & $\geq$0.018 & N & L\_II \\
  94 &     Lup & J161051.60$-$385314.0 & YSOc\_star$+$dust(IR3) &  0.0 &   $-$1.15 & $\geq$2300 & $\geq$0.29 &   $-$1.15 & $\geq$2300 & $\geq$0.29 & N & L\_II \\
  95 &     Lup & J161118.69$-$385823.6 & YSOc\_star$+$dust(MP1) &  3.0 &   $-$2.02 &       2100 &       17 &   $-$2.14 &       2400 &       29 & N &    G \\
  96 &     Lup & J161125.99$-$391123.2 & YSOc\_star$+$dust(MP1) &  6.0 &   $-$2.16 &       2000 &       3.4 &   $-$2.33 &       2700 &       10 & N &    G \\
  97 &     Lup & J161131.93$-$381110.4 & YSOc\_star$+$dust(MP1) &  2.0 &   $-$2.29 &       2400 &       0.089 &   $-$2.28 &       2900 &       0.14 & N &    G \\
  98 &     Lup & J161144.86$-$383244.7 & YSOc\_star$+$dust(MP1) &  3.0 &   $-$2.28 &       2600 &       0.056 &   $-$2.11 &       3800 &       0.14 & N &    G \\
  99 &     Lup & J161148.67$-$381758.3 & YSOc\_star$+$dust(IR1) &  1.0 &   $-$0.68 &       2500 &       0.039 &   $-$0.62 &       3200 &       0.053 & N &    G \\
 100 &     Lup & J161159.81$-$382338.5 & YSOc\_star$+$dust(IR2) &  0.0 &   $-$1.03 & $\geq$2400 & $\geq$0.081 &   $-$1.03 & $\geq$2400 & $\geq$0.081 & N & L\_II \\
 101 &     Lup & J161200.06$-$385556.9 & YSOc\_star$+$dust(MP1) &  2.0 &   $-$2.34 &       2100 &       2.5 &   $-$2.37 &       2400 &       3.5 & N &    G \\
 102 &     Lup & J161204.48$-$380959.0 & YSOc\_star$+$dust(IR1) &  2.9 &   $-$0.01 &       1000 &       0.0066 &   $-$0.04 &       1500 &       0.011 & N &    G \\
 103 &     Lup & J161211.22$-$383219.8 & YSOc\_star$+$dust(IR3) &  6.0 &   $-$0.75 &       1700 &       0.24 &   $-$1.17 &       4300 &       0.98 & N &    G \\
 104 &     Lup & J161219.60$-$383742.2 & YSOc\_star$+$dust(MP1) &  4.0 &   $-$2.25 &       2200 &       2.1 &   $-$2.38 &       2900 &       5.0 & N &    G \\
 105 &     Lup & J161243.75$-$381503.3 & YSOc\_star$+$dust(IR1) &  0.0 &   $-$1.07 & $\geq$2800 & $\geq$0.48 &   $-$1.07 & $\geq$2800 & $\geq$0.48 & N & L\_II \\
 106 &     Lup & J161251.72$-$384215.9 & YSOc\_star$+$dust(MP1) &  1.0 &   $-$2.15 &       2200 &       2.9 &   $-$2.14 &       2300 &       3.5 & N &    G \\
 107 &     Lup & J161255.96$-$375643.8 & YSOc\_star$+$dust(MP1) &  3.0 &   $-$2.25 &       2100 &       5.2 &   $-$2.34 &       2500 &       9.1 & N &    G \\
 108 &     Lup & J161340.95$-$383723.7 & YSOc\_star$+$dust(MP1) &  5.0 &   $-$2.45 &       2300 &       2.2 &   $-$2.59 &       4100 &       8.8 & N &    G \\
 109 &     Lup & J155945.28$-$415457.2 & YSOc\_star$+$dust(IR4) &  2.0 &   $-$1.43 &       2000 &       1.1 &   $-$1.50 &       2400 &       1.7 & N &    G \\
 110 &     Lup & J160007.43$-$414948.9 & YSOc\_star$+$dust(IR2) &  6.0 &   $-$1.41 &       1800 &       3.5 &   $-$1.44 &       2300 &       9.1 & N &    G \\
 111 &     Lup & J160026.13$-$415355.6 & YSOc\_star$+$dust(IR3) &  3.0 &   $-$1.12 &       2500 &       0.065 &   $-$1.17 &       3800 &       0.17 & N &    G \\
 112 &     Lup & J160031.05$-$414337.2 & YSOc\_star$+$dust(IR2) &  0.0 &   $-$0.80 & $\geq$2400 & $\geq$0.21 &   $-$0.80 & $\geq$2400 & $\geq$0.21 & N & L\_II \\
 113 &     Lup & J160044.53$-$415531.2 & YSOc\_star$+$dust(IR3) &  0.0 &   $-$0.62 & $\geq$2700 & $\geq$0.93 &   $-$0.62 & $\geq$2700 & $\geq$0.93 & N & L\_II \\
 114 &     Lup & J160111.55$-$413730.1 & YSOc\_star$+$dust(MP1) &  3.0 &   $-$2.28 &       2300 &       0.24 &   $-$2.37 &       2900 &       0.47 & N &    G \\
 115 &     Lup & J160115.55$-$415235.3 &            YSOc\_red &  2.9 &   $-$0.19 &        130 &       0.11 &   $-$0.36 &        170 &       0.12 & N &    G \\
 116 &     Lup & J160129.69$-$420803.6 & YSOc\_star$+$dust(MP1) &  4.0 &   $-$1.92 &       2200 &       0.21 &   $-$2.01 &       3200 &       0.53 & N &    G \\
 117 &     Lup & J160143.28$-$413605.7 & YSOc\_star$+$dust(MP1) &  3.0 &   $-$2.33 &       2300 &       0.33 &   $-$2.40 &       3000 &       0.67 & N &    G \\
 118 &     Lup & J160157.04$-$414243.9 & YSOc\_star$+$dust(MP1) &  6.0 &   $-$2.17 &       2000 &       6.3 &   $-$2.25 &       2800 &       20 & N &    G \\
 119 &     Lup & J160221.61$-$414053.7 &         YSOc\_PAH$-$em &  2.9 &    0.92 &        360 &       0.060 &    0.56 &       1400 &       0.087 & N &    G \\
 120 &     Lup & J160229.91$-$415111.1 & YSOc\_star$+$dust(MP1) &  6.0 &   $-$2.17 &       2100 &       0.11 &   $-$2.35 &       3000 &       0.38 & N &    G \\
 121 &     Per & J032519.52$+$303424.2 &                YSOc &  5.9 &   $-$0.08 &        750 &       0.0099 &   $-$0.11 &        960 &       0.023 & N &    G \\
 122 &     Per & J032522.32$+$304513.9 &            YSOc\_red &  5.9 &    2.34 &         68 &       1.9 &    2.31 &         74 &       2.3 & Y &    G \\
 123 &     Per & J032536.22$+$304515.7 &                 red &  5.9 &    1.59 &        190 &       0.050 &    1.57 &        200 &       0.093 & N &    G \\
 124 &     Per & J032536.49$+$304522.2 &            YSOc\_red &  5.9 &    2.62 &         59 &       10 &    2.89 &         73 &       12 & Y &    G \\
 125 &     Per & J032538.83$+$304406.2 &            YSOc\_red &  5.9 &    2.16 &         69 &       4.4 &    2.12 &         77 &       5.3 & Y &    G \\
 126 &     Per & J032539.12$+$304358.2 &            YSOc\_red &  5.9 &    2.36 & $\leq$160 & $\geq$0.68 &    2.19 & $\leq$190 & $\geq$1.1 & Y &  L\_I \\
 127 &     Per & J032637.47$+$301528.1 &            YSOc\_red &  5.9 &    1.09 &         69 &       1.0 &    0.99 &         92 &       1.2 & Y &    G \\
 128 &     Per & J032738.25$+$301358.6 & YSOc\_star$+$dust(IR4) &  5.9 &   $-$0.19 &        270 &       0.77 &   $-$0.51 &        480 &       1.1 & Y &    G \\
 129 &     Per & J032738.83$+$301257.9 &            YSOc\_red &  5.9 &    0.95 &        180 &       0.021 &    1.02 &        190 &       0.039 & N &    G \\
 130 &     Per & J032739.08$+$301303.1 &            YSOc\_red &  5.9 &    2.68 &         59 &       8.1 &    2.55 &         66 &       9.4 & Y &    G \\
 131 &     Per & J032741.47$+$302016.8 & YSOc\_star$+$dust(IR2) &  3.0 &   $-$0.85 &       1500 &       0.31 &   $-$0.89 &       3100 &       0.82 & N &    G \\
 132 &     Per & J032743.23$+$301228.9 &            YSOc\_red &  5.9 &    2.39 &         61 &       1.7 &    2.34 &         75 &       2.0 & Y &    G \\
 133 &     Per & J032747.67$+$301204.5 & YSOc\_star$+$dust(IR1) &  5.9 &   $-$0.09 &        790 &       2.3 &   $-$0.29 &       1100 &       5.6 & N &    G \\
 134 &     Per & J032800.09$+$300847.0 & YSOc\_star$+$dust(IR2) &  4.8 &   $-$0.95 &       1400 &       0.20 &   $-$0.94 &       3100 &       0.65 & N &    G \\
 135 &     Per & J032800.39$+$300801.3 &            YSOc\_red &  5.9 &    0.95 &        220 &       0.30 &    0.98 &        290 &       0.49 & Y &    G \\
 136 &     Per & J032832.56$+$311105.1 &            YSOc\_red &  5.9 &    0.78 &         70 &       0.18 &    0.54 &        140 &       0.21 & Y &    G \\
 137 &     Per & J032834.49$+$310051.1 & YSOc\_star$+$dust(IR1) &  5.9 &    0.83 &        210 &       1.3 &    0.89 &        310 &       2.1 & Y &    G \\
 138 &     Per & J032834.53$+$310705.5 &                YSOc &  5.9 &    0.54 &        150 &       0.13 &    0.45 &        220 &       0.17 & Y &    G \\
 139 &     Per & J032834.94$+$305454.5 &                YSOc &  5.9 &    0.06 &        660 &       0.0087 &    0.01 &        820 &       0.020 & N &    G \\
 140 &     Per & J032835.03$+$302009.9 & YSOc\_star$+$dust(IR4) &  5.9 &    0.15 &        340 &       0.040 &   $-$0.29 &        730 &       0.072 & Y &    G \\
 141 &     Per & J032837.09$+$311330.8 &            YSOc\_red &  5.9 &    2.35 &        100 &       8.8 &    1.64 &        130 &       12 & Y &    G \\
 142 &     Per & J032838.78$+$311806.6 & YSOc\_star$+$dust(IR2) &  5.9 &   $-$0.18 &        730 &       0.017 &   $-$0.21 &        840 &       0.039 & N &    G \\
 143 &     Per & J032839.10$+$310601.7 &            YSOc\_red &  5.9 &    1.68 &         29 &       0.22 &    1.66 &         34 &       0.23 & Y &    G \\
 144 &     Per & J032839.71$+$311731.9 &            YSOc\_red &  5.9 &    0.57 &        240 &       0.19 &    0.63 &        330 &       0.30 & Y &    G \\
 145 &     Per & J032840.63$+$311756.5 &                 red &  5.9 &    1.02 &        280 &       0.0018 &    1.07 &        290 &       0.0036 & N &    G \\
 146 &     Per & J032842.41$+$302953.2 & YSOc\_star$+$dust(IR2) &  1.5 &   $-$0.89 &       1600 &       0.16 &   $-$0.96 &       3200 &       0.36 & N &    G \\
 147 &     Per & J032843.24$+$311042.7 & YSOc\_star$+$dust(IR4) & 13.5 &   $-$1.47 &       1400 &       0.031 &   $-$1.81 &       3300 &       0.29 & N &    G \\
 148 &     Per & J032843.28$+$311732.9 & YSOc\_star$+$dust(IR1) &  5.9 &    0.36 &        440 &       1.9 &    0.33 &        610 &       4.0 & Y &    G \\
 149 &     Per & J032844.09$+$312052.7 & YSOc\_star$+$dust(IR2) &  4.4 &   $-$1.12 &       1600 &       0.021 &   $-$1.24 &       3300 &       0.072 & N &    G \\
 150 &     Per & J032845.30$+$310541.9 &            YSOc\_red &  5.9 &    1.11 &         62 &       0.46 &    1.18 &         90 &       0.54 & Y &    G \\
 151 &     Per & J032846.21$+$311638.4 & YSOc\_star$+$dust(IR3) &  2.1 &   $-$1.65 &       1900 &       0.30 &   $-$1.78 &       3400 &       0.83 & N &    G \\
 152 &     Per & J032847.65$+$312406.0 & YSOc\_star$+$dust(IR1) &  9.3 &   $-$1.10 &       1300 &       0.058 &   $-$1.29 &       3200 &       0.29 & N &    G \\
 153 &     Per & J032847.84$+$311655.1 & YSOc\_star$+$dust(IR2) &  6.6 &   $-$0.81 &       1300 &       0.11 &   $-$0.99 &       3100 &       0.45 & N &    G \\
 154 &     Per & J032848.77$+$311608.8 &            YSOc\_red &  5.9 &    0.33 &        490 &       0.013 &    0.25 &        690 &       0.023 & N &    G \\
 155 &     Per & J032850.62$+$304244.7 & YSOc\_star$+$dust(IR1) &  5.9 &   $-$0.17 &        660 &       0.051 &   $-$0.40 &        960 &       0.12 & N &    G \\
 156 &     Per & J032851.03$+$311818.5 & YSOc\_star$+$dust(IR2) &  7.3 &   $-$0.62 &       1300 &       0.59 &   $-$0.84 &       3100 &       2.4 & N &    G \\
 157 &     Per & J032851.08$+$311632.4 & YSOc\_star$+$dust(IR2) &  2.0 &   $-$1.26 &       1800 &       0.033 &   $-$1.37 &       3300 &       0.089 & N &    G \\
 158 &     Per & J032851.20$+$311954.8 & YSOc\_star$+$dust(IR2) &  5.4 &   $-$0.63 &       1400 &       0.29 &   $-$0.85 &       3200 &       1.0 & N &    G \\
 159 &     Per & J032851.26$+$311739.3 & YSOc\_star$+$dust(IR2) &  5.9 &    0.78 &        660 &       0.011 &    0.62 &       1000 &       0.028 & N &    G \\
 160 &     Per & J032852.15$+$311547.1 & YSOc\_star$+$dust(IR2) &  1.8 &   $-$1.21 &       1700 &       0.039 &   $-$1.31 &       3300 &       0.098 & N &    G \\
 161 &     Per & J032852.17$+$304505.5 & YSOc\_star$+$dust(IR1) &  3.6 &   $-$0.69 &       1300 &       1.0 &   $-$0.90 &       2900 &       2.6 & N &    G \\
 162 &     Per & J032852.17$+$312245.3 & YSOc\_star$+$dust(IR3) &  3.3 &   $-$1.16 &       1700 &       0.13 &   $-$1.26 &       3400 &       0.42 & N &    G \\
 163 &     Per & J032852.92$+$311626.4 & YSOc\_star$+$dust(IR2) &  1.9 &   $-$1.28 &       1800 &       0.024 &   $-$1.33 &       3300 &       0.063 & N &    G \\
 164 &     Per & J032853.96$+$311809.3 & YSOc\_star$+$dust(IR3) & 16.7 &   $-$0.54 &        860 &       0.14 &   $-$1.01 &       3200 &       1.2 & N &    G \\
 165 &     Per & J032854.09$+$311654.2 & YSOc\_star$+$dust(IR3) &  3.4 &   $-$0.80 &       1600 &       0.060 &   $-$0.90 &       3200 &       0.17 & N &    G \\
 166 &     Per & J032854.63$+$311651.1 & YSOc\_star$+$dust(IR2) &  9.7 &   $-$0.68 &       1200 &       0.21 &   $-$0.98 &       3200 &       1.1 & N &    G \\
 167 &     Per & J032855.08$+$311628.7 & YSOc\_star$+$dust(IR1) & 11.2 &   $-$0.50 &        980 &       0.23 &   $-$0.71 &       2800 &       0.99 & N &    G \\
 168 &     Per & J032855.55$+$311436.7 &              rising &  5.9 &    3.03 &         57 &       67 &    2.71 &         57 &       76 & Y &    G \\
 169 &     Per & J032856.12$+$311908.4 &                YSOc &  0.0 &   $-$0.36 & $\geq$560 & $\geq$0.038 &   $-$0.36 & $\geq$560 & $\geq$0.037 & N & L\_II \\
 170 &     Per & J032856.32$+$312227.9 & YSOc\_star$+$dust(IR2) &  5.9 &   $-$0.14 &        440 &       0.16 &   $-$0.45 &        740 &       0.28 & Y &    G \\
 171 &     Per & J032856.60$+$310737.0 &            YSOc\_red &  5.9 &    0.12 &        160 &       0.014 &    0.03 &        200 &       0.020 & N &    G \\
 172 &     Per & J032856.65$+$311835.5 & YSOc\_star$+$dust(IR2) &  9.6 &   $-$0.78 &       1100 &       0.39 &   $-$0.92 &       3100 &       1.8 & N &    G \\
 173 &     Per & J032856.97$+$311622.3 & YSOc\_star$+$dust(IR4) &  5.9 &   $-$0.22 &       1000 &       0.12 &   $-$0.78 &       1400 &       0.33 & N &    G \\
 174 &     Per & J032857.18$+$311534.6 & YSOc\_star$+$dust(IR2) &  7.5 &   $-$0.35 &       1200 &       0.016 &   $-$0.62 &       3000 &       0.063 & N &    G \\
 175 &     Per & J032857.21$+$311419.1 & YSOc\_star$+$dust(MP1) &  0.0 &   $-$1.82 & $\geq$2000 & $\geq$2.2 &   $-$1.82 & $\geq$2000 & $\geq$2.2 & N & L\_II \\
 176 &     Per & J032857.36$+$311415.9 &            YSOc\_red &  5.9 &    1.60 &         85 &       8.0 &    1.48 &        100 &       10 & Y &    G \\
 177 &     Per & J032857.70$+$311948.1 & YSOc\_star$+$dust(IR2) &  4.6 &   $-$0.61 &       1400 &       0.076 &   $-$0.79 &       3100 &       0.24 & N &    G \\
 178 &     Per & J032858.11$+$311803.7 & YSOc\_star$+$dust(MP1) &  3.6 &   $-$2.16 &       1900 &       0.059 &   $-$2.23 &       3500 &       0.21 & N &    G \\
 179 &     Per & J032858.26$+$312209.2 & YSOc\_star$+$dust(IR2) &  9.8 &   $-$0.49 &        830 &       0.019 &   $-$0.25 &       2800 &       0.070 & N &    G \\
 180 &     Per & J032858.27$+$312202.0 & YSOc\_star$+$dust(IR1) &  9.1 &   $-$0.66 &       1200 &       0.030 &   $-$0.96 &       3100 &       0.14 & N &    G \\
 181 &     Per & J032858.43$+$312217.5 &            YSOc\_red &  5.9 &    0.83 &        320 &       0.63 &    0.76 &        390 &       1.1 & Y &    G \\
 182 &     Per & J032859.23$+$312032.5 & YSOc\_star$+$dust(IR1) &  5.9 &    0.13 &        790 &       0.0056 &   $-$0.08 &       1200 &       0.014 & N &    G \\
 183 &     Per & J032859.32$+$311548.7 & YSOc\_star$+$dust(IR4) &  5.9 &    0.06 &        620 &       0.48 &   $-$0.12 &        750 &       1.1 & N &    G \\
 184 &     Per & J032859.56$+$312146.7 & YSOc\_star$+$dust(IR1) &  8.0 &   $-$0.83 &       1200 &       0.24 &   $-$1.01 &       3000 &       0.94 & N &    G \\
 185 &     Per & J032900.55$+$311200.8 &                 red &  5.9 &    2.16 &         30 &       0.67 &    2.07 &         32 &       0.70 & Y &    G \\
 186 &     Per & J032901.56$+$312020.6 &              rising &  5.9 &    2.09 &        190 &       11 &    2.29 &        280 &       15 & Y &    G \\
 187 &     Per & J032901.88$+$311653.2 & YSOc\_star$+$dust(IR2) &  5.9 &    0.12 &        520 &       0.010 &   $-$0.27 &        860 &       0.022 & N &    G \\
 188 &     Per & J032902.81$+$312217.2 & YSOc\_star$+$dust(IR2) & 14.9 &   $-$0.71 &       1100 &       0.013 &   $-$1.22 &       3200 &       0.100 & N &    G \\
 189 &     Per & J032903.15$+$312238.0 & YSOc\_star$+$dust(IR1) &  8.5 &   $-$0.36 &       1100 &       0.096 &   $-$0.62 &       3000 &       0.39 & N &    G \\
 190 &     Per & J032903.22$+$312545.1 & YSOc\_star$+$dust(IR2) &  6.2 &   $-$0.51 &       1200 &       0.0086 &   $-$0.59 &       3000 &       0.030 & N &    G \\
 191 &     Per & J032903.33$+$312314.6 &            YSOc\_red &  5.9 &    1.13 & $\leq$310 & $\geq$0.090 &    1.01 & $\leq$390 & $\geq$0.18 & Y &  L\_I \\
 192 &     Per & J032903.78$+$311603.8 &              rising &  5.9 &    1.21 &        170 &       38 &    1.02 &        250 &       59 & Y &    G \\
 193 &     Per & J032903.87$+$305629.8 & YSOc\_star$+$dust(IR2) &  5.9 &   $-$0.17 &       1100 &       0.0074 &   $-$0.43 &       1600 &       0.023 & N &    G \\
 194 &     Per & J032903.87$+$312148.6 & YSOc\_star$+$dust(IR1) &  8.1 &   $-$0.74 &       1200 &       0.58 &   $-$0.97 &       3100 &       2.5 & N &    G \\
 195 &     Per & J032904.06$+$311446.5 &            YSOc\_red &  5.9 &    1.43 & $\leq$37 & $\geq$0.14 &    1.41 & $\leq$59 & $\geq$0.16 & Y &  L\_I \\
 196 &     Per & J032904.12$+$305612.8 & YSOc\_star$+$dust(IR2) &  1.5 &   $-$0.79 &       1600 &       0.021 &   $-$0.76 &       3200 &       0.047 & N &    G \\
 197 &     Per & J032904.64$+$312205.7 &                red1 &  0.0 & ... &       ... &       ... & ... &       ... &       ... & N &  O \\
 198 &     Per & J032904.68$+$311659.0 &                YSOc &  5.9 &   $-$0.23 &        920 &       0.034 &   $-$0.52 &       1200 &       0.088 & N &    G \\
 199 &     Per & J032904.73$+$311134.9 &                YSOc & 17.2 &   $-$0.32 &        770 &       0.015 &   $-$0.70 &       2100 &       0.066 & N &    G \\
 200 &     Per & J032904.95$+$312038.4 & YSOc\_star$+$dust(IR2) &  5.9 &    0.22 &        610 &       0.052 &    0.08 &        810 &       0.12 & N &    G \\
 201 &     Per & J032905.18$+$312036.9 &            YSOc\_red &  5.9 &    0.34 &       1000 &       0.023 &   $-$1.08 &       1300 &       0.064 & N &    G \\
 202 &     Per & J032905.78$+$311639.6 & YSOc\_star$+$dust(IR1) & 19.9 &   $-$0.50 &        910 &       0.44 &   $-$1.08 &       3000 &       4.1 & N &    G \\
 203 &     Per & J032906.05$+$303039.2 &            YSOc\_red &  5.9 &    0.87 &        300 &       0.020 &    0.72 &        560 &       0.035 & N &    G \\
 204 &     Per & J032906.33$+$311346.4 & YSOc\_star$+$dust(IR3) & 24.2 &   $-$0.39 &        840 &       0.038 &   $-$1.08 &       2800 &       0.42 & N &    G \\
 205 &     Per & J032907.78$+$312157.3 &              rising &  5.9 &    2.18 &        150 &       21 &    2.19 &        210 &       27 & Y &    G \\
 206 &     Per & J032907.96$+$312251.4 & YSOc\_star$+$dust(IR2) & 10.7 &   $-$0.66 &       1200 &       0.24 &   $-$1.12 &       3100 &       1.3 & N &    G \\
 207 &     Per & J032908.97$+$312256.1 &                YSOc &  5.9 &   $-$0.05 &        770 &       0.12 &   $-$0.37 &        930 &       0.27 & N &    G \\
 208 &     Per & J032909.10$+$312305.5 &         YSOc\_PAH$-$em &  5.9 &    0.12 &        670 &       0.11 &   $-$0.48 &        920 &       0.27 & N &    G \\
 209 &     Per & J032909.10$+$312128.7 &                YSOc &  5.9 &    0.88 &        500 &       0.23 &    1.01 &        560 &       0.47 & N &    G \\
 210 &     Per & J032909.34$+$312104.1 & YSOc\_star$+$dust(IR3) &  5.9 &   $-$0.12 &        840 &       0.022 &   $-$0.58 &       1100 &       0.056 & N &    G \\
 211 &     Per & J032909.40$+$311413.8 &                YSOc &  0.0 &   $-$0.68 & $\geq$620 & $\geq$0.0084 &   $-$0.68 & $\geq$620 & $\geq$0.0084 & N & L\_II \\
 212 &     Per & J032909.49$+$312720.9 & YSOc\_star$+$dust(IR2) &  3.6 &   $-$0.83 &       1500 &       0.022 &   $-$0.96 &       3200 &       0.064 & N &    G \\
 213 &     Per & J032909.65$+$312256.3 & YSOc\_star$+$dust(IR4) &  5.0 &   $-$1.26 &       1600 &       0.35 &   $-$1.04 &       3300 &       1.3 & N &    G \\
 214 &     Per & J032910.47$+$312334.7 & YSOc\_star$+$dust(IR2) & 11.0 &   $-$0.85 &       1200 &       0.020 &   $-$1.04 &       3200 &       0.12 & N &    G \\
 215 &     Per & J032910.49$+$311331.0 &                 red &  5.9 &    2.58 &         41 &       5.4 &    2.55 &         43 &       5.8 & Y &    G \\
 216 &     Per & J032910.65$+$311340.0 &            YSOc\_red &  5.9 &    0.74 &        340 &       0.0017 &    0.46 &        350 &       0.0033 & N &    G \\
 217 &     Per & J032910.68$+$311820.6 &            YSOc\_red &  5.9 &    1.95 &         63 &       2.8 &    1.90 &         70 &       3.3 & Y &    G \\
 218 &     Per & J032910.84$+$311642.6 & YSOc\_star$+$dust(IR1) &  5.9 &   $-$0.13 &        900 &       0.028 &   $-$0.34 &       1200 &       0.073 & N &    G \\
 219 &     Per & J032910.99$+$311826.0 &            YSOc\_red &  5.9 &    0.69 &        230 &       0.010 &    0.60 &        230 &       0.019 & N &    G \\
 220 &     Per & J032911.26$+$311831.4 &            YSOc\_red &  5.9 &    1.94 & $\leq$76 & $\geq$0.44 &    1.86 & $\leq$100 & $\geq$0.60 & Y &  L\_I \\
 221 &     Per & J032911.89$+$312127.0 &                YSOc &  5.9 &    0.34 &        700 &       0.061 &    0.24 &        780 &       0.14 & N &    G \\
 222 &     Per & J032912.06$+$311305.4 &            YSOc\_red &  5.9 &    0.98 &         55 &       0.99 &    0.87 &         55 &       1.1 & N &    G \\
 223 &     Per & J032912.06$+$311301.7 &            YSOc\_red &  5.9 &    0.55 & $\leq$13 & $\geq$2.7 &    0.17 & $\leq$16 & $\geq$2.7 & Y &  L\_I \\
 224 &     Per & J032912.97$+$311814.3 &                YSOc &  5.9 &    1.05 &        240 &       1.1 &    1.56 &        300 &       1.7 & Y &    G \\
 225 &     Per & J032913.14$+$312252.8 & YSOc\_star$+$dust(IR2) & 10.4 &   $-$1.05 &       1300 &       0.24 &   $-$1.35 &       3200 &       1.3 & N &    G \\
 226 &     Per & J032913.54$+$311358.2 &                 red &  5.9 &    2.41 &         37 &       0.80 &    2.41 &         39 &       0.86 & Y &    G \\
 227 &     Per & J032914.40$+$311444.1 &                YSOc & 13.9 &   $-$0.32 &        820 &       0.010 &   $-$0.71 &       2400 &       0.043 & N &    G \\
 228 &     Per & J032916.61$+$312349.4 & YSOc\_star$+$dust(IR2) &  6.8 &   $-$0.85 &       1400 &       0.089 &   $-$1.25 &       3200 &       0.36 & N &    G \\
 229 &     Per & J032916.69$+$311618.2 & YSOc\_star$+$dust(MP1) &  1.2 &   $-$2.40 &       2000 &       0.14 &   $-$2.37 &       3500 &       0.37 & N &    G \\
 230 &     Per & J032916.83$+$312325.1 & YSOc\_star$+$dust(IR2) &  5.9 &   $-$0.14 &       1000 &       0.014 &   $-$0.60 &       1400 &       0.040 & N &    G \\
 231 &     Per & J032917.17$+$312746.5 &            YSOc\_red &  5.9 &    1.75 &         49 &       0.40 &    1.76 &         58 &       0.46 & Y &    G \\
 232 &     Per & J032917.50$+$312748.3 &            YSOc\_red &  5.9 &    1.01 &        230 &       0.0020 &    0.95 &        240 &       0.0030 & N &    G \\
 233 &     Per & J032917.68$+$312245.0 & YSOc\_star$+$dust(IR1) &  4.6 &   $-$0.77 &       1400 &       1.4 &   $-$0.92 &       3000 &       4.2 & N &    G \\
 234 &     Per & J032917.78$+$311948.0 & YSOc\_star$+$dust(IR2) &  5.4 &   $-$0.97 &       1500 &       0.016 &   $-$1.10 &       3200 &       0.058 & N &    G \\
 235 &     Per & J032918.26$+$312319.9 &            YSOc\_red &  5.9 &    1.26 & $\leq$100 & $\geq$0.070 &    1.22 & $\leq$150 & $\geq$0.098 & Y &  L\_I \\
 236 &     Per & J032918.67$+$312017.7 & YSOc\_star$+$dust(IR2) &  5.9 &    0.39 &        590 &       0.0090 &    0.17 &        830 &       0.021 & N &    G \\
 237 &     Per & J032918.74$+$312325.4 & YSOc\_star$+$dust(IR2) &  5.9 &   $-$0.23 &       1300 &       0.26 &   $-$0.70 &       1800 &       0.89 & N &    G \\
 238 &     Per & J032920.06$+$312407.5 & YSOc\_star$+$dust(IR2) &  5.9 &    0.42 & $\leq$360 & $\geq$0.28 &    0.27 & $\leq$460 & $\geq$0.53 & Y &  L\_I \\
 239 &     Per & J032920.44$+$311834.2 & YSOc\_star$+$dust(IR1) &  5.9 &   $-$0.14 &        680 &       0.41 &   $-$0.30 &        870 &       0.93 & N &    G \\
 240 &     Per & J032921.57$+$312110.3 & YSOc\_star$+$dust(IR2) &  1.2 &   $-$1.03 &       1800 &       0.070 &   $-$1.05 &       3300 &       0.17 & N &    G \\
 241 &     Per & J032921.87$+$311536.2 & YSOc\_star$+$dust(IR2) &  4.6 &   $-$1.13 &       1500 &       0.38 &   $-$1.23 &       3200 &       1.3 & N &    G \\
 242 &     Per & J032923.17$+$312030.2 & YSOc\_star$+$dust(IR2) &  2.0 &   $-$0.83 &       1600 &       0.088 &   $-$0.88 &       3200 &       0.22 & N &    G \\
 243 &     Per & J032923.25$+$312653.1 & YSOc\_star$+$dust(IR2) &  3.0 &   $-$1.02 &       1600 &       0.034 &   $-$1.14 &       3200 &       0.093 & N &    G \\
 244 &     Per & J032923.48$+$313329.5 &            YSOc\_red &  5.9 &    1.51 &         61 &       0.36 &    1.61 &         76 &       0.43 & Y &    G \\
 245 &     Per & J032924.09$+$311957.6 & YSOc\_star$+$dust(IR2) &  5.9 &    0.36 &        630 &       0.025 &   $-$0.15 &        100 &       0.061 & N &    G \\
 246 &     Per & J032925.93$+$312640.1 &                YSOc &  3.7 &   $-$0.60 &       1400 &       0.46 &   $-$0.78 &       2700 &       1.1 & N &    G \\
 247 &     Per & J032926.81$+$312647.6 & YSOc\_star$+$dust(MP1) &  1.9 &   $-$1.72 &       1900 &       0.29 &   $-$1.69 &       3400 &       0.81 & N &    G \\
 248 &     Per & J032928.88$+$305841.9 & YSOc\_star$+$dust(IR2) &  0.8 &   $-$0.64 &       1700 &       0.041 &   $-$0.76 &       3300 &       0.093 & N &    G \\
 249 &     Per & J032929.27$+$311834.7 & YSOc\_star$+$dust(IR4) &  4.4 &   $-$0.66 &       1200 &       0.14 &   $-$0.56 &       2900 &       0.37 & N &    G \\
 250 &     Per & J032929.80$+$312102.6 & YSOc\_star$+$dust(IR3) &  3.7 &   $-$0.77 &       1600 &       0.084 &   $-$0.93 &       3300 &       0.26 & N &    G \\
 251 &     Per & J032930.40$+$311903.3 & YSOc\_star$+$dust(IR2) &  1.6 &   $-$0.86 &       1500 &       0.11 &   $-$0.94 &       3100 &       0.26 & N &    G \\
 252 &     Per & J032932.57$+$312436.9 & YSOc\_star$+$dust(IR1) &  6.7 &   $-$1.05 &       1400 &       0.060 &   $-$1.16 &       3200 &       0.24 & N &    G \\
 253 &     Per & J032932.88$+$312712.6 & YSOc\_star$+$dust(IR2) &  1.5 &   $-$1.48 &       1800 &       0.030 &   $-$1.51 &       3300 &       0.074 & N &    G \\
 254 &     Per & J032937.73$+$312202.5 & YSOc\_star$+$dust(IR2) &  1.3 &   $-$0.81 &       1600 &       0.018 &   $-$0.77 &       3200 &       0.041 & N &    G \\
 255 &     Per & J032944.16$+$311947.3 &                YSOc &  6.9 &   $-$0.63 &        990 &       0.0039 &   $-$0.78 &       2500 &       0.011 & N &    G \\
 256 &     Per & J032946.00$+$310439.0 & YSOc\_star$+$dust(IR4) &  0.0 &   $-$0.98 & $\geq$470 & $\geq$0.052 &   $-$0.98 & $\geq$470 & $\geq$0.052 & N & L\_II \\
 257 &     Per & J032951.82$+$313906.0 &                 red &  5.9 &    3.44 &         38 &       0.56 &    3.34 &         41 &       0.61 & Y &    G \\
 258 &     Per & J032954.04$+$312052.9 & YSOc\_star$+$dust(IR2) &  3.0 &   $-$0.52 &       1200 &       0.19 &   $-$0.58 &       2900 &       0.46 & N &    G \\
 259 &     Per & J033015.14$+$302349.4 &            YSOc\_red &  5.9 &    1.70 &         97 &       1.7 &    1.58 &        120 &       2.3 & Y &    G \\
 260 &     Per & J033022.45$+$313240.5 & YSOc\_star$+$dust(IR2) &  5.9 &    0.47 &        660 &       0.0095 &    0.35 &        990 &       0.023 & N &    G \\
 261 &     Per & J033024.08$+$311404.4 & YSOc\_star$+$dust(IR2) &  0.9 &   $-$1.02 &       1700 &       0.027 &   $-$1.07 &       3200 &       0.061 & N &    G \\
 262 &     Per & J033025.97$+$310217.9 & YSOc\_star$+$dust(MP1) &  1.8 &   $-$2.45 &       2000 &       0.40 &   $-$2.44 &       3500 &       1.1 & N &    G \\
 263 &     Per & J033027.14$+$302829.8 &            YSOc\_red &  5.9 &   $-$0.00 &        310 &       0.25 &   $-$0.21 &        510 &       0.45 & N &    G \\
 264 &     Per & J033032.68$+$302626.6 &            YSOc\_red &  5.9 &    2.08 &         36 &       0.16 &    1.94 &         43 &       0.17 & Y &    G \\
 265 &     Per & J033035.47$+$311558.6 & YSOc\_star$+$dust(IR3) &  5.9 &   $-$0.19 &        610 &       0.024 &   $-$0.68 &       1200 &       0.051 & N &    G \\
 266 &     Per & J033035.92$+$303024.4 & YSOc\_star$+$dust(IR1) &  3.2 &   $-$1.06 &       1500 &       2.5 &   $-$1.13 &       3200 &       6.9 & N &    G \\
 267 &     Per & J033036.97$+$303127.7 & YSOc\_star$+$dust(IR2) &  9.9 &   $-$0.54 &       1100 &       0.67 &   $-$0.92 &       3000 &       3.2 & N &    G \\
 268 &     Per & J033038.20$+$303211.9 & YSOc\_star$+$dust(IR2) &  5.9 &    0.35 &        300 &       0.042 &   $-$0.10 &        630 &       0.074 & N &    G \\
 269 &     Per & J033043.98$+$303247.0 & YSOc\_star$+$dust(IR1) &  5.8 &   $-$0.64 &       1200 &       1.3 &   $-$0.77 &       2900 &       4.1 & N &    G \\
 270 &     Per & J033052.51$+$305417.8 & YSOc\_star$+$dust(IR2) &  7.6 &   $-$0.44 &       1100 &       0.17 &   $-$0.69 &       2900 &       0.59 & N &    G \\
 271 &     Per & J033110.68$+$304940.6 & YSOc\_star$+$dust(IR2) &  2.4 &   $-$0.69 &       1400 &       0.16 &   $-$0.78 &       3000 &       0.37 & N &    G \\
 272 &     Per & J033114.70$+$304955.4 & YSOc\_star$+$dust(IR1) &  5.9 &    0.01 &        660 &       0.21 &   $-$0.09 &        930 &       0.48 & N &    G \\
 273 &     Per & J033118.30$+$304939.5 & YSOc\_star$+$dust(IR1) &  7.0 &   $-$0.68 &       1200 &       0.65 &   $-$0.90 &       3000 &       2.4 & N &    G \\
 274 &     Per & J033120.11$+$304917.7 & YSOc\_star$+$dust(IR1) &  2.7 &   $-$0.77 &       1400 &       0.035 &   $-$0.81 &       3000 &       0.087 & N &    G \\
 275 &     Per & J033120.98$+$304530.1 &            YSOc\_red &  5.9 &    0.98 &         35 &       1.1 &    1.10 &         37 &       1.2 & Y &    G \\
 276 &     Per & J033128.87$+$303053.3 & YSOc\_star$+$dust(IR1) &  1.8 &   $-$1.29 &       1600 &       0.92 &   $-$1.29 &       3200 &       2.2 & N &    G \\
 277 &     Per & J033131.17$+$304411.1 &                YSOc &  8.8 &   $-$1.14 &       1300 &       0.0060 &   $-$1.35 &       3000 &       0.031 & N &    G \\
 278 &     Per & J033142.40$+$310624.9 & YSOc\_star$+$dust(IR4) &  6.1 &   $-$1.27 &       1600 &       0.12 &   $-$1.35 &       3300 &       0.51 & N &    G \\
 279 &     Per & J033217.96$+$304947.5 &                 red &  5.9 &    1.07 &         28 &       1.2 &    0.81 &         29 &       1.3 & Y &    G \\
 280 &     Per & J033229.17$+$310240.8 & YSOc\_star$+$dust(IR1) &  5.9 &    0.40 &        110 &       0.57 &    0.08 &        220 &       0.70 & Y &    G \\
 281 &     Per & J033232.99$+$310221.7 & YSOc\_star$+$dust(IR1) &  6.5 &   $-$0.88 &       1300 &       0.21 &   $-$1.04 &       3100 &       0.82 & N &    G \\
 282 &     Per & J033234.05$+$310055.8 & YSOc\_star$+$dust(IR2) &  5.8 &   $-$0.66 &       1300 &       0.51 &   $-$0.75 &       3100 &       1.7 & N &    G \\
 283 &     Per & J033241.63$+$311044.2 &                YSOc &  0.0 &   $-$0.50 & $\geq$540 & $\geq$0.023 &   $-$0.50 & $\geq$540 & $\geq$0.020 & N & L\_II \\
 284 &     Per & J033241.70$+$311046.3 & YSOc\_star$+$dust(IR2) &  6.4 &   $-$0.37 &       1100 &       0.14 &   $-$0.55 &       2900 &       0.46 & N &    G \\
 285 &     Per & J033247.20$+$305916.3 & YSOc\_star$+$dust(IR2) & 20.7 &   $-$0.66 &        910 &       0.48 &   $-$1.26 &       3000 &       5.1 & N &    G \\
 286 &     Per & J033257.84$+$310608.3 &            YSOc\_red &  5.9 &    0.30 &        150 &       0.012 &    0.36 &        180 &       0.018 & N &    G \\
 287 &     Per & J033306.41$+$310804.6 & YSOc\_star$+$dust(IR1) &  5.9 &    0.34 &        490 &       0.058 &    0.13 &        670 &       0.12 & N &    G \\
 288 &     Per & J033309.56$+$310531.2 &         YSOc\_PAH$-$em &  5.9 &    1.13 &        190 &       0.050 &    0.72 &        360 &       0.077 & Y &    G \\
 289 &     Per & J033312.84$+$312124.2 & YSOc\_star$+$dust(IR1) &  5.9 &    0.41 &        450 &       3.1 &    0.25 &        640 &       6.3 & Y &    G \\
 290 &     Per & J033313.80$+$312005.3 &            YSOc\_red &  5.9 &    1.44 &         60 &       0.100 &    1.44 &         90 &       0.12 & Y &    G \\
 291 &     Per & J033314.38$+$310710.9 &            YSOc\_red &  5.9 &    2.22 &         36 &       0.63 &    2.33 &         43 &       0.68 & Y &    G \\
 292 &     Per & J033316.44$+$310652.5 &                 red &  5.9 &    1.73 &         24 &       1.1 &    1.63 &         25 &       1.1 & Y &    G \\
 293 &     Per & J033316.65$+$310755.2 &            YSOc\_red &  5.9 &    1.57 &         88 &       2.6 &    1.67 &        120 &       3.3 & Y &    G \\
 294 &     Per & J033317.85$+$310931.9 &            YSOc\_red &  5.9 &    3.33 &         76 &       1.8 &    3.11 &         94 &       2.2 & Y &    G \\
 295 &     Per & J033320.32$+$310721.5 &            YSOc\_red &  5.9 &    0.88 &        150 &       0.17 &    0.75 &        200 &       0.25 & Y &    G \\
 296 &     Per & J033327.29$+$310710.2 &            YSOc\_red &  5.9 &    1.93 &         78 &       1.7 &    1.91 &         95 &       2.2 & Y &    G \\
 297 &     Per & J033330.41$+$311050.6 & YSOc\_star$+$dust(IR1) &  6.9 &   $-$0.91 &       1200 &       2.8 &   $-$1.09 &       2900 &       9.8 & N &    G \\
 298 &     Per & J033341.29$+$311341.0 & YSOc\_star$+$dust(IR1) & 11.7 &   $-$0.57 &        910 &       0.19 &   $-$0.83 &       2900 &       0.89 & N &    G \\
 299 &     Per & J033346.92$+$305350.1 & YSOc\_star$+$dust(IR2) &  0.7 &   $-$1.04 &       1700 &       0.025 &   $-$1.01 &       3200 &       0.055 & N &    G \\
 300 &     Per & J033351.07$+$311227.8 & YSOc\_star$+$dust(MP1) &  2.8 &   $-$2.15 &       1900 &       0.19 &   $-$2.13 &       3400 &       0.58 & N &    G \\
 301 &     Per & J033401.66$+$311439.8 & YSOc\_star$+$dust(IR2) &  3.4 &   $-$0.92 &       1500 &       0.45 &   $-$1.09 &       3200 &       1.3 & N &    G \\
 302 &     Per & J033430.78$+$311324.4 & YSOc\_star$+$dust(IR2) &  3.2 &   $-$1.04 &       1600 &       0.061 &   $-$1.18 &       3200 &       0.18 & N &    G \\
 303 &     Per & J033449.84$+$311550.3 & YSOc\_star$+$dust(IR4) &  2.1 &   $-$1.38 &       1800 &       0.37 &   $-$1.36 &       3300 &       0.99 & N &    G \\
 304 &     Per & J033915.81$+$312430.7 & YSOc\_star$+$dust(IR2) &  8.7 &   $-$0.74 &       1300 &       0.048 &   $-$0.92 &       3100 &       0.23 & N &    G \\
 305 &     Per & J034001.49$+$311017.3 & YSOc\_star$+$dust(IR4) &  6.8 &   $-$1.34 &       1600 &       0.038 &   $-$1.45 &       3300 &       0.17 & N &    G \\
 306 &     Per & J034109.13$+$314437.9 & YSOc\_star$+$dust(IR1) &  8.0 &   $-$0.72 &        980 &       1.5 &   $-$0.84 &       2800 &       5.1 & N &    G \\
 307 &     Per & J034114.11$+$315946.3 & YSOc\_star$+$dust(MP1) &  0.0 &   $-$2.02 & $\geq$2100 & $\geq$0.39 &   $-$2.02 & $\geq$2100 & $\geq$0.39 & N & L\_II \\
 308 &     Per & J034119.19$+$320203.8 & YSOc\_star$+$dust(IR1) &  4.2 &   $-$1.35 &       1600 &       0.072 &   $-$1.44 &       3200 &       0.23 & N &    G \\
 309 &     Per & J034124.42$+$315327.9 & YSOc\_star$+$dust(IR1) & 11.3 &   $-$0.83 &       1100 &       0.0059 &   $-$1.11 &       3000 &       0.030 & N &    G \\
 310 &     Per & J034139.17$+$313610.7 & YSOc\_star$+$dust(IR4) &  0.0 &   $-$0.76 & $\geq$2000 & $\geq$0.53 &   $-$0.76 & $\geq$2000 & $\geq$0.53 & N & L\_II \\
 311 &     Per & J034141.09$+$314804.6 &                YSOc &  5.9 &   $-$0.11 &        700 &       0.012 &   $-$0.11 &        800 &       0.028 & N &    G \\
 312 &     Per & J034153.26$+$315019.2 & YSOc\_star$+$dust(IR1) &  5.9 &   $-$0.25 &        890 &       0.011 &   $-$0.38 &       1100 &       0.027 & N &    G \\
 313 &     Per & J034155.71$+$314811.4 & YSOc\_star$+$dust(IR1) &  5.9 &    0.25 &        490 &       0.11 &    0.27 &        650 &       0.22 & N &    G \\
 314 &     Per & J034157.44$+$314836.7 & YSOc\_star$+$dust(IR1) &  8.7 &   $-$1.01 &       1200 &       1.1 &   $-$1.25 &       3000 &       4.6 & N &    G \\
 315 &     Per & J034157.75$+$314800.8 & YSOc\_star$+$dust(IR2) &  8.8 &   $-$0.70 &       1300 &       0.22 &   $-$0.95 &       3200 &       1.1 & N &    G \\
 316 &     Per & J034158.67$+$314821.4 &            YSOc\_red &  5.9 &    0.59 &        510 &       0.017 &    0.54 &        660 &       0.036 & N &    G \\
 317 &     Per & J034201.01$+$314913.4 & YSOc\_star$+$dust(IR3) &  6.1 &   $-$1.18 &       1500 &       0.021 &   $-$1.30 &       3300 &       0.087 & N &    G \\
 318 &     Per & J034202.17$+$314802.1 &            YSOc\_red &  5.9 &    1.47 &        180 &       0.070 &    1.26 &        260 &       0.12 & Y &    G \\
 319 &     Per & J034204.34$+$314711.6 & YSOc\_star$+$dust(IR1) &  5.2 &   $-$0.78 &       1400 &       0.058 &   $-$0.94 &       3100 &       0.19 & N &    G \\
 320 &     Per & J034210.69$+$314705.6 & YSOc\_star$+$dust(IR3) & 17.3 &   $-$0.63 &        960 &       0.0070 &   $-$1.17 &       2500 &       0.042 & N &    G \\
 321 &     Per & J034219.27$+$314327.0 & YSOc\_star$+$dust(IR1) &  9.8 &   $-$0.57 &        970 &       0.17 &   $-$0.77 &       2900 &       0.69 & N &    G \\
 322 &     Per & J034220.32$+$320531.0 & YSOc\_star$+$dust(IR4) &  4.1 &   $-$1.00 &       1600 &       0.061 &   $-$1.06 &       3300 &       0.20 & N &    G \\
 323 &     Per & J034223.33$+$315742.7 & YSOc\_star$+$dust(IR4) &  0.0 &   $-$1.99 & $\geq$2100 & $\geq$0.40 &   $-$1.99 & $\geq$2100 & $\geq$0.40 & N & L\_II \\
 324 &     Per & J034227.12$+$314432.9 & YSOc\_star$+$dust(MP1) &  7.6 &   $-$0.93 &       1500 &       0.073 &   $-$0.91 &       3300 &       0.37 & N &    G \\
 325 &     Per & J034232.10$+$315249.5 & YSOc\_star$+$dust(IR2) &  5.2 &   $-$1.14 &       1600 &       0.0050 &   $-$1.29 &       3200 &       0.020 & N &    G \\
 326 &     Per & J034232.91$+$314220.6 & YSOc\_star$+$dust(IR2) &  5.4 &   $-$0.96 &       1500 &       0.12 &   $-$1.01 &       3200 &       0.43 & N &    G \\
 327 &     Per & J034233.13$+$315214.7 & YSOc\_star$+$dust(IR3) &  4.8 &   $-$0.82 &       1500 &       0.014 &   $-$0.84 &       3200 &       0.046 & N &    G \\
 328 &     Per & J034234.19$+$315101.0 & YSOc\_star$+$dust(IR4) &  3.7 &   $-$0.98 &       1600 &       0.015 &   $-$0.92 &       3300 &       0.048 & N &    G \\
 329 &     Per & J034236.47$+$315517.6 & YSOc\_star$+$dust(IR3) &  7.2 &   $-$0.90 &       1400 &       0.0080 &   $-$1.05 &       3200 &       0.034 & N &    G \\
 330 &     Per & J034244.50$+$315958.7 & YSOc\_star$+$dust(IR1) &  8.4 &   $-$1.23 &       1400 &       0.0051 &   $-$1.48 &       3200 &       0.025 & N &    G \\
 331 &     Per & J034249.18$+$315011.2 & YSOc\_star$+$dust(IR4) &  6.1 &   $-$1.27 &       1600 &       0.079 &   $-$1.42 &       3300 &       0.34 & N &    G \\
 332 &     Per & J034254.67$+$314345.3 & YSOc\_star$+$dust(MP1) &  1.2 &   $-$2.25 &       2000 &       0.15 &   $-$2.11 &       3500 &       0.38 & N &    G \\
 333 &     Per & J034255.95$+$315842.0 & YSOc\_star$+$dust(IR1) &  3.9 &   $-$0.98 &       1000 &       1.3 &   $-$1.18 &       2400 &       2.7 & N &    G \\
 334 &     Per & J034256.05$+$315644.8 &                YSOc &  5.9 &    0.15 &        640 &       0.014 &    0.16 &        720 &       0.032 & N &    G \\
 335 &     Per & J034301.94$+$314435.6 & YSOc\_star$+$dust(IR1) &  4.3 &   $-$0.95 &       1500 &       0.013 &   $-$1.11 &       3200 &       0.039 & N &    G \\
 336 &     Per & J034306.77$+$314820.5 & YSOc\_star$+$dust(MP1) &  3.7 &   $-$2.34 &       1900 &       0.100 &   $-$2.35 &       3500 &       0.36 & N &    G \\
 337 &     Per & J034313.70$+$320045.2 & YSOc\_star$+$dust(IR2) &  9.0 &   $-$0.68 &       1300 &       0.048 &   $-$1.01 &       3200 &       0.25 & N &    G \\
 338 &     Per & J034321.47$+$314246.3 & YSOc\_star$+$dust(IR3) &  7.3 &   $-$1.22 &       1500 &       0.016 &   $-$1.42 &       3300 &       0.070 & N &    G \\
 339 &     Per & J034322.22$+$314613.6 & YSOc\_star$+$dust(IR1) &  7.2 &   $-$0.89 &       1300 &       0.084 &   $-$1.05 &       3100 &       0.34 & N &    G \\
 340 &     Per & J034323.57$+$321225.9 & YSOc\_star$+$dust(IR3) &  3.0 &   $-$1.39 &       1700 &       0.019 &   $-$1.39 &       3300 &       0.057 & N &    G \\
 341 &     Per & J034325.48$+$315516.5 & YSOc\_star$+$dust(MP1) & 12.4 &   $-$1.06 &       1300 &       0.023 &   $-$1.16 &       3300 &       0.17 & N &    G \\
 342 &     Per & J034328.21$+$320159.1 & YSOc\_star$+$dust(IR2) &  4.5 &   $-$1.22 &       1600 &       0.21 &   $-$1.30 &       3300 &       0.73 & N &    G \\
 343 &     Per & J034328.46$+$320505.8 & YSOc\_star$+$dust(IR2) &  9.9 &   $-$0.77 &       1300 &       0.017 &   $-$1.03 &       3200 &       0.095 & N &    G \\
 344 &     Per & J034329.43$+$315219.5 & YSOc\_star$+$dust(IR1) &  5.9 &    0.79 &        400 &       0.11 &    0.42 &        620 &       0.21 & N &    G \\
 345 &     Per & J034336.02$+$315009.0 & YSOc\_star$+$dust(IR1) &  5.9 &    0.14 &        790 &       0.017 &   $-$0.20 &       1100 &       0.042 & N &    G \\
 346 &     Per & J034344.48$+$314309.3 & YSOc\_star$+$dust(IR2) &  5.9 &   $-$0.23 &        860 &       0.62 &   $-$0.54 &       1200 &       1.6 & N &    G \\
 347 &     Per & J034344.63$+$320817.8 & YSOc\_star$+$dust(IR4) &  2.5 &   $-$0.69 &       1300 &       0.15 &   $-$0.55 &       3000 &       0.36 & N &    G \\
 348 &     Per & J034345.17$+$320358.6 & YSOc\_star$+$dust(IR1) &  5.9 &   $-$0.22 &        540 &       0.69 &    0.05 &        710 &       1.4 & Y &    G \\
 349 &     Per & J034348.83$+$321551.5 & YSOc\_star$+$dust(IR2) &  2.3 &   $-$0.84 &       1600 &       0.052 &   $-$0.98 &       3200 &       0.13 & N &    G \\
 350 &     Per & J034350.96$+$320324.7 &            YSOc\_red &  5.9 &    1.51 & $\leq$20 & $\geq$0.44 &    1.45 & $\leq$27 & $\geq$0.45 & Y &  L\_I \\
 351 &     Per & J034351.02$+$320308.1 &            YSOc\_red &  5.9 &   $-$0.28 &         58 &       0.34 &   $-$0.23 &         73 &       0.39 & Y &    G \\
 352 &     Per & J034355.00$+$320103.1 & YSOc\_star$+$dust(IR2) & 13.1 &   $-$0.42 &       1000 &       0.0055 &   $-$0.82 &       3100 &       0.033 & N &    G \\
 353 &     Per & J034355.24$+$315532.1 & YSOc\_star$+$dust(IR1) & 10.8 &   $-$0.78 &       1100 &       0.089 &   $-$0.82 &       3000 &       0.45 & N &    G \\
 354 &     Per & J034355.28$+$320753.3 & YSOc\_star$+$dust(IR2) &  1.4 &   $-$0.95 &       1600 &       0.024 &   $-$1.01 &       3200 &       0.056 & N &    G \\
 355 &     Per & J034356.03$+$320213.3 & YSOc\_star$+$dust(IR2) & 10.4 &   $-$0.83 &       1300 &       0.40 &   $-$1.12 &       3200 &       2.3 & N &    G \\
 356 &     Per & J034356.52$+$320052.8 &                 red &  5.9 &    0.50 &         21 &       1.8 &    0.62 &         22 &       1.9 & Y &    G \\
 357 &     Per & J034356.84$+$320304.7 &            YSOc\_red &  5.9 &    1.37 &         25 &       1.1 &    1.40 &         27 &       1.1 & Y &    G \\
 358 &     Per & J034357.23$+$320133.7 & YSOc\_star$+$dust(IR2) &  9.4 &   $-$0.98 &       1300 &       0.015 &   $-$1.20 &       3200 &       0.081 & N &    G \\
 359 &     Per & J034357.27$+$320047.5 &                 red &  5.9 &    0.02 &        400 &       0.0011 &   $-$0.02 &        410 &       0.0020 & N &    G \\
 360 &     Per & J034357.64$+$320044.8 &                Galc &  7.7 &   $-$0.31 &       1200 &       0.0019 &   $-$0.58 &       2900 &       0.0072 & N &    G \\
 361 &     Per & J034357.82$+$320312.4 &                 red &  5.9 &    1.79 &        200 &       0.00090 &    1.79 &        210 &       0.0016 & N &    G \\
 362 &     Per & J034358.57$+$321727.5 & YSOc\_star$+$dust(IR2) &  3.2 &   $-$0.87 &       1600 &       0.14 &   $-$0.94 &       3200 &       0.40 & N &    G \\
 363 &     Per & J034358.92$+$321127.2 & YSOc\_star$+$dust(IR2) &  5.0 &   $-$0.51 &       1300 &       0.19 &   $-$0.61 &       3100 &       0.61 & N &    G \\
 364 &     Per & J034359.10$+$321421.2 & YSOc\_star$+$dust(IR2) &  6.9 &   $-$0.89 &       1400 &       0.062 &   $-$1.07 &       3300 &       0.28 & N &    G \\
 365 &     Per & J034359.41$+$320035.7 &            YSOc\_red &  5.9 &    0.14 &        300 &       0.055 &   $-$0.20 &        490 &       0.088 & N &    G \\
 366 &     Per & J034359.65$+$320154.1 &                YSOc & 19.8 &   $-$0.34 &        730 &       1.5 &   $-$0.94 &       2800 &       11 & N &    G \\
 367 &     Per & J034359.88$+$320441.4 & YSOc\_star$+$dust(IR2) &  2.4 &   $-$0.90 &       1600 &       0.017 &   $-$0.87 &       3200 &       0.046 & N &    G \\
 368 &     Per & J034400.48$+$320432.7 &            YSOc\_red & 16.0 &   $-$0.36 &        830 &       0.0057 &   $-$0.75 &       2800 &       0.037 & N &    G \\
 369 &     Per & J034401.57$+$322358.9 & YSOc\_star$+$dust(IR2) &  2.4 &   $-$1.00 &       1700 &       0.030 &   $-$1.04 &       3300 &       0.079 & N &    G \\
 370 &     Per & J034402.40$+$320204.9 &            YSOc\_red &  5.9 &    1.53 &         76 &       0.18 &    1.53 &         96 &       0.22 & Y &    G \\
 371 &     Per & J034402.63$+$320159.5 &            YSOc\_red &  5.9 &    1.12 &        270 &       0.018 &    1.04 &        280 &       0.034 & N &    G \\
 372 &     Per & J034402.92$+$315227.7 & YSOc\_star$+$dust(IR2) &  5.3 &   $-$1.06 &       1500 &       0.017 &   $-$1.21 &       3200 &       0.061 & N &    G \\
 373 &     Per & J034405.78$+$320001.1 & YSOc\_star$+$dust(IR1) & 12.9 &   $-$0.52 &       1000 &       0.0092 &   $-$0.82 &       3000 &       0.053 & N &    G \\
 374 &     Per & J034405.78$+$320028.5 &                YSOc & 22.5 &   $-$0.38 &        730 &       0.040 &   $-$0.94 &       2000 &       0.21 & N &    G \\
 375 &     Per & J034406.01$+$321532.1 & YSOc\_star$+$dust(IR1) &  1.6 &   $-$1.05 &       1600 &       0.013 &   $-$1.08 &       3200 &       0.030 & N &    G \\
 376 &     Per & J034406.47$+$314325.1 & YSOc\_star$+$dust(MP1) &  0.6 &   $-$2.34 &       2000 &       0.17 &   $-$2.30 &       3400 &       0.38 & N &    G \\
 377 &     Per & J034406.80$+$320754.0 & YSOc\_star$+$dust(IR2) &  2.6 &   $-$0.98 &       1600 &       0.052 &   $-$1.02 &       3200 &       0.14 & N &    G \\
 378 &     Per & J034409.16$+$320709.3 & YSOc\_star$+$dust(MP1) &  0.0 &   $-$2.27 & $\geq$2200 & $\geq$0.93 &   $-$2.27 & $\geq$2200 & $\geq$0.93 & N & L\_II \\
 379 &     Per & J034409.20$+$320237.8 & YSOc\_star$+$dust(IR1) &  5.9 &    0.69 &        350 &       0.16 &    0.61 &        470 &       0.31 & N &    G \\
 380 &     Per & J034410.13$+$320404.5 & YSOc\_star$+$dust(IR2) &  2.7 &   $-$0.94 &       1600 &       0.044 &   $-$0.94 &       3200 &       0.12 & N &    G \\
 381 &     Per & J034411.63$+$320313.1 & YSOc\_star$+$dust(IR3) &  8.7 &   $-$1.10 &       1400 &       0.18 &   $-$1.35 &       3200 &       0.91 & N &    G \\
 382 &     Per & J034412.98$+$320135.5 &                YSOc &  5.9 &    0.37 &        380 &       1.7 &    0.25 &        500 &       3.1 & Y &    G \\
 383 &     Per & J034415.84$+$315936.7 & YSOc\_star$+$dust(IR2) &  2.1 &   $-$0.81 &       1600 &       0.019 &   $-$0.83 &       3200 &       0.048 & N &    G \\
 384 &     Per & J034418.10$+$321053.5 & YSOc\_star$+$dust(IR4) & 14.3 &   $-$0.90 &        100 &       0.052 &   $-$1.06 &       2800 &       0.31 & N &    G \\
 385 &     Per & J034418.17$+$320457.0 & YSOc\_star$+$dust(IR3) &  8.5 &   $-$0.49 &       1100 &       0.38 &   $-$0.54 &       3100 &       1.7 & N &    G \\
 386 &     Per & J034418.21$+$320959.3 & YSOc\_star$+$dust(IR3) &  2.9 &   $-$1.21 &       1800 &       0.041 &   $-$1.19 &       3400 &       0.12 & N &    G \\
 387 &     Per & J034418.27$+$320732.5 & YSOc\_star$+$dust(IR4) &  0.0 &   $-$1.55 & $\geq$650 & $\geq$0.0034 &   $-$1.55 & $\geq$650 & $\geq$0.0034 & N & L\_II \\
 388 &     Per & J034418.59$+$321253.1 & YSOc\_star$+$dust(IR1) &  7.9 &   $-$0.83 &       1200 &       0.076 &   $-$1.03 &       3000 &       0.30 & N &    G \\
 389 &     Per & J034419.14$+$320931.3 & YSOc\_star$+$dust(MP1) &  0.0 &   $-$2.37 & $\geq$2100 & $\geq$0.31 &   $-$2.37 & $\geq$2100 & $\geq$0.31 & N & L\_II \\
 390 &     Per & J034419.14$+$321718.2 &                YSOc &  0.0 &   $-$2.66 & $\geq$2300 & $\geq$89 &   $-$2.66 & $\geq$2300 & $\geq$89 & N & L\_II \\
 391 &     Per & J034419.25$+$320734.7 & YSOc\_star$+$dust(IR4) &  0.0 &   $-$1.26 & $\geq$640 & $\geq$0.018 &   $-$1.26 & $\geq$640 & $\geq$0.018 & N & L\_II \\
 392 &     Per & J034420.18$+$320856.5 & YSOc\_star$+$dust(IR2) &  2.7 &   $-$1.39 &       1800 &       0.061 &   $-$1.50 &       3400 &       0.18 & N &    G \\
 393 &     Per & J034421.23$+$320114.5 & YSOc\_star$+$dust(IR4) & 12.9 &   $-$0.92 &       1300 &       0.012 &   $-$1.15 &       3300 &       0.095 & N &    G \\
 394 &     Per & J034421.29$+$321237.2 & YSOc\_star$+$dust(IR2) &  2.1 &   $-$1.35 &       1700 &       0.024 &   $-$1.37 &       3300 &       0.063 & N &    G \\
 395 &     Per & J034421.31$+$321156.3 & YSOc\_star$+$dust(IR3) &  2.9 &   $-$1.04 &       1700 &       0.070 &   $-$1.16 &       3300 &       0.21 & N &    G \\
 396 &     Per & J034421.35$+$315932.6 &            YSOc\_red &  5.9 &    0.21 &        360 &       0.25 &    0.44 &        480 &       0.43 & Y &    G \\
 397 &     Per & J034421.57$+$321509.7 & YSOc\_star$+$dust(MP1) &  1.6 &   $-$1.61 &       1900 &       0.040 &   $-$1.40 &       3400 &       0.100 & N &    G \\
 398 &     Per & J034421.62$+$321037.7 & YSOc\_star$+$dust(IR1) &  5.7 &   $-$1.00 &       1300 &       0.17 &   $-$1.05 &       3000 &       0.57 & N &    G \\
 399 &     Per & J034422.29$+$320542.8 & YSOc\_star$+$dust(IR3) &  5.6 &   $-$0.57 &       1400 &       0.14 &   $-$0.65 &       3100 &       0.50 & N &    G \\
 400 &     Per & J034422.34$+$321200.7 & YSOc\_star$+$dust(IR2) &  3.6 &   $-$0.86 &       1600 &       0.091 &   $-$1.04 &       3200 &       0.28 & N &    G \\
 401 &     Per & J034422.58$+$320153.6 & YSOc\_star$+$dust(IR4) &  2.9 &   $-$0.92 &       1700 &       0.012 &   $-$0.74 &       3300 &       0.34 & N &    G \\
 402 &     Per & J034422.70$+$320142.3 & YSOc\_star$+$dust(IR4) &  7.1 &   $-$1.36 &       1500 &       0.014 &   $-$1.00 &       3300 &       0.063 & N &    G \\
 403 &     Per & J034423.65$+$320152.7 & YSOc\_star$+$dust(IR3) &  8.6 &   $-$1.01 &       1400 &       0.030 &   $-$1.24 &       3200 &       0.15 & N &    G \\
 404 &     Per & J034424.46$+$320143.7 & YSOc\_star$+$dust(IR2) &  6.0 &   $-$0.97 &       1400 &       0.0079 &   $-$0.93 &       3200 &       0.029 & N &    G \\
 405 &     Per & J034424.84$+$321348.4 &            YSOc\_red &  5.9 &    1.73 &        180 &       0.0080 &    1.69 &        190 &       0.015 & N &    G \\
 406 &     Per & J034425.32$+$321012.7 & YSOc\_star$+$dust(IR3) &  3.0 &   $-$1.20 &       1700 &       0.061 &   $-$1.21 &       3300 &       0.17 & N &    G \\
 407 &     Per & J034425.52$+$321131.2 & YSOc\_star$+$dust(IR1) &  5.5 &   $-$0.53 &       1200 &       0.18 &   $-$0.64 &       2900 &       0.56 & N &    G \\
 408 &     Per & J034425.55$+$320617.1 & YSOc\_star$+$dust(IR4) &  5.5 &   $-$1.03 &       1600 &       0.078 &   $-$1.08 &       3300 &       0.31 & N &    G \\
 409 &     Per & J034425.71$+$321549.2 & YSOc\_star$+$dust(IR2) &  4.3 &   $-$0.81 &       1500 &       0.011 &   $-$0.86 &       3200 &       0.035 & N &    G \\
 410 &     Per & J034426.04$+$320430.4 & YSOc\_star$+$dust(IR1) &  6.1 &   $-$0.94 &       1400 &       1.5 &   $-$1.09 &       3200 &       5.5 & N &    G \\
 411 &     Per & J034426.70$+$320820.3 & YSOc\_star$+$dust(IR2) &  7.2 &   $-$0.92 &       1400 &       0.12 &   $-$1.03 &       3200 &       0.50 & N &    G \\
 412 &     Per & J034427.22$+$322028.8 & YSOc\_star$+$dust(IR2) &  2.0 &   $-$1.19 &       1700 &       0.022 &   $-$1.19 &       3300 &       0.059 & N &    G \\
 413 &     Per & J034427.26$+$321420.9 & YSOc\_star$+$dust(IR2) &  3.6 &   $-$0.90 &       1600 &       0.062 &   $-$0.98 &       3300 &       0.19 & N &    G \\
 414 &     Per & J034427.26$+$321037.3 & YSOc\_star$+$dust(IR2) &  3.9 &   $-$1.33 &       1600 &       0.038 &   $-$1.01 &       3300 &       0.12 & N &    G \\
 415 &     Per & J034427.90$+$322718.9 & YSOc\_star$+$dust(IR2) &  4.4 &   $-$0.93 &       1500 &       0.086 &   $-$1.04 &       3200 &       0.28 & N &    G \\
 416 &     Per & J034428.14$+$321600.2 & YSOc\_star$+$dust(MP1) &  2.2 &   $-$2.24 &       1900 &       0.081 &   $-$2.19 &       3500 &       0.24 & N &    G \\
 417 &     Per & J034428.51$+$315954.0 & YSOc\_star$+$dust(IR3) &  2.3 &   $-$1.32 &       1800 &       0.11 &   $-$1.35 &       3400 &       0.32 & N &    G \\
 418 &     Per & J034428.95$+$320137.9 & YSOc\_star$+$dust(IR2) & 11.9 &   $-$0.52 &       1100 &       0.036 &   $-$0.79 &       3100 &       0.21 & N &    G \\
 419 &     Per & J034429.23$+$320115.7 & YSOc\_star$+$dust(IR4) &  7.8 &   $-$1.00 &       1500 &       0.031 &   $-$1.06 &       3300 &       0.16 & N &    G \\
 420 &     Per & J034429.74$+$321039.8 & YSOc\_star$+$dust(IR2) &  5.3 &   $-$0.68 &       1400 &       0.21 &   $-$0.75 &       3200 &       0.78 & N &    G \\
 421 &     Per & J034429.80$+$320054.6 & YSOc\_star$+$dust(IR2) &  2.9 &   $-$0.88 &       1500 &       0.031 &   $-$0.98 &       3200 &       0.085 & N &    G \\
 422 &     Per & J034429.98$+$321922.6 & YSOc\_star$+$dust(MP1) &  2.5 &   $-$2.19 &       1900 &       0.070 &   $-$2.08 &       3500 &       0.21 & N &    G \\
 423 &     Per & J034430.14$+$320118.2 & YSOc\_star$+$dust(IR4) &  9.4 &   $-$1.48 &       1600 &       0.022 &   $-$1.65 &       3400 &       0.14 & N &    G \\
 424 &     Per & J034430.30$+$321135.2 & YSOc\_star$+$dust(IR1) &  5.9 &    0.20 &        710 &       0.012 &    0.04 &        930 &       0.029 & N &    G \\
 425 &     Per & J034430.84$+$320955.7 & YSOc\_star$+$dust(IR3) &  0.0 &   $-$1.11 & $\geq$2000 & $\geq$0.46 &   $-$1.11 & $\geq$2000 & $\geq$0.46 & N & L\_II \\
 426 &     Per & J034431.13$+$321848.5 & YSOc\_star$+$dust(IR2) &  7.6 &   $-$0.57 &       1200 &       0.023 &   $-$0.77 &       3100 &       0.094 & N &    G \\
 427 &     Per & J034431.19$+$320558.9 & YSOc\_star$+$dust(IR4) &  0.0 &   $-$0.64 & $\geq$510 & $\geq$0.023 &   $-$0.64 & $\geq$510 & $\geq$0.023 & N & L\_II \\
 428 &     Per & J034431.37$+$320014.2 & YSOc\_star$+$dust(IR2) & 11.6 &   $-$0.79 &       1300 &       0.13 &   $-$1.13 &       3200 &       0.90 & N &    G \\
 429 &     Per & J034431.55$+$320844.9 & YSOc\_star$+$dust(MP1) &  0.9 &   $-$2.36 &       2000 &       0.28 &   $-$1.83 &       3500 &       0.70 & N &    G \\
 430 &     Per & J034432.04$+$321143.7 &         YSOc\_PAH$-$em &  5.9 &   $-$0.26 &       1300 &       1.0 &   $-$0.67 &       1700 &       3.4 & N &    G \\
 431 &     Per & J034432.59$+$320855.7 & YSOc\_star$+$dust(IR4) &  3.0 &   $-$1.68 &       1800 &       0.11 &   $-$1.41 &       3400 &       0.34 & N &    G \\
 432 &     Per & J034433.22$+$321257.4 & YSOc\_star$+$dust(IR4) &  8.4 &   $-$0.97 &       1400 &       0.015 &   $-$1.13 &       3300 &       0.078 & N &    G \\
 433 &     Per & J034433.79$+$315830.2 & YSOc\_star$+$dust(IR4) &  5.7 &   $-$0.95 &       1500 &       0.051 &   $-$1.00 &       3300 &       0.20 & N &    G \\
 434 &     Per & J034434.05$+$320657.0 & YSOc\_star$+$dust(IR4) &  0.0 &   $-$0.81 & $\geq$570 & $\geq$0.0068 &   $-$0.81 & $\geq$570 & $\geq$0.0068 & N & L\_II \\
 435 &     Per & J034434.14$+$321635.7 & YSOc\_star$+$dust(IR2) &  4.1 &   $-$0.96 &       1500 &       0.022 &   $-$1.01 &       3200 &       0.069 & N &    G \\
 436 &     Per & J034434.21$+$320946.3 & YSOc\_star$+$dust(MP1) &  0.0 &   $-$2.03 & $\geq$2200 & $\geq$6.4 &   $-$2.03 & $\geq$2200 & $\geq$6.4 & N & L\_II \\
 437 &     Per & J034434.29$+$321240.7 & YSOc\_star$+$dust(IR2) & 14.3 &   $-$0.77 &       1200 &       0.044 &   $-$1.18 &       3200 &       0.35 & N &    G \\
 438 &     Per & J034434.69$+$321600.1 & YSOc\_star$+$dust(IR2) &  5.9 &   $-$0.09 &        760 &       0.068 &   $-$0.50 &       1000 &       0.16 & N &    G \\
 439 &     Per & J034434.71$+$321554.4 & YSOc\_star$+$dust(MP1) &  5.1 &   $-$1.89 &       1800 &       0.046 &   $-$1.55 &       3400 &       0.19 & N &    G \\
 440 &     Per & J034434.81$+$315655.2 & YSOc\_star$+$dust(IR4) &  3.2 &   $-$1.11 &       1600 &       0.054 &   $-$0.96 &       3300 &       0.16 & N &    G \\
 441 &     Per & J034434.99$+$321531.1 & YSOc\_star$+$dust(IR2) &  3.4 &   $-$1.02 &       1600 &       0.044 &   $-$1.20 &       3200 &       0.13 & N &    G \\
 442 &     Per & J034435.34$+$322837.2 &            YSOc\_red &  5.9 &    0.01 &        410 &       0.0020 &   $-$0.09 &        420 &       0.0033 & N &    G \\
 443 &     Per & J034435.38$+$320736.2 & YSOc\_star$+$dust(IR2) &  4.7 &   $-$0.84 &       1600 &       0.16 &   $-$1.04 &       3300 &       0.58 & N &    G \\
 444 &     Per & J034435.38$+$321004.6 & YSOc\_star$+$dust(IR3) &  0.0 &   $-$1.43 & $\geq$1900 & $\geq$3.1 &   $-$1.43 & $\geq$1900 & $\geq$3.1 & N & L\_II \\
 445 &     Per & J034435.47$+$320856.3 & YSOc\_star$+$dust(IR2) &  3.4 &   $-$0.89 &       1400 &       0.055 &   $-$0.52 &       3000 &       0.15 & N &    G \\
 446 &     Per & J034435.69$+$320303.5 & YSOc\_star$+$dust(IR1) &  7.9 &   $-$0.77 &       1300 &       0.050 &   $-$0.98 &       3100 &       0.21 & N &    G \\
 447 &     Per & J034435.96$+$320924.3 & YSOc\_star$+$dust(IR2) &  5.9 &   $-$0.01 &        480 &       0.100 &   $-$0.80 &        840 &       0.23 & N &    G \\
 448 &     Per & J034436.96$+$320645.2 & YSOc\_star$+$dust(IR4) &  1.2 &   $-$1.87 &       1900 &       1.2 &   $-$1.87 &       3400 &       3.0 & N &    G \\
 449 &     Per & J034437.40$+$321224.2 & YSOc\_star$+$dust(IR4) &  5.3 &   $-$0.60 &       1400 &       0.082 &   $-$0.62 &       3200 &       0.28 & N &    G \\
 450 &     Per & J034437.88$+$320804.1 & YSOc\_star$+$dust(IR2) &  5.6 &   $-$0.97 &       1500 &       0.29 &   $-$1.10 &       3200 &       1.1 & N &    G \\
 451 &     Per & J034437.98$+$320329.7 & YSOc\_star$+$dust(IR2) &  4.2 &   $-$0.96 &       1600 &       0.27 &   $-$1.11 &       3300 &       0.89 & N &    G \\
 452 &     Per & J034438.01$+$321137.0 & YSOc\_star$+$dust(IR3) &  2.6 &   $-$1.24 &       1700 &       0.037 &   $-$1.04 &       3300 &       0.100 & N &    G \\
 453 &     Per & J034438.46$+$320735.7 & YSOc\_star$+$dust(IR3) &  2.8 &   $-$0.79 &       1600 &       0.29 &   $-$0.94 &       3300 &       0.81 & N &    G \\
 454 &     Per & J034438.54$+$320800.6 & YSOc\_star$+$dust(IR3) &  3.6 &   $-$0.62 &       1500 &       0.17 &   $-$0.65 &       3200 &       0.51 & N &    G \\
 455 &     Per & J034438.97$+$320319.7 & YSOc\_star$+$dust(IR1) &  1.7 &   $-$1.16 &       1600 &       0.018 &   $-$0.90 &       3100 &       0.040 & N &    G \\
 456 &     Per & J034439.19$+$322008.9 & YSOc\_star$+$dust(IR3) &  2.2 &   $-$1.57 &       1800 &       0.061 &   $-$1.49 &       3400 &       0.17 & N &    G \\
 457 &     Per & J034439.21$+$320944.8 & YSOc\_star$+$dust(IR2) &  3.1 &   $-$1.15 &       1600 &       0.099 &   $-$0.77 &       3200 &       0.27 & N &    G \\
 458 &     Per & J034439.80$+$321804.0 & YSOc\_star$+$dust(IR3) &  3.5 &   $-$1.19 &       1700 &       0.11 &   $-$1.24 &       3300 &       0.35 & N &    G \\
 459 &     Per & J034441.74$+$321202.2 & YSOc\_star$+$dust(IR4) &  5.5 &   $-$0.68 &       1500 &       0.064 &   $-$0.70 &       3200 &       0.24 & N &    G \\
 460 &     Per & J034442.04$+$320859.9 & YSOc\_star$+$dust(IR4) &  4.6 &   $-$1.65 &       1800 &       0.18 &   $-$1.65 &       3400 &       0.69 & N &    G \\
 461 &     Per & J034442.15$+$320902.1 &                YSOc &  0.0 &   $-$0.52 & $\geq$510 & $\geq$0.058 &   $-$0.52 & $\geq$510 & $\geq$0.058 & N & L\_II \\
 462 &     Per & J034442.58$+$321002.5 & YSOc\_star$+$dust(IR2) &  5.5 &   $-$0.96 &       1500 &       0.048 &   $-$1.09 &       3200 &       0.18 & N &    G \\
 463 &     Per & J034442.76$+$320833.7 & YSOc\_star$+$dust(IR2) &  3.8 &   $-$1.10 &       1600 &       0.052 &   $-$1.09 &       3200 &       0.16 & N &    G \\
 464 &     Per & J034443.03$+$321559.6 & YSOc\_star$+$dust(IR1) &  4.4 &   $-$0.36 &       1200 &       0.021 &   $-$0.50 &       2900 &       0.059 & N &    G \\
 465 &     Per & J034443.06$+$313733.7 & YSOc\_star$+$dust(IR4) &  6.5 &   $-$0.95 &       1500 &       0.022 &   $-$1.09 &       3300 &       0.097 & N &    G \\
 466 &     Per & J034443.32$+$320131.5 &            YSOc\_red &  5.9 &    0.50 & $\leq$450 & $\geq$1.2 &    0.53 & $\leq$500 & $\geq$2.5 & Y &  L\_I \\
 467 &     Per & J034443.53$+$320742.7 & YSOc\_star$+$dust(MP1) &  4.8 &   $-$1.88 &       1800 &       0.14 &   $-$1.80 &       3400 &       0.54 & N &    G \\
 468 &     Per & J034443.78$+$321030.4 & YSOc\_star$+$dust(IR2) &  3.6 &   $-$0.45 &       1500 &       0.13 &   $-$0.66 &       3100 &       0.37 & N &    G \\
 469 &     Per & J034443.96$+$320136.2 &                 red &  5.9 &    0.96 &         40 &       3.0 &    0.99 &         49 &       3.2 & Y &    G \\
 470 &     Per & J034444.59$+$320812.5 & YSOc\_star$+$dust(IR1) &  4.0 &   $-$0.84 &       1400 &       0.095 &   $-$1.00 &       3000 &       0.26 & N &    G \\
 471 &     Per & J034444.72$+$320402.5 & YSOc\_star$+$dust(IR2) &  4.8 &   $-$0.92 &       1500 &       0.46 &   $-$1.03 &       3200 &       1.6 & N &    G \\
 472 &     Per & J034445.20$+$320119.6 & YSOc\_star$+$dust(IR1) & 10.8 &   $-$0.34 &        900 &       0.032 &   $-$0.61 &       2600 &       0.12 & N &    G \\
 473 &     Per & J034450.35$+$315236.0 & YSOc\_star$+$dust(IR2) &  4.1 &   $-$0.98 &       1500 &       0.013 &   $-$0.99 &       3200 &       0.041 & N &    G \\
 474 &     Per & J034452.00$+$322625.4 & YSOc\_star$+$dust(IR2) &  5.4 &   $-$1.43 &       1600 &       0.038 &   $-$1.53 &       3300 &       0.15 & N &    G \\
 475 &     Per & J034452.05$+$315825.2 & YSOc\_star$+$dust(IR2) &  6.0 &   $-$1.11 &       1500 &       0.044 &   $-$1.17 &       3200 &       0.17 & N &    G \\
 476 &     Per & J034455.62$+$320919.8 & YSOc\_star$+$dust(MP1) &  3.7 &   $-$2.22 &       1900 &       0.15 &   $-$1.80 &       3400 &       0.51 & N &    G \\
 477 &     Per & J034456.14$+$320915.2 & YSOc\_star$+$dust(IR4) &  4.0 &   $-$0.96 &       1500 &       0.41 &   $-$0.85 &       3200 &       1.3 & N &    G \\
 478 &     Per & J034456.84$+$315411.4 & YSOc\_star$+$dust(IR4) &  2.1 &   $-$1.33 &       1700 &       0.013 &   $-$1.16 &       3300 &       0.036 & N &    G \\
 479 &     Per & J034456.90$+$322035.6 &            YSOc\_red & 14.3 &   $-$0.41 &        850 &       0.0041 &   $-$0.68 &       2600 &       0.020 & N &    G \\
 480 &     Per & J034457.72$+$320741.7 & YSOc\_star$+$dust(IR4) &  2.6 &   $-$0.90 &       1600 &       0.014 &   $-$0.87 &       3300 &       0.039 & N &    G \\
 481 &     Per & J034457.85$+$320401.5 & YSOc\_star$+$dust(IR4) &  1.6 &   $-$1.62 &       1900 &       0.025 &   $-$1.65 &       3400 &       0.066 & N &    G \\
 482 &     Per & J034458.55$+$315827.1 & YSOc\_star$+$dust(IR1) &  4.6 &   $-$1.02 &       1500 &       0.0065 &   $-$1.18 &       3200 &       0.021 & N &    G \\
 483 &     Per & J034459.85$+$321331.9 & YSOc\_star$+$dust(IR3) &  3.2 &   $-$1.51 &       1700 &       0.026 &   $-$1.61 &       3300 &       0.080 & N &    G \\
 484 &     Per & J034500.45$+$320320.1 & YSOc\_star$+$dust(IR4) &  8.3 &   $-$1.53 &       1500 &       0.011 &   $-$1.59 &       3300 &       0.062 & N &    G \\
 485 &     Per & J034501.43$+$320501.7 & YSOc\_star$+$dust(MP1) &  0.0 &   $-$2.31 & $\geq$2000 & $\geq$0.32 &   $-$2.31 & $\geq$2000 & $\geq$0.32 & N & L\_II \\
 486 &     Per & J034504.66$+$321501.1 & YSOc\_star$+$dust(IR4) &  4.1 &   $-$1.93 &       1800 &       0.038 &   $-$1.82 &       3400 &       0.14 & N &    G \\
 487 &     Per & J034507.64$+$321027.9 & YSOc\_star$+$dust(IR2) &  0.0 &   $-$2.38 & $\geq$2100 & $\geq$0.39 &   $-$2.38 & $\geq$2100 & $\geq$0.39 & N & L\_II \\
 488 &     Per & J034513.08$+$322005.3 & YSOc\_star$+$dust(IR2) &  4.3 &   $-$1.26 &       1600 &       0.0094 &   $-$1.36 &       3100 &       0.029 & N &    G \\
 489 &     Per & J034513.51$+$322434.8 & YSOc\_star$+$dust(IR1) &  3.7 &   $-$1.10 &       1500 &       0.017 &   $-$1.05 &       3100 &       0.048 & N &    G \\
 490 &     Per & J034513.82$+$321210.0 &            YSOc\_red &  5.9 &    0.76 &        290 &       0.054 &    0.43 &        470 &       0.092 & N &    G \\
 491 &     Per & J034516.34$+$320620.1 & YSOc\_star$+$dust(IR1) &  8.6 &   $-$0.43 &        940 &       0.63 &   $-$0.71 &       2700 &       2.2 & N &    G \\
 492 &     Per & J034517.82$+$321205.8 & YSOc\_star$+$dust(IR2) &  3.2 &   $-$1.35 &       1700 &       0.026 &   $-$1.36 &       3300 &       0.082 & N &    G \\
 493 &     Per & J034520.46$+$320634.5 & YSOc\_star$+$dust(IR2) &  5.2 &   $-$0.83 &       1300 &       0.49 &   $-$0.91 &       3100 &       1.7 & N &    G \\
 494 &     Per & J034525.15$+$320930.3 & YSOc\_star$+$dust(IR2) &  3.5 &   $-$0.56 &       1300 &       0.18 &   $-$0.62 &       3000 &       0.48 & N &    G \\
 495 &     Per & J034529.72$+$315919.7 & YSOc\_star$+$dust(IR3) &  4.3 &   $-$1.05 &       1600 &       0.016 &   $-$1.10 &       3300 &       0.055 & N &    G \\
 496 &     Per & J034533.47$+$314555.3 & YSOc\_star$+$dust(IR2) &  6.3 &   $-$0.97 &       1400 &       0.012 &   $-$1.08 &       3200 &       0.048 & N &    G \\
 497 &     Per & J034535.64$+$315954.4 & YSOc\_star$+$dust(IR3) &  5.4 &   $-$0.97 &       1600 &       0.040 &   $-$1.10 &       3300 &       0.16 & N &    G \\
 498 &     Per & J034536.83$+$322557.0 & YSOc\_star$+$dust(IR2) &  3.9 &   $-$1.02 &       1700 &       0.60 &   $-$1.08 &       3300 &       2.0 & N &    G \\
 499 &     Per & J034547.37$+$314311.5 & YSOc\_star$+$dust(IR4) &  3.8 &   $-$1.81 &       1700 &       0.022 &   $-$1.83 &       3400 &       0.070 & N &    G \\
 500 &     Per & J034548.27$+$322412.0 &            YSOc\_red &  5.3 &   $-$0.72 &       1200 &       4.7 &   $-$0.77 &       3000 &       15 & N &    G \\
 501 &     Per & J034558.25$+$322647.5 & YSOc\_star$+$dust(IR2) &  3.7 &   $-$1.26 &       1600 &       0.030 &   $-$1.35 &       3200 &       0.091 & N &    G \\
 502 &     Per & J034657.38$+$324917.4 & YSOc\_star$+$dust(IR2) &  2.5 &   $-$1.27 &       1700 &       0.029 &   $-$1.23 &       3300 &       0.080 & N &    G \\
 503 &     Per & J034658.51$+$324658.9 & YSOc\_star$+$dust(IR4) &  3.3 &   $-$1.36 &       1700 &       0.032 &   $-$1.42 &       3300 &       0.099 & N &    G \\
 504 &     Per & J034705.43$+$324308.5 &            YSOc\_red &  5.9 &    0.36 &        300 &       0.58 &    0.48 &        400 &       0.96 & Y &    G \\
 505 &     Per & J034741.58$+$325144.1 &                YSOc &  5.9 &    0.78 &        270 &       5.0 &    1.09 &        350 &       8.3 & Y &    G \\
 506 &    Serp & J182753.82$-$000233.3 & YSOc\_star$+$dust(IR4) &  2.9 &   $-$1.26 &       2200 &       0.17 &   $-$1.23 &       3300 &       0.35 & N &    G \\
 507 &    Serp & J182808.46$-$000106.4 & YSOc\_star$+$dust(IR1) &  7.0 &   $-$0.85 &       1500 &       0.59 &   $-$1.00 &       3000 &       2.3 & N &    G \\
 508 &    Serp & J182811.01$-$000139.4 & YSOc\_star$+$dust(MP1) & 14.5 &   $-$2.20 &       1800 &       0.53 &   $-$2.61 &       7900 &       270 & N &    G \\
 509 &    Serp & J182813.51$-$000249.1 & YSOc\_star$+$dust(IR3) &  5.5 &   $-$0.76 &       1700 &       0.72 &   $-$0.86 &       2800 &       2.2 & N &    G \\
 510 &    Serp & J182815.02$-$000258.8 & YSOc\_star$+$dust(IR1) &  9.6 &    0.03 &        690 &       0.25 &   $-$0.42 &       1200 &       1.1 & N &    G \\
 511 &    Serp & J182815.19$-$000140.6 & YSOc\_star$+$dust(IR2) &  3.8 &   $-$1.11 &       1900 &       0.041 &   $-$1.13 &       3200 &       0.100 & N &    G \\
 512 &    Serp & J182815.26$-$000243.3 & YSOc\_star$+$dust(IR4) &  6.2 &   $-$0.85 &        820 &       1.2 &   $-$0.87 &       2000 &       1.4 & N &    G \\
 513 &    Serp & J182816.29$-$000316.1 & YSOc\_star$+$dust(IR2) &  6.6 &   $-$0.95 &       1500 &       0.29 &   $-$1.10 &       3200 &       1.0 & N &    G \\
 514 &    Serp & J182818.53$-$000332.9 & YSOc\_star$+$dust(IR3) &  5.0 &   $-$1.09 &       1400 &       0.015 &   $-$1.15 &       3300 &       0.043 & N &    G \\
 515 &    Serp & J182819.81$-$000147.4 & YSOc\_star$+$dust(IR1) &  8.4 &   $-$1.03 &       1300 &       0.019 &   $-$1.17 &       3100 &       0.081 & N &    G \\
 516 &    Serp & J182820.10$+$002914.5 & YSOc\_star$+$dust(MP1) &  9.1 &   $-$2.32 &       1800 &       1.2 &   $-$2.61 &       3500 &       8.8 & N &    G \\
 517 &    Serp & J182821.43$+$001041.1 & YSOc\_star$+$dust(IR3) &  7.0 &   $-$1.26 &       1700 &       0.071 &   $-$1.42 &       2100 &       0.20 & N &    G \\
 518 &    Serp & J182821.59$+$000016.4 & YSOc\_star$+$dust(IR2) &  6.6 &   $-$0.67 &       1300 &       0.32 &   $-$0.80 &       3100 &       1.2 & N &    G \\
 519 &    Serp & J182827.38$-$001150.0 & YSOc\_star$+$dust(MP1) & 19.0 &   $-$2.09 &       1700 &       4.6 &   $-$2.61 &       3700 &       300 & N &    G \\
 520 &    Serp & J182827.40$+$000023.9 & YSOc\_star$+$dust(MP1) & 11.1 &   $-$1.99 &       1600 &       0.34 &   $-$2.28 &       3400 &       2.8 & N &    G \\
 521 &    Serp & J182828.50$+$002650.1 & YSOc\_star$+$dust(IR3) & 10.8 &   $-$1.04 &       1400 &       0.011 &   $-$1.35 &       3300 &       0.074 & N &    G \\
 522 &    Serp & J182829.05$+$002756.2 & YSOc\_star$+$dust(IR4) & 12.6 &   $-$0.67 &       1200 &       0.049 &   $-$0.87 &       3200 &       0.36 & N &    G \\
 523 &    Serp & J182840.25$+$001617.4 & YSOc\_star$+$dust(IR2) & 14.3 &   $-$1.04 &       1200 &       0.012 &   $-$1.46 &       3200 &       0.098 & N &    G \\
 524 &    Serp & J182840.52$+$002214.5 & YSOc\_star$+$dust(MP1) & 11.7 &   $-$1.93 &       1600 &       0.26 &   $-$2.22 &       3400 &       2.3 & N &    G \\
 525 &    Serp & J182841.87$-$000321.3 & YSOc\_star$+$dust(IR1) &  9.6 &    0.37 &        410 &       0.16 &    0.14 &        770 &       0.48 & N &    G \\
 526 &    Serp & J182844.01$+$005337.9 &            YSOc\_red &  9.6 &    0.45 &        260 &       0.28 &    0.26 &        460 &       0.65 & Y &    G \\
 527 &    Serp & J182844.78$+$005125.8 &            YSOc\_red &  9.6 &    1.07 &        120 &       0.040 &    1.05 &        180 &       0.078 & Y &    G \\
 528 &    Serp & J182844.81$+$004808.6 & YSOc\_star$+$dust(IR1) &  8.0 &   $-$0.96 &       1500 &       0.033 &   $-$1.12 &       2000 &       0.089 & N &    G \\
 529 &    Serp & J182844.96$+$005203.5 &            YSOc\_red &  9.6 &    1.33 &         77 &       0.89 &    1.27 &        120 &       1.3 & Y &    G \\
 530 &    Serp & J182844.98$+$004524.0 & YSOc\_star$+$dust(IR2) &  5.0 &   $-$1.34 &       1600 &       0.19 &   $-$1.48 &       1900 &       0.36 & N &    G \\
 531 &    Serp & J182845.58$-$000712.7 & YSOc\_star$+$dust(IR1) & 15.7 &   $-$1.01 &       1500 &       19 &   $-$1.47 &       3200 &       77 & N &    G \\
 532 &    Serp & J182846.13$+$000301.6 & YSOc\_star$+$dust(IR1) & 12.7 &   $-$0.86 &       1100 &       0.028 &   $-$1.26 &       3000 &       0.17 & N &    G \\
 533 &    Serp & J182847.84$+$000840.3 &                YSOc &  8.3 &   $-$0.78 &       1400 &       11 &   $-$1.06 &       3000 &       40 & N &    G \\
 534 &    Serp & J182848.09$+$001926.7 & YSOc\_star$+$dust(IR4) &  5.0 &   $-$0.82 &       1100 &       0.0071 &   $-$0.95 &       2500 &       0.018 & N &    G \\
 535 &    Serp & J182850.21$+$000949.7 & YSOc\_star$+$dust(IR1) &  5.5 &   $-$0.44 &        890 &       0.41 &   $-$0.51 &       1100 &       0.60 & N &    G \\
 536 &    Serp & J182850.38$-$001255.1 & YSOc\_star$+$dust(IR4) & 10.2 &   $-$1.71 &       1300 &       0.87 &   $-$1.98 &       3300 &       6.1 & N &    G \\
 537 &    Serp & J182851.22$+$001927.3 &            YSOc\_red &  9.6 &    0.45 &        250 &       0.060 &    0.34 &        460 &       0.13 & Y &    G \\
 538 &    Serp & J182852.01$+$001551.6 & YSOc\_star$+$dust(IR2) &  7.4 &   $-$1.14 &       1500 &       0.0071 &   $-$1.36 &       3300 &       0.033 & N &    G \\
 539 &    Serp & J182852.76$+$002846.8 &            YSOc\_red &  9.6 &    0.06 &        620 &       0.0097 &   $-$0.09 &        900 &       0.036 & N &    G \\
 540 &    Serp & J182853.64$+$001940.9 & YSOc\_star$+$dust(IR4) & 25.0 &   $-$0.72 &        960 &       0.011 &   $-$1.37 &       3000 &       0.16 & N &    G \\
 541 &    Serp & J182853.95$+$004553.0 & YSOc\_star$+$dust(IR3) & 13.5 &   $-$0.84 &       1500 &       0.066 &   $-$1.17 &       2400 &       0.49 & N &    G \\
 542 &    Serp & J182854.05$+$002930.0 &            YSOc\_red &  9.6 &    1.36 &         58 &       3.1 &    1.31 &         85 &       4.0 & Y &    G \\
 543 &    Serp & J182854.50$+$002852.4 &                YSOc &  0.0 &   $-$1.01 & $\geq$760 & $\geq$0.049 &   $-$1.01 & $\geq$760 & $\geq$0.049 & N & L\_II \\
 544 &    Serp & J182854.87$+$002952.5 &            YSOc\_red &  9.6 &    1.91 &         51 &       2.6 &    1.82 &         74 &       3.3 & Y &    G \\
 545 &    Serp & J182854.91$+$001832.7 &            YSOc\_red &  9.6 &    0.90 &        120 &       0.050 &    0.84 &        190 &       0.089 & Y &    G \\
 546 &    Serp & J182855.30$+$002052.3 & YSOc\_star$+$dust(IR1) & 14.1 &   $-$0.34 &        940 &       0.100 &   $-$0.78 &       2900 &       0.61 & N &    G \\
 547 &    Serp & J182855.78$+$002944.8 &            YSOc\_red &  9.6 &    1.89 & $\leq$54 & $\geq$0.18 &    1.80 & $\leq$99 & $\geq$0.27 & Y &  L\_I \\
 548 &    Serp & J182856.64$+$003008.3 &            YSOc\_red &  9.6 &    1.78 &        180 &       0.0036 &    1.69 &        190 &       0.0098 & N &    G \\
 549 &    Serp & J182857.15$+$004836.1 & YSOc\_star$+$dust(MP1) & 10.0 &   $-$0.37 &        900 &       0.0064 &   $-$0.50 &       2600 &       0.023 & N &    G \\
 550 &    Serp & J182858.09$+$001724.5 & YSOc\_star$+$dust(IR4) &  3.0 &   $-$1.92 &       1600 &       0.47 &   $-$2.04 &       1800 &       0.68 & N &    G \\
 551 &    Serp & J182858.61$+$004859.4 & YSOc\_star$+$dust(IR1) &  7.0 &   $-$1.02 &       1500 &       0.043 &   $-$1.11 &       1900 &       0.099 & N &    G \\
 552 &    Serp & J182859.46$+$003003.1 & YSOc\_star$+$dust(IR3) & 18.4 &   $-$0.61 &        900 &       0.17 &   $-$1.14 &       3100 &       1.5 & N &    G \\
 553 &    Serp & J182900.25$+$001658.0 & YSOc\_star$+$dust(IR1) &  5.0 &   $-$1.05 &       1400 &       0.15 &   $-$1.14 &       1600 &       0.26 & N &    G \\
 554 &    Serp & J182900.57$+$004507.9 & YSOc\_star$+$dust(IR1) & 10.0 &   $-$0.97 &       1300 &       0.061 &   $-$1.14 &       3200 &       0.33 & N &    G \\
 555 &    Serp & J182900.82$+$002746.9 & YSOc\_star$+$dust(IR1) & 10.5 &   $-$0.38 &       1000 &       0.037 &   $-$0.66 &       2900 &       0.16 & N &    G \\
 556 &    Serp & J182900.90$+$002931.6 & YSOc\_star$+$dust(IR1) &  9.3 &   $-$0.42 &        930 &       1.2 &   $-$0.69 &       2800 &       4.2 & N &    G \\
 557 &    Serp & J182901.08$+$003145.3 & YSOc\_star$+$dust(IR2) & 23.3 &   $-$0.77 &        100 &       0.19 &   $-$1.46 &       3200 &       2.9 & N &    G \\
 558 &    Serp & J182901.23$+$002933.0 & YSOc\_star$+$dust(IR1) &  5.5 &   $-$0.54 &       1000 &       0.32 &   $-$0.62 &       1300 &       0.49 & N &    G \\
 559 &    Serp & J182901.53$+$001730.0 & YSOc\_star$+$dust(IR3) & 12.0 &   $-$1.21 &       1300 &       0.0098 &   $-$1.63 &       3200 &       0.066 & N &    G \\
 560 &    Serp & J182901.75$+$002946.6 & YSOc\_star$+$dust(IR2) &  5.0 &   $-$0.65 &       1400 &       0.63 &   $-$0.77 &       1600 &       1.1 & N &    G \\
 561 &    Serp & J182901.84$+$002954.6 & YSOc\_star$+$dust(IR1) &  4.0 &   $-$1.04 &       1200 &       1.8 &   $-$1.13 &       1400 &       2.6 & N &    G \\
 562 &    Serp & J182902.12$+$003120.7 &            YSOc\_red &  9.6 &    0.24 &         85 &       0.050 &    0.29 &        130 &       0.074 & Y &    G \\
 563 &    Serp & J182902.84$+$003009.6 & YSOc\_star$+$dust(IR2) &  9.6 &   $-$0.14 &        460 &       0.17 &   $-$0.57 &       1000 &       0.51 & Y &    G \\
 564 &    Serp & J182903.94$+$002021.7 & YSOc\_star$+$dust(IR1) &  2.0 &   $-$0.84 &       1400 &       0.81 &   $-$0.87 &       1600 &       1.0 & N &    G \\
 565 &    Serp & J182904.37$+$003324.0 & YSOc\_star$+$dust(IR1) &  9.6 &    0.20 &        530 &       0.66 &    0.23 &        690 &       2.1 & N &    G \\
 566 &    Serp & J182905.17$+$003843.9 & YSOc\_star$+$dust(IR2) & 11.0 &   $-$1.04 &       1400 &       0.016 &   $-$1.22 &       3400 &       0.12 & N &    G \\
 567 &    Serp & J182905.76$+$002232.6 & YSOc\_star$+$dust(MP1) &  0.5 &   $-$1.75 &       2100 &       0.32 &   $-$1.69 &       2100 &       0.34 & N &    G \\
 568 &    Serp & J182906.15$+$001944.5 & YSOc\_star$+$dust(IR4) &  6.0 &   $-$1.10 &       1700 &       0.045 &   $-$1.20 &       2100 &       0.100 & N &    G \\
 569 &    Serp & J182906.20$+$003043.3 &            YSOc\_red &  9.6 &    1.70 &        120 &       1.5 &    1.52 &        160 &       2.7 & Y &    G \\
 570 &    Serp & J182906.76$+$003034.3 &            YSOc\_red &  9.6 &    1.66 &         76 &       1.9 &    1.61 &         99 &       2.8 & Y &    G \\
 571 &    Serp & J182906.97$+$003838.0 & YSOc\_star$+$dust(IR2) & 15.2 &   $-$0.75 &       1100 &       0.078 &   $-$1.12 &       3100 &       0.61 & N &    G \\
 572 &    Serp & J182907.42$+$001921.5 & YSOc\_star$+$dust(IR3) &  3.8 &   $-$1.61 &       1700 &       0.014 &   $-$1.69 &       3300 &       0.044 & N &    G \\
 573 &    Serp & J182907.64$+$005222.3 & YSOc\_star$+$dust(IR2) &  5.3 &   $-$0.77 &       1500 &       0.024 &   $-$0.89 &       3200 &       0.082 & N &    G \\
 574 &    Serp & J182907.75$+$005403.8 & YSOc\_star$+$dust(IR2) &  9.0 &   $-$0.99 &       1600 &       0.050 &   $-$1.26 &       2100 &       0.17 & N &    G \\
 575 &    Serp & J182908.09$-$000737.1 & YSOc\_star$+$dust(MP1) & 14.0 &   $-$2.27 &       1900 &       0.57 &   $-$2.61 &       3800 &       18 & N &    G \\
 576 &    Serp & J182908.18$+$010544.6 & YSOc\_star$+$dust(MP1) &  0.0 &   $-$2.05 & $\geq$2100 & $\geq$0.25 &   $-$2.05 & $\geq$2100 & $\geq$0.25 & N & L\_II \\
 577 &    Serp & J182909.05$+$003128.0 &                Galc &  9.6 &    0.25 &        400 &       0.0078 &    0.25 &        410 &       0.024 & N &    G \\
 578 &    Serp & J182909.07$+$003132.4 &                 red &  9.6 &    2.27 &         54 &       0.89 &    2.21 &         58 &       1.1 & Y &    G \\
 579 &    Serp & J182909.56$+$003702.1 &                YSOc & 25.2 &   $-$1.16 &       1200 &       2.9 &   $-$1.96 &       3400 &       81 & N &    G \\
 580 &    Serp & J182911.50$+$002038.8 & YSOc\_star$+$dust(MP1) &  9.0 &   $-$0.85 &       1600 &       0.028 &   $-$0.94 &       2200 &       0.099 & N &    G \\
 581 &    Serp & J182912.49$+$001815.1 & YSOc\_star$+$dust(IR4) & 13.9 &   $-$1.03 &       1300 &       0.019 &   $-$1.35 &       3300 &       0.17 & N &    G \\
 582 &    Serp & J182912.89$+$000947.7 & YSOc\_star$+$dust(IR3) &  6.9 &   $-$1.12 &       1900 &       0.021 &   $-$1.15 &       3900 &       0.11 & N &    G \\
 583 &    Serp & J182914.33$+$010730.1 & YSOc\_star$+$dust(IR2) &  3.5 &   $-$1.31 &       1700 &       0.014 &   $-$1.36 &       3300 &       0.044 & N &    G \\
 584 &    Serp & J182915.13$+$003937.9 & YSOc\_star$+$dust(IR2) &  8.0 &   $-$1.75 &       1400 &       0.12 &   $-$2.00 &       1800 &       0.28 & N &    G \\
 585 &    Serp & J182915.39$-$001251.9 & YSOc\_star$+$dust(IR4) &  9.5 &   $-$1.59 &       1800 &       0.42 &   $-$1.91 &       3100 &       2.9 & N &    G \\
 586 &    Serp & J182915.57$+$003911.9 & YSOc\_star$+$dust(IR2) & 10.9 &   $-$0.31 &       1100 &       0.073 &   $-$0.66 &       3000 &       0.37 & N &    G \\
 587 &    Serp & J182915.63$+$003923.0 & YSOc\_star$+$dust(IR2) &  0.0 &   $-$0.47 &        990 &       0.056 &   $-$0.47 &        990 &       0.056 & N &    G \\
 588 &    Serp & J182916.18$+$001822.7 &                YSOc &  9.6 &   $-$0.07 &        430 &       1.8 &   $-$0.13 &        740 &       4.7 & Y &    G \\
 589 &    Serp & J182919.70$+$001803.1 & YSOc\_star$+$dust(IR2) &  5.0 &   $-$0.95 &       1500 &       0.098 &   $-$1.06 &       1700 &       0.17 & N &    G \\
 590 &    Serp & J182920.03$+$012101.5 & YSOc\_star$+$dust(MP1) &  8.5 &   $-$2.30 &       1700 &       0.58 &   $-$2.52 &       3500 &       3.7 & N &    G \\
 591 &    Serp & J182920.42$+$012103.8 & YSOc\_star$+$dust(IR4) &  9.1 &   $-$1.41 &       1500 &       0.17 &   $-$1.59 &       3300 &       0.99 & N &    G \\
 592 &    Serp & J182920.95$+$003034.6 & YSOc\_star$+$dust(MP1) & 16.7 &   $-$1.76 &       1500 &       2.8 &   $-$2.21 &       3400 &       40 & N &    G \\
 593 &    Serp & J182921.84$+$001938.6 & YSOc\_star$+$dust(IR1) &  5.0 &   $-$0.95 &       1800 &       0.063 &   $-$1.06 &       2500 &       0.15 & N &    G \\
 594 &    Serp & J182926.41$+$003004.4 & YSOc\_star$+$dust(IR4) & 13.4 &   $-$0.73 &       1300 &       0.018 &   $-$1.11 &       3300 &       0.15 & N &    G \\
 595 &    Serp & J182926.79$+$003949.9 & YSOc\_star$+$dust(IR2) & 19.4 &   $-$0.54 &        830 &       0.050 &   $-$1.03 &       3100 &       0.48 & N &    G \\
 596 &    Serp & J182927.29$+$003906.7 & YSOc\_star$+$dust(IR2) &  0.0 &   $-$1.04 &        100 &       0.0060 &   $-$1.04 &       3000 &       0.076 & N &    G \\
 597 &    Serp & J182927.35$+$003849.8 &                YSOc &  9.6 &    0.32 &        610 &       0.012 &    0.24 &        970 &       0.048 & N &    G \\
 598 &    Serp & J182928.23$-$002257.2 & YSOc\_star$+$dust(IR3) & 22.4 &   $-$0.79 &       1200 &       5.1 &   $-$1.94 &       3200 &       53 & N &    G \\
 599 &    Serp & J182928.97$+$001310.4 & YSOc\_star$+$dust(IR4) &  8.6 &   $-$2.01 &       1600 &       1.1 &   $-$2.18 &       3500 &       6.0 & N &    G \\
 600 &    Serp & J182929.28$+$001800.0 & YSOc\_star$+$dust(IR2) &  6.5 &   $-$1.24 &       1600 &       0.031 &   $-$1.40 &       2000 &       0.071 & N &    G \\
 601 &    Serp & J182930.84$+$010107.3 & YSOc\_star$+$dust(IR1) &  5.4 &   $-$0.94 &       1400 &       0.16 &   $-$1.01 &       3100 &       0.53 & N &    G \\
 602 &    Serp & J182931.96$+$011842.9 & YSOc\_star$+$dust(IR1) &  9.6 &    0.26 &        410 &       5.9 &    0.32 &        740 &       20 & Y &    G \\
 603 &    Serp & J182932.54$-$001323.3 & YSOc\_star$+$dust(MP1) &  3.0 &   $-$2.51 &       2600 &       8.4 &   $-$2.56 &       3000 &       18 & N &    G \\
 604 &    Serp & J182933.00$+$004008.9 & YSOc\_star$+$dust(IR2) &  9.2 &   $-$1.02 &       1500 &       0.034 &   $-$1.26 &       3400 &       0.21 & N &    G \\
 605 &    Serp & J182933.36$+$010824.6 & YSOc\_star$+$dust(IR2) &  0.0 &   $-$0.81 & $\geq$1700 & $\geq$0.71 &   $-$0.81 & $\geq$1700 & $\geq$0.71 & N & L\_II \\
 606 &    Serp & J182935.62$+$003503.9 & YSOc\_star$+$dust(MP1) &  4.5 &   $-$1.02 &       1600 &       0.20 &   $-$0.98 &       1800 &       0.34 & N &    G \\
 607 &    Serp & J182936.20$+$004216.8 & YSOc\_star$+$dust(IR1) &  6.0 &   $-$0.68 &       1100 &       0.12 &   $-$0.64 &       1500 &       0.21 & N &    G \\
 608 &    Serp & J182936.35$+$003356.0 & YSOc\_star$+$dust(MP1) &  7.4 &   $-$2.12 &       1800 &       0.043 &   $-$2.25 &       3500 &       0.24 & N &    G \\
 609 &    Serp & J182936.45$+$004621.7 & YSOc\_star$+$dust(IR2) &  5.3 &   $-$1.11 &       1500 &       0.0069 &   $-$1.27 &       3200 &       0.025 & N &    G \\
 610 &    Serp & J182936.71$+$004758.0 & YSOc\_star$+$dust(IR1) &  7.4 &   $-$1.08 &       1400 &       0.061 &   $-$1.18 &       3100 &       0.25 & N &    G \\
 611 &    Serp & J182937.67$+$011130.0 & YSOc\_star$+$dust(MP1) &  9.7 &   $-$2.02 &       1800 &       0.70 &   $-$2.25 &       3400 &       4.1 & N &    G \\
 612 &    Serp & J182938.82$+$004438.1 & YSOc\_star$+$dust(IR3) &  8.8 &   $-$1.25 &       1500 &       0.019 &   $-$1.46 &       3300 &       0.100 & N &    G \\
 613 &    Serp & J182939.86$+$011756.1 & YSOc\_star$+$dust(IR3) &  9.2 &   $-$0.84 &       1500 &       0.053 &   $-$1.07 &       3200 &       0.24 & N &    G \\
 614 &    Serp & J182940.21$+$001513.1 & YSOc\_star$+$dust(IR1) &  9.6 &    0.87 &        370 &       0.074 &    0.68 &        750 &       0.24 & N &    G \\
 615 &    Serp & J182941.21$+$004902.1 & YSOc\_star$+$dust(IR3) &  8.5 &   $-$1.07 &       1600 &       0.041 &   $-$1.36 &       2100 &       0.13 & N &    G \\
 616 &    Serp & J182941.25$+$004729.6 & YSOc\_star$+$dust(IR2) &  5.0 &   $-$0.96 &       1300 &       0.0034 &   $-$0.99 &       2700 &       0.0090 & N &    G \\
 617 &    Serp & J182941.46$+$010738.0 & YSOc\_star$+$dust(IR1) &  6.2 &   $-$0.89 &       1400 &       0.39 &   $-$1.00 &       3200 &       1.5 & N &    G \\
 618 &    Serp & J182941.52$+$011004.4 & YSOc\_star$+$dust(MP1) &  9.6 &   $-$1.92 &       1700 &       0.14 &   $-$2.08 &       3400 &       1.0 & N &    G \\
 619 &    Serp & J182941.69$+$004427.1 & YSOc\_star$+$dust(IR3) &  3.0 &   $-$0.88 &       1800 &       0.15 &   $-$0.97 &       1900 &       0.22 & N &    G \\
 620 &    Serp & J182942.16$+$012021.1 & YSOc\_star$+$dust(IR2) &  2.4 &   $-$0.50 &       2000 &       0.066 &   $-$0.68 &       3100 &       0.12 & N &    G \\
 621 &    Serp & J182943.92$+$010720.8 & YSOc\_star$+$dust(IR1) &  8.0 &   $-$1.28 &       1600 &       0.074 &   $-$1.46 &       3200 &       0.29 & N &    G \\
 622 &    Serp & J182944.11$+$003356.1 & YSOc\_star$+$dust(MP1) &  4.5 &   $-$1.41 &       2000 &       0.18 &   $-$1.36 &       2500 &       0.42 & N &    G \\
 623 &    Serp & J182944.31$+$010453.4 &      star$+$dust(IR2) & 12.4 &   $-$0.76 &       1400 &       18 &   $-$1.41 &       3300 &       130 & N &    G \\
 624 &    Serp & J182944.52$+$011311.5 & YSOc\_star$+$dust(IR3) &  3.6 &   $-$1.08 &       1700 &       0.052 &   $-$1.15 &       3300 &       0.16 & N &    G \\
 625 &    Serp & J182945.03$+$003526.6 & YSOc\_star$+$dust(IR4) &  3.0 &   $-$1.06 &       1500 &       0.060 &   $-$1.11 &       1600 &       0.080 & N &    G \\
 626 &    Serp & J182946.28$+$011025.4 & YSOc\_star$+$dust(IR2) &  2.6 &   $-$1.34 &       1700 &       0.047 &   $-$1.42 &       3300 &       0.13 & N &    G \\
 627 &    Serp & J182947.01$+$011626.9 &                YSOc &  9.6 &   $-$0.11 &        680 &       0.042 &   $-$0.19 &        860 &       0.15 & N &    G \\
 628 &    Serp & J182947.26$+$003955.7 & YSOc\_star$+$dust(IR4) &  5.0 &   $-$0.78 &       1600 &       0.037 &   $-$0.85 &       1900 &       0.072 & N &    G \\
 629 &    Serp & J182947.27$+$003223.1 & YSOc\_star$+$dust(IR3) &  6.0 &   $-$0.90 &       1600 &       0.060 &   $-$1.08 &       1900 &       0.13 & N &    G \\
 630 &    Serp & J182947.63$+$010422.4 & YSOc\_star$+$dust(IR4) &  0.0 &   $-$0.60 & $\geq$460 & $\geq$0.016 &   $-$0.60 & $\geq$460 & $\geq$0.016 & N & L\_II \\
 631 &    Serp & J182948.10$+$011644.9 &            YSOc\_red &  9.6 &    1.37 &         57 &       2.2 &    1.30 &         68 &       2.7 & Y &    G \\
 632 &    Serp & J182948.78$+$011342.2 & YSOc\_star$+$dust(IR4) & 25.0 &   $-$0.81 &       1000 &       0.015 &   $-$1.48 &       3100 &       0.26 & N &    G \\
 633 &    Serp & J182949.13$+$011619.9 &              rising &  9.6 &    3.80 &         79 &       7.7 &    3.78 &        130 &       10 & Y &    G \\
 634 &    Serp & J182949.25$+$011631.5 &            YSOc\_red &  9.6 &    1.45 &        260 &       0.45 &    1.29 &        300 &       1.3 & N &    G \\
 635 &    Serp & J182949.58$+$011706.0 &                YSOc &  9.6 &    0.66 &        480 &       0.33 &    0.69 &        550 &       1.1 & N &    G \\
 636 &    Serp & J182949.62$+$005052.8 & YSOc\_star$+$dust(MP1) &  8.8 &   $-$2.02 &       2300 &       0.48 &   $-$2.28 &       3400 &       2.3 & N &    G \\
 637 &    Serp & J182949.63$+$011521.9 &            YSOc\_red &  9.6 &    2.65 & $\leq$58 & $\geq$1.3 &    2.59 & $\leq$97 & $\geq$2.1 & Y &  L\_I \\
 638 &    Serp & J182949.69$+$011456.8 &                YSOc &  9.6 &    0.25 &        460 &       0.100 &    0.15 &        470 &       0.32 & N &    G \\
 639 &    Serp & J182950.02$+$005101.5 & YSOc\_star$+$dust(IR4) &  8.0 &   $-$1.49 &       1800 &       0.062 &   $-$1.70 &       2200 &       0.20 & N &    G \\
 640 &    Serp & J182950.16$+$005608.1 & YSOc\_star$+$dust(IR1) &  0.0 &   $-$0.77 &       1200 &       0.11 &   $-$0.77 &       3100 &       0.53 & N &    G \\
 641 &    Serp & J182950.41$+$004343.7 & YSOc\_star$+$dust(IR2) &  8.8 &   $-$1.39 &       1500 &       0.15 &   $-$1.58 &       3300 &       0.80 & N &    G \\
 642 &    Serp & J182951.15$+$011640.7 &            YSOc\_red &  9.6 &    1.04 &        140 &       1.7 &    1.03 &        240 &       3.0 & Y &    G \\
 643 &    Serp & J182951.17$+$011319.8 & YSOc\_star$+$dust(IR4) & 11.1 &   $-$1.16 &       1400 &       0.0090 &   $-$1.35 &       3300 &       0.060 & N &    G \\
 644 &    Serp & J182951.30$+$002748.0 & YSOc\_star$+$dust(MP1) &  0.0 &   $-$2.20 & $\geq$2000 & $\geq$0.30 &   $-$2.20 & $\geq$2000 & $\geq$0.30 & N & L\_II \\
 645 &    Serp & J182952.06$+$003643.6 &            YSOc\_red &  9.6 &   $-$0.04 &        660 &       0.016 &   $-$0.13 &        940 &       0.060 & N &    G \\
 646 &    Serp & J182952.20$+$011547.8 &            YSOc\_red &  9.6 &    1.54 &         84 &       2.6 &    1.41 &        110 &       4.0 & Y &    G \\
 647 &    Serp & J182952.21$+$011559.1 &            YSOc\_red &  9.6 &    1.87 &        230 &       0.024 &    1.95 &        250 &       0.068 & N &    G \\
 648 &    Serp & J182952.39$+$003553.0 & YSOc\_star$+$dust(IR2) & 40.0 &   $-$0.33 &        550 &       0.19 &   $-$1.44 &       3000 &       5.6 & N &    G \\
 649 &    Serp & J182952.44$+$003149.6 & YSOc\_star$+$dust(IR2) & 15.0 &   $-$0.64 &       1000 &       0.011 &   $-$1.12 &       2800 &       0.064 & N &    G \\
 650 &    Serp & J182952.52$+$003611.7 &            YSOc\_red &  9.6 &    0.77 &         54 &       0.69 &    0.64 &        100 &       0.85 & Y &    G \\
 651 &    Serp & J182952.85$+$011456.1 &            YSOc\_red &  9.6 &    1.49 &        120 &       1.2 &    1.39 &        170 &       2.1 & Y &    G \\
 652 &    Serp & J182953.04$+$004010.5 & YSOc\_star$+$dust(IR2) &  5.2 &   $-$1.02 &       1500 &       0.024 &   $-$1.08 &       3200 &       0.085 & N &    G \\
 653 &    Serp & J182953.05$+$003606.7 & YSOc\_star$+$dust(IR2) &  9.6 &    0.25 &        530 &       0.15 &   $-$0.22 &        860 &       0.57 & N &    G \\
 654 &    Serp & J182953.08$+$010034.7 & YSOc\_star$+$dust(IR1) &  8.6 &   $-$0.87 &       1200 &       0.035 &   $-$0.98 &       3100 &       0.15 & N &    G \\
 655 &    Serp & J182953.09$+$010617.9 & YSOc\_star$+$dust(IR1) &  5.5 &   $-$1.08 &       1500 &       0.030 &   $-$1.14 &       3100 &       0.099 & N &    G \\
 656 &    Serp & J182953.16$+$011227.7 &                YSOc &  8.4 &   $-$0.88 &       1300 &       0.0045 &   $-$1.21 &       3200 &       0.021 & N &    G \\
 657 &    Serp & J182953.59$+$011701.9 & YSOc\_star$+$dust(IR2) &  7.4 &   $-$1.24 &       1500 &       0.17 &   $-$1.45 &       3300 &       0.79 & N &    G \\
 658 &    Serp & J182953.83$+$011330.7 & YSOc\_star$+$dust(IR2) & 14.0 &   $-$0.90 &       1300 &       0.019 &   $-$1.29 &       3200 &       0.14 & N &    G \\
 659 &    Serp & J182954.08$+$010711.0 & YSOc\_star$+$dust(IR1) &  8.9 &   $-$0.62 &       1300 &       0.020 &   $-$0.76 &       2800 &       0.066 & N &    G \\
 660 &    Serp & J182954.23$+$004507.7 & YSOc\_star$+$dust(MP1) &  2.0 &   $-$2.19 &       2400 &       0.66 &   $-$2.16 &       2600 &       1.0 & N &    G \\
 661 &    Serp & J182954.31$+$003601.3 &                YSOc &  9.6 &   $-$0.18 &         52 &       0.55 &   $-$0.29 &        110 &       0.64 & Y &    G \\
 662 &    Serp & J182954.93$+$005914.1 & YSOc\_star$+$dust(IR4) &  6.3 &   $-$1.06 &       1500 &       0.033 &   $-$1.13 &       3200 &       0.13 & N &    G \\
 663 &    Serp & J182955.19$+$011322.4 & YSOc\_star$+$dust(IR2) & 17.0 &   $-$0.36 &        880 &       0.062 &   $-$0.72 &       3000 &       0.48 & N &    G \\
 664 &    Serp & J182955.32$+$004939.3 &                YSOc &  2.0 &   $-$0.84 &       1100 &       2.0 &   $-$0.75 &       1200 &       2.4 & N &    G \\
 665 &    Serp & J182955.38$+$005324.3 & YSOc\_star$+$dust(IR4) &  3.7 &   $-$1.63 &       1700 &       0.024 &   $-$1.60 &       3300 &       0.078 & N &    G \\
 666 &    Serp & J182955.69$+$011431.6 &                YSOc &  9.6 &   $-$0.23 &        810 &       0.28 &   $-$0.52 &       1100 &       1.2 & N &    G \\
 667 &    Serp & J182955.93$+$004015.0 & YSOc\_star$+$dust(IR1) & 11.0 &   $-$0.84 &       1400 &       0.040 &   $-$1.14 &       2200 &       0.18 & N &    G \\
 668 &    Serp & J182956.21$+$003339.2 &                YSOc & 15.0 &   $-$1.06 &       1000 &       0.033 &   $-$1.40 &       2800 &       0.19 & N &    G \\
 669 &    Serp & J182956.55$+$011259.6 & YSOc\_star$+$dust(IR1) & 14.2 &   $-$0.65 &       1000 &       0.089 &   $-$1.01 &       3000 &       0.59 & N &    G \\
 670 &    Serp & J182956.67$+$011239.2 &                YSOc &  9.6 &   $-$0.11 &        690 &       0.060 &    0.10 &        760 &       0.21 & N &    G \\
 671 &    Serp & J182956.87$+$011446.5 &                YSOc &  9.6 &    0.30 &        320 &       5.8 &    0.20 &        620 &       15 & Y &    G \\
 672 &    Serp & J182957.02$+$003300.3 & YSOc\_star$+$dust(IR1) &  7.5 &   $-$1.28 &       1400 &       1.4 &   $-$1.48 &       3200 &       6.0 & N &    G \\
 673 &    Serp & J182957.14$+$003318.5 & YSOc\_star$+$dust(IR1) &  4.0 &   $-$1.10 &       1200 &       0.42 &   $-$1.22 &       1400 &       0.60 & N &    G \\
 674 &    Serp & J182957.59$+$011300.5 &            YSOc\_red &  9.6 &    1.01 & $\leq$250 & $\geq$1.4 &    1.05 & $\leq$340 & $\geq$3.5 & Y &  L\_I \\
 675 &    Serp & J182957.63$+$010005.8 & YSOc\_star$+$dust(IR3) &  4.6 &   $-$1.38 &       1700 &       0.012 &   $-$1.45 &       3300 &       0.041 & N &    G \\
 676 &    Serp & J182957.66$+$011304.6 &            YSOc\_red &  9.6 &    0.27 &        560 &       0.15 &   $-$0.04 &        820 &       0.55 & N &    G \\
 677 &    Serp & J182957.73$+$011405.8 &              rising &  9.6 &    0.28 &        430 &       19 &   $-$0.19 &        800 &       48 & Y &    G \\
 678 &    Serp & J182957.81$+$011531.8 & YSOc\_star$+$dust(IR4) & 24.4 &   $-$0.86 &       1100 &       0.18 &   $-$1.42 &       3100 &       2.8 & N &    G \\
 679 &    Serp & J182957.81$+$011228.0 &                YSOc & 40.0 &   $-$0.42 &       1100 &       0.044 &   $-$1.65 &       3000 &       1.8 & N &    G \\
 680 &    Serp & J182957.84$+$011251.4 & YSOc\_star$+$dust(IR1) &  9.6 &    0.67 & $\leq$320 & $\geq$1.7 &    0.32 & $\leq$460 & $\geq$4.8 & Y &  L\_I \\
 681 &    Serp & J182957.85$+$011237.9 & YSOc\_star$+$dust(IR2) & 40.0 &   $-$0.38 &        880 &       0.14 &   $-$1.56 &       3100 &       6.1 & N &    G \\
 682 &    Serp & J182957.89$+$011246.2 &                YSOc & 40.0 &   $-$0.40 &        850 &       0.47 &   $-$1.53 &       3300 &       32 & N &    G \\
 683 &    Serp & J182958.19$+$011521.8 &                YSOc & 12.8 &   $-$0.36 &        890 &       0.57 &   $-$0.65 &       2800 &       2.6 & N &    G \\
 684 &    Serp & J182958.72$+$003620.5 & YSOc\_star$+$dust(IR2) &  5.4 &   $-$0.99 &       1500 &       0.049 &   $-$1.12 &       3200 &       0.17 & N &    G \\
 685 &    Serp & J182958.77$+$011426.2 &            YSOc\_red &  9.6 &    0.46 & $\leq$290 & $\geq$0.64 &    0.32 & $\leq$510 & $\geq$1.6 & Y &  L\_I \\
 686 &    Serp & J182959.03$+$011225.1 &            YSOc\_red &  9.6 &    0.22 &        360 &       0.013 &    0.26 &        380 &       0.040 & N &    G \\
 687 &    Serp & J182959.12$+$011120.3 & YSOc\_star$+$dust(MP1) &  8.1 &   $-$1.65 &       1700 &       0.037 &   $-$1.62 &       3400 &       0.21 & N &    G \\
 688 &    Serp & J182959.15$+$003735.5 & YSOc\_star$+$dust(IR2) &  2.9 &   $-$1.01 &       1600 &       0.019 &   $-$0.97 &       3200 &       0.051 & N &    G \\
 689 &    Serp & J182959.23$+$011407.8 & YSOc\_star$+$dust(IR1) &  7.7 &   $-$0.77 &       1200 &       0.59 &   $-$1.25 &       2900 &       2.2 & N &    G \\
 690 &    Serp & J182959.28$+$011401.7 &            YSOc\_red &  9.6 &    1.03 &         59 &       1.7 &    0.99 &         73 &       2.1 & Y &    G \\
 691 &    Serp & J182959.38$+$011041.1 &                YSOc &  9.6 &    0.51 &        440 &       0.0081 &    0.39 &        450 &       0.026 & N &    G \\
 692 &    Serp & J182959.57$+$011159.0 &            YSOc\_red &  9.6 &    1.15 & $\leq$330 & $\geq$1.3 &    1.35 & $\leq$380 & $\geq$3.6 & Y &  L\_I \\
 693 &    Serp & J182959.93$+$011311.6 &            YSOc\_red &  9.6 &    2.57 &        130 &       2.0 &    2.40 &        170 &       4.0 & Y &    G \\
 694 &    Serp & J183000.07$+$010305.7 & YSOc\_star$+$dust(IR4) &  6.7 &   $-$0.45 &       1300 &       0.037 &   $-$0.58 &       3200 &       0.16 & N &    G \\
 695 &    Serp & J183000.19$+$011403.7 & YSOc\_star$+$dust(IR1) &  9.6 &   $-$0.23 &        890 &       0.037 &   $-$0.58 &       1400 &       0.18 & N &    G \\
 696 &    Serp & J183000.30$+$010944.7 &                YSOc &  9.6 &   $-$0.12 &        520 &       0.097 &   $-$0.22 &        520 &       0.32 & N &    G \\
 697 &    Serp & J183000.48$+$003728.7 & YSOc\_star$+$dust(MP1) & 15.0 &   $-$1.07 &       1400 &       0.019 &   $-$1.33 &       2900 &       0.12 & N &    G \\
 698 &    Serp & J183000.71$+$011301.4 &            YSOc\_red &  9.6 &    1.68 &         54 &       1.3 &    1.69 &         60 &       1.5 & Y &    G \\
 699 &    Serp & J183001.10$+$011324.4 & YSOc\_star$+$dust(IR4) &  9.6 &   $-$0.16 &        670 &       0.041 &   $-$0.32 &        900 &       0.15 & N &    G \\
 700 &    Serp & J183001.67$+$010443.1 & YSOc\_star$+$dust(IR2) & 11.5 &   $-$0.59 &       1100 &       0.018 &   $-$0.90 &       3100 &       0.100 & N &    G \\
 701 &    Serp & J183001.79$+$003216.3 & YSOc\_star$+$dust(IR2) &  4.0 &   $-$1.01 &       1600 &       0.091 &   $-$1.07 &       1800 &       0.15 & N &    G \\
 702 &    Serp & J183002.08$+$011359.0 &            YSOc\_red &  9.6 &    0.36 &        510 &       0.091 &    0.30 &        730 &       0.31 & N &    G \\
 703 &    Serp & J183002.73$+$011228.2 &            YSOc\_red &  9.6 &    0.21 &        370 &       2.2 &    0.03 &        610 &       5.8 & Y &    G \\
 704 &    Serp & J183003.40$+$011619.4 & YSOc\_star$+$dust(IR3) &  5.9 &   $-$0.57 &       1400 &       0.21 &   $-$0.75 &       3100 &       0.74 & N &    G \\
 705 &    Serp & J183003.50$+$002345.0 & YSOc\_star$+$dust(IR2) &  3.0 &   $-$1.08 &       1600 &       0.056 &   $-$1.12 &       1800 &       0.081 & N &    G \\
 706 &    Serp & J183003.58$+$011641.0 & YSOc\_star$+$dust(IR4) & 20.0 &   $-$0.79 &        100 &       0.0070 &   $-$1.23 &       2900 &       0.075 & N &    G \\
 707 &    Serp & J183003.83$+$005340.7 & YSOc\_star$+$dust(IR4) &  3.5 &   $-$1.71 &       1800 &       0.024 &   $-$1.70 &       3400 &       0.079 & N &    G \\
 708 &    Serp & J183003.84$+$005620.6 & YSOc\_star$+$dust(IR3) &  3.2 &   $-$1.51 &       1700 &       0.018 &   $-$1.55 &       3300 &       0.054 & N &    G \\
 709 &    Serp & J183004.09$+$010656.0 & YSOc\_star$+$dust(IR3) &  9.6 &   $-$0.77 &       1300 &       0.0060 &   $-$0.92 &       3200 &       0.032 & N &    G \\
 710 &    Serp & J183004.90$+$011439.5 & YSOc\_star$+$dust(IR2) &  3.3 &   $-$1.25 &       1700 &       0.034 &   $-$1.36 &       3300 &       0.100 & N &    G \\
 711 &    Serp & J183005.01$+$011236.1 & YSOc\_star$+$dust(IR1) &  7.5 &   $-$0.92 &        130 &       0.0090 &   $-$1.06 &       3100 &       0.039 & N &    G \\
 712 &    Serp & J183005.26$+$004104.6 &                 red &  9.6 &    1.30 &        100 &       0.080 &    1.24 &        130 &       0.14 & Y &    G \\
 713 &    Serp & J183005.44$+$010102.4 & YSOc\_star$+$dust(IR4) &  4.5 &   $-$0.97 &       1600 &       0.027 &   $-$0.92 &       3300 &       0.091 & N &    G \\
 714 &    Serp & J183005.70$+$003931.8 &              rising & 30.0 &   $-$0.39 &        530 &       0.070 &   $-$0.14 &       2800 &       0.79 & N &    G \\
 715 &    Serp & J183006.09$+$010617.2 & YSOc\_star$+$dust(IR2) &  4.9 &   $-$0.79 &       1500 &       0.093 &   $-$0.90 &       3200 &       0.31 & N &    G \\
 716 &    Serp & J183006.41$+$010105.8 & YSOc\_star$+$dust(IR1) &  6.8 &   $-$0.78 &       1300 &       0.18 &   $-$0.98 &       3100 &       0.68 & N &    G \\
 717 &    Serp & J183007.70$+$011204.6 & YSOc\_star$+$dust(IR1) &  7.4 &   $-$0.79 &       1100 &       0.35 &   $-$0.96 &       2900 &       1.2 & N &    G \\
 718 &    Serp & J183008.50$+$010137.5 & YSOc\_star$+$dust(IR1) &  5.7 &   $-$0.70 &       1300 &       0.070 &   $-$0.76 &       3000 &       0.23 & N &    G \\
 719 &    Serp & J183008.62$+$005846.7 & YSOc\_star$+$dust(IR1) &  0.5 &   $-$0.48 &       1200 &       0.36 &   $-$0.43 &       1200 &       0.38 & N &    G \\
 720 &    Serp & J183008.92$+$004722.1 & YSOc\_star$+$dust(MP1) &  3.5 &   $-$1.37 &       1800 &       0.036 &   $-$1.23 &       3400 &       0.12 & N &    G \\
 721 &    Serp & J183009.21$+$011752.7 & YSOc\_star$+$dust(IR1) &  8.9 &   $-$0.87 &       1100 &       0.025 &   $-$1.02 &       2900 &       0.100 & N &    G \\
 722 &    Serp & J183009.43$+$010247.3 & YSOc\_star$+$dust(MP1) &  9.3 &   $-$1.92 &       1700 &       1.1 &   $-$2.14 &       3400 &       7.6 & N &    G \\
 723 &    Serp & J183010.84$+$004700.8 & YSOc\_star$+$dust(IR4) &  5.6 &   $-$1.47 &       2000 &       0.100 &   $-$1.51 &       3300 &       0.032 & N &    G \\
 724 &    Serp & J183011.10$+$011238.2 & YSOc\_star$+$dust(IR2) &  2.7 &   $-$0.71 &       1900 &       0.071 &   $-$0.82 &       2800 &       0.11 & N &    G \\
 725 &    Serp & J183013.28$+$010248.9 & YSOc\_star$+$dust(IR4) &  3.1 &   $-$1.31 &       1700 &       0.030 &   $-$1.28 &       3300 &       0.087 & N &    G \\
 726 &    Serp & J183013.96$+$010851.5 & YSOc\_star$+$dust(IR4) &  3.4 &   $-$1.04 &       2100 &       0.042 &   $-$1.07 &       3300 &       0.091 & N &    G \\
 727 &    Serp & J183016.98$+$011307.6 & YSOc\_star$+$dust(IR2) &  7.7 &   $-$0.63 &       1200 &       0.0061 &   $-$0.75 &       3100 &       0.025 & N &    G \\
 728 &    Serp & J183017.28$+$012132.9 & YSOc\_star$+$dust(MP1) &  7.5 &   $-$2.14 &       1800 &       1.9 &   $-$2.33 &       3400 &       11 & N &    G \\
 729 &    Serp & J183018.17$+$011416.9 & YSOc\_star$+$dust(IR2) &  9.6 &   $-$0.29 &       1200 &       0.13 &   $-$0.97 &       1800 &       0.85 & N &    G \\
 730 &    Serp & J183022.39$+$012044.0 & YSOc\_star$+$dust(MP1) &  2.1 &   $-$1.32 &       1800 &       0.044 &   $-$1.18 &       3400 &       0.12 & N &    G \\
 731 &    Serp & J183023.11$+$012009.8 & YSOc\_star$+$dust(MP1) &  1.9 &   $-$1.61 &       1900 &       0.032 &   $-$1.41 &       3400 &       0.086 & N &    G \\
 732 &    Serp & J183023.42$+$010504.8 & YSOc\_star$+$dust(IR1) &  4.4 &   $-$0.49 &       1200 &       0.071 &   $-$0.52 &       2900 &       0.19 & N &    G \\
 733 &     Oph & J162110.92$-$234328.7 & YSOc\_star$+$dust(MP1) &  7.6 &   $-$2.08 &       1900 &       3.0 &   $-$2.22 &       3500 &       19 & N &    G \\
 734 &     Oph & J162118.47$-$225457.9 & YSOc\_star$+$dust(IR2) &  2.7 &   $-$1.07 &       1600 &       0.055 &   $-$1.11 &       3200 &       0.15 & N &    G \\
 735 &     Oph & J162119.18$-$234228.6 & YSOc\_star$+$dust(MP1) &  0.0 &   $-$1.98 & $\geq$2200 & $\geq$1.8 &   $-$1.98 & $\geq$2200 & $\geq$1.8 & N & L\_II \\
 736 &     Oph & J162131.92$-$230140.2 & YSOc\_star$+$dust(IR2) &  6.8 &   $-$1.02 &       1400 &       0.100 &   $-$1.15 &       3200 &       0.41 & N &    G \\
 737 &     Oph & J162138.72$-$225328.3 & YSOc\_star$+$dust(IR1) &  9.8 &    1.07 &        470 &       0.0030 &    0.99 &        930 &       0.012 & N &    G \\
 738 &     Oph & J162141.98$-$231343.2 & YSOc\_star$+$dust(IR3) &  2.6 &   $-$1.47 &       1800 &       0.020 &   $-$1.44 &       3300 &       0.070 & N &    G \\
 739 &     Oph & J162145.13$-$234231.6 & YSOc\_star$+$dust(IR1) &  9.8 &    0.64 &        220 &       0.035 &    0.30 &        490 &       0.085 & N &    G \\
 740 &     Oph & J162148.47$-$234027.3 & YSOc\_star$+$dust(IR2) &  5.9 &   $-$0.33 &       1200 &       0.017 &   $-$0.41 &       2900 &       0.060 & N &    G \\
 741 &     Oph & J162157.67$-$242943.5 & YSOc\_star$+$dust(MP1) &  0.0 &   $-$2.37 & $\geq$2100 & $\geq$0.55 &   $-$2.37 & $\geq$2100 & $\geq$0.55 & N & L\_II \\
 742 &     Oph & J162218.52$-$232148.1 & YSOc\_star$+$dust(IR1) &  3.3 &   $-$0.74 &       1400 &       0.44 &   $-$0.79 &       3000 &       1.1 & N &    G \\
 743 &     Oph & J162220.99$-$230402.4 &         YSOc\_PAH$-$em &  9.8 &    0.93 &        550 &       0.010 &    0.17 &       1300 &       0.048 & N &    G \\
 744 &     Oph & J162224.41$-$245018.7 & YSOc\_star$+$dust(MP1) &  6.4 &   $-$2.17 &       1800 &       0.37 &   $-$2.37 &       3500 &       1.9 & N &    G \\
 745 &     Oph & J162224.95$-$232954.9 & YSOc\_star$+$dust(IR1) &  3.9 &   $-$0.99 &       1400 &       0.11 &   $-$1.07 &       3100 &       0.31 & N &    G \\
 746 &     Oph & J162235.63$-$233734.0 & YSOc\_star$+$dust(IR4) &  5.0 &   $-$1.29 &       1700 &       0.036 &   $-$1.41 &       3400 &       0.14 & N &    G \\
 747 &     Oph & J162241.75$-$242538.2 & YSOc\_star$+$dust(IR2) &  2.9 &   $-$1.31 &       1700 &       0.0049 &   $-$1.49 &       3300 &       0.010 & N &    G \\
 748 &     Oph & J162244.94$-$231713.4 & YSOc\_star$+$dust(IR2) &  3.4 &   $-$1.23 &       1700 &       0.0075 &   $-$1.28 &       3300 &       0.020 & N &    G \\
 749 &     Oph & J162245.39$-$243123.8 & YSOc\_star$+$dust(IR4) &  2.8 &   $-$0.83 &       1600 &       0.15 &   $-$0.71 &       3300 &       0.41 & N &    G \\
 750 &     Oph & J162247.18$-$230013.4 & YSOc\_star$+$dust(IR3) &  4.9 &   $-$1.42 &       1700 &       0.027 &   $-$1.56 &       3300 &       0.100 & N &    G \\
 751 &     Oph & J162248.64$-$230217.8 & YSOc\_star$+$dust(IR2) &  1.6 &   $-$1.01 &       1700 &       0.0060 &   $-$0.98 &       3300 &       0.020 & N &    G \\
 752 &     Oph & J162259.83$-$232635.0 & YSOc\_star$+$dust(MP1) &  3.6 &   $-$2.35 &       1900 &       0.13 &   $-$2.39 &       3500 &       0.47 & N &    G \\
 753 &     Oph & J162305.43$-$230256.7 & YSOc\_star$+$dust(IR2) &  9.8 &    0.47 &        650 &       0.0086 &   $-$0.27 &       1400 &       0.044 & N &    G \\
 754 &     Oph & J162305.87$-$233817.8 & YSOc\_star$+$dust(IR1) &  9.7 &   $-$1.25 &       1300 &       0.0019 &   $-$1.56 &       3200 &       0.010 & N &    G \\
 755 &     Oph & J162306.86$-$225736.6 &                YSOc &  9.8 &   $-$0.04 &        740 &       0.0043 &   $-$0.19 &       1100 &       0.019 & N &    G \\
 756 &     Oph & J162308.79$-$225742.6 & YSOc\_star$+$dust(IR2) &  4.8 &   $-$1.24 &       1600 &       0.16 &   $-$1.40 &       3200 &       0.58 & N &    G \\
 757 &     Oph & J162309.22$-$241704.6 & YSOc\_star$+$dust(IR1) &  7.7 &   $-$0.96 &       1200 &       0.41 &   $-$1.03 &       3100 &       1.7 & N &    G \\
 758 &     Oph & J162312.54$-$243641.3 & YSOc\_star$+$dust(MP1) &  5.0 &   $-$2.15 &       1800 &       0.18 &   $-$2.27 &       3500 &       0.75 & N &    G \\
 759 &     Oph & J162313.69$-$230358.2 & YSOc\_star$+$dust(IR3) &  2.2 &   $-$1.62 &       1800 &       0.0085 &   $-$1.63 &       3400 &       0.024 & N &    G \\
 760 &     Oph & J162315.63$-$234300.4 & YSOc\_star$+$dust(IR1) &  9.2 &   $-$0.70 &       1200 &       0.021 &   $-$0.94 &       3000 &       0.100 & N &    G \\
 761 &     Oph & J162332.21$-$242553.8 & YSOc\_star$+$dust(IR2) &  9.8 &    0.12 &        740 &       0.0024 &   $-$0.04 &       1300 &       0.011 & N &    G \\
 762 &     Oph & J162332.83$-$225846.8 & YSOc\_star$+$dust(IR4) &  2.2 &   $-$1.07 &       1700 &       0.046 &   $-$1.05 &       3300 &       0.12 & N &    G \\
 763 &     Oph & J162334.63$-$230846.6 & YSOc\_star$+$dust(MP1) &  5.3 &   $-$2.12 &       1800 &       0.81 &   $-$2.26 &       3500 &       3.5 & N &    G \\
 764 &     Oph & J162334.81$-$234030.1 & YSOc\_star$+$dust(IR2) &  6.3 &   $-$1.22 &       1500 &       0.21 &   $-$1.35 &       3300 &       0.91 & N &    G \\
 765 &     Oph & J162336.10$-$240220.9 & YSOc\_star$+$dust(IR1) &  3.4 &   $-$1.18 &       1400 &       0.068 &   $-$1.22 &       3100 &       0.18 & N &    G \\
 766 &     Oph & J162338.52$-$230544.7 & YSOc\_star$+$dust(IR3) &  3.1 &   $-$1.22 &       1700 &       0.013 &   $-$1.32 &       3300 &       0.040 & N &    G \\
 767 &     Oph & J162340.00$-$233337.4 &                YSOc &  9.8 &    0.03 &        450 &       0.0021 &    0.01 &        460 &       0.0070 & N &    G \\
 768 &     Oph & J162350.51$-$225838.0 & YSOc\_star$+$dust(IR2) &  1.6 &   $-$1.12 &       1700 &       0.056 &   $-$1.22 &       3200 &       0.14 & N &    G \\
 769 &     Oph & J162355.54$-$234210.5 & YSOc\_star$+$dust(MP1) &  7.7 &   $-$2.09 &       1700 &       1.3 &   $-$2.31 &       3400 &       7.4 & N &    G \\
 770 &     Oph & J162413.45$-$241822.1 & YSOc\_star$+$dust(IR1) &  7.7 &   $-$0.92 &       1300 &       0.067 &   $-$1.16 &       3000 &       0.26 & N &    G \\
 771 &     Oph & J162415.90$-$241114.9 & YSOc\_star$+$dust(IR2) &  5.8 &   $-$0.71 &       1400 &       0.010 &   $-$0.89 &       3100 &       0.040 & N &    G \\
 772 &     Oph & J162435.19$-$242619.7 & YSOc\_star$+$dust(IR4) &  5.1 &   $-$1.07 &       1500 &       0.024 &   $-$1.07 &       3300 &       0.090 & N &    G \\
 773 &     Oph & J162452.30$-$250127.0 & YSOc\_star$+$dust(IR1) &  3.6 &   $-$1.02 &       1600 &       0.0057 &   $-$1.04 &       3200 &       0.020 & N &    G \\
 774 &     Oph & J162453.02$-$250556.2 & YSOc\_star$+$dust(MP1) &  2.9 &   $-$2.47 &       1900 &       0.100 &   $-$2.52 &       3500 &       0.33 & N &    G \\
 775 &     Oph & J162459.76$-$245600.6 & YSOc\_star$+$dust(IR4) &  4.6 &   $-$1.28 &       1600 &       0.095 &   $-$1.36 &       3300 &       0.34 & N &    G \\
 776 &     Oph & J162502.08$-$245932.2 & YSOc\_star$+$dust(IR2) &  4.7 &   $-$0.49 &       1200 &       0.17 &   $-$0.64 &       2900 &       0.47 & N &    G \\
 777 &     Oph & J162506.22$-$244657.0 & YSOc\_star$+$dust(IR2) &  5.7 &   $-$0.89 &       1500 &       0.016 &   $-$0.99 &       3200 &       0.060 & N &    G \\
 778 &     Oph & J162506.91$-$235050.3 & YSOc\_star$+$dust(MP1) &  4.0 &   $-$1.10 &       1700 &       0.085 &   $-$0.97 &       3400 &       0.30 & N &    G \\
 779 &     Oph & J162522.14$-$241750.6 & YSOc\_star$+$dust(IR3) &  7.6 &   $-$1.06 &       1500 &       0.026 &   $-$1.31 &       3300 &       0.12 & N &    G \\
 780 &     Oph & J162522.59$-$243453.2 &                YSOc & 20.7 &   $-$0.68 &        870 &       0.019 &   $-$1.24 &       2800 &       0.15 & N &    G \\
 781 &     Oph & J162524.33$-$242944.3 & YSOc\_star$+$dust(IR1) &  2.7 &   $-$0.76 &       1400 &       0.13 &   $-$0.75 &       3000 &       0.32 & N &    G \\
 782 &     Oph & J162527.57$-$243647.6 & YSOc\_star$+$dust(IR1) &  9.8 &    0.36 &        860 &       0.020 &    0.06 &       1600 &       0.12 & N &    G \\
 783 &     Oph & J162532.11$-$235402.3 & YSOc\_star$+$dust(IR3) &  7.8 &   $-$2.25 &       1800 &       2.2 &   $-$2.52 &       3500 &       14 & N &    G \\
 784 &     Oph & J162532.52$-$232626.4 & YSOc\_star$+$dust(IR4) &  2.1 &   $-$1.10 &       1700 &       0.081 &   $-$0.92 &       3300 &       0.22 & N &    G \\
 785 &     Oph & J162533.15$-$232530.4 & YSOc\_star$+$dust(IR2) &  4.6 &   $-$1.20 &       1600 &       0.038 &   $-$1.26 &       3300 &       0.13 & N &    G \\
 786 &     Oph & J162535.49$-$243210.4 & YSOc\_star$+$dust(IR3) &  8.0 &   $-$1.18 &       1500 &       0.035 &   $-$1.49 &       3300 &       0.17 & N &    G \\
 787 &     Oph & J162536.72$-$241542.4 & YSOc\_star$+$dust(IR3) &  6.6 &   $-$0.82 &       1400 &       0.27 &   $-$1.04 &       3200 &       1.1 & N &    G \\
 788 &     Oph & J162538.11$-$242236.3 & YSOc\_star$+$dust(IR4) & 13.2 &   $-$0.79 &       1200 &       0.099 &   $-$1.03 &       3200 &       0.72 & N &    G \\
 789 &     Oph & J162539.42$-$232641.8 & YSOc\_star$+$dust(IR3) &  3.2 &   $-$1.13 &       1700 &       0.085 &   $-$1.19 &       3300 &       0.26 & N &    G \\
 790 &     Oph & J162539.58$-$242634.9 & YSOc\_star$+$dust(IR2) &  9.8 &   $-$0.30 &        980 &       0.23 &   $-$0.82 &       1500 &       1.3 & N &    G \\
 791 &     Oph & J162542.87$-$232526.0 & YSOc\_star$+$dust(IR2) &  3.7 &   $-$1.11 &       1600 &       0.13 &   $-$1.22 &       3300 &       0.40 & N &    G \\
 792 &     Oph & J162546.63$-$242336.0 &            YSOc\_red &  9.8 &   $-$0.06 &        690 &       0.0023 &   $-$0.28 &       1100 &       0.0095 & N &    G \\
 793 &     Oph & J162556.15$-$242048.1 & YSOc\_star$+$dust(IR2) &  4.5 &   $-$0.60 &       1300 &       0.71 &   $-$0.62 &       3100 &       2.2 & N &    G \\
 794 &     Oph & J162601.36$-$242520.4 & YSOc\_star$+$dust(IR1) & 12.6 &   $-$0.91 &       1200 &       0.023 &   $-$1.25 &       3100 &       0.15 & N &    G \\
 795 &     Oph & J162603.01$-$242336.0 & YSOc\_star$+$dust(IR4) &  5.7 &   $-$1.16 &       1400 &       1.9 &   $-$1.20 &       3300 &       7.3 & N &    G \\
 796 &     Oph & J162604.56$-$241751.5 & YSOc\_star$+$dust(IR4) & 14.9 &   $-$0.75 &       1200 &       0.0087 &   $-$1.14 &       3200 &       0.070 & N &    G \\
 797 &     Oph & J162605.76$-$244255.0 & YSOc\_star$+$dust(MP1) & 12.9 &   $-$2.02 &       1600 &       3.0 &   $-$2.41 &       3500 &       32 & N &    G \\
 798 &     Oph & J162607.03$-$242724.0 & YSOc\_star$+$dust(IR1) & 20.7 &   $-$0.56 &        890 &       0.068 &   $-$1.14 &       2900 &       0.60 & N &    G \\
 799 &     Oph & J162610.32$-$242054.6 &                YSOc & 27.0 &   $-$0.46 &        920 &       0.30 &   $-$1.31 &       3300 &       6.7 & N &    G \\
 800 &     Oph & J162614.63$-$242507.5 &                red1 &  0.0 & ... & ... & ... & ... & ... & ... & N &  O \\
 801 &     Oph & J162616.84$-$242222.9 & YSOc\_star$+$dust(IR1) & 10.8 &   $-$1.00 &       1200 &       0.40 &   $-$1.16 &       3100 &       2.1 & N &    G \\
 802 &     Oph & J162617.06$-$242021.4 & YSOc\_star$+$dust(IR3) &  4.2 &   $-$0.95 &       1600 &       0.34 &   $-$1.02 &       3300 &       1.2 & N &    G \\
 803 &     Oph & J162617.23$-$242345.1 &                YSOc &  9.8 &    0.69 &        490 &       0.083 &    0.68 &        570 &       0.28 & N &    G \\
 804 &     Oph & J162618.13$-$243033.0 & YSOc\_star$+$dust(IR4) & 13.3 &   $-$1.09 &       1300 &       0.012 &   $-$1.41 &       3300 &       0.098 & N &    G \\
 805 &     Oph & J162618.81$-$242610.4 & YSOc\_star$+$dust(IR2) & 10.1 &   $-$0.56 &       1200 &       0.010 &   $-$1.07 &       3100 &       0.051 & N &    G \\
 806 &     Oph & J162618.86$-$242819.6 &                YSOc & 19.7 &   $-$0.73 &        960 &       0.56 &   $-$1.30 &       3000 &       5.4 & N &    G \\
 807 &     Oph & J162618.98$-$242414.2 &                YSOc &  9.8 &   $-$0.14 &        760 &       0.027 &   $-$0.33 &       1000 &       0.11 & N &    G \\
 808 &     Oph & J162619.48$-$243727.4 & YSOc\_star$+$dust(IR4) &  1.6 &   $-$1.35 &       1800 &       0.054 &   $-$1.37 &       3400 &       0.14 & N &    G \\
 809 &     Oph & J162620.82$-$242839.4 & YSOc\_star$+$dust(IR2) & 16.7 &   $-$0.64 &        980 &       0.015 &   $-$0.93 &       3100 &       0.12 & N &    G \\
 810 &     Oph & J162620.96$-$240846.7 & YSOc\_star$+$dust(IR1) &  3.9 &   $-$0.99 &       1500 &       0.012 &   $-$1.08 &       3100 &       0.036 & N &    G \\
 811 &     Oph & J162621.35$-$242304.3 &              rising &  9.8 &    1.46 &        150 &       8.7 &    1.12 &        300 &       14 & Y &    G \\
 812 &     Oph & J162621.52$-$242600.9 & YSOc\_star$+$dust(IR3) &  4.6 &   $-$1.30 &       1600 &       0.026 &   $-$1.27 &       3300 &       0.088 & N &    G \\
 813 &     Oph & J162621.89$-$244439.8 & YSOc\_star$+$dust(IR1) &  3.7 &   $-$0.99 &       1500 &       0.030 &   $-$1.06 &       3200 &       0.088 & N &    G \\
 814 &     Oph & J162622.26$-$242407.0 &                YSOc &  9.8 &    0.19 &        720 &       0.0040 &   $-$0.15 &       1200 &       0.020 & N &    G \\
 815 &     Oph & J162622.94$-$242846.1 & YSOc\_star$+$dust(IR3) & 13.8 &   $-$0.73 &       1200 &       0.016 &   $-$1.20 &       3200 &       0.12 & N &    G \\
 816 &     Oph & J162623.40$-$242100.8 & YSOc\_star$+$dust(IR1) &  8.5 &   $-$0.62 &       1100 &       2.0 &   $-$0.88 &       3000 &       7.8 & N &    G \\
 817 &     Oph & J162623.57$-$242439.4 &                YSOc &  9.8 &   $-$0.01 &        670 &       0.26 &    0.01 &        810 &       0.97 & N &    G \\
 818 &     Oph & J162623.67$-$244314.0 & YSOc\_star$+$dust(IR3) &  4.0 &   $-$1.12 &       1500 &       0.45 &   $-$1.18 &       3200 &       1.4 & N &    G \\
 819 &     Oph & J162623.81$-$241829.0 & YSOc\_star$+$dust(IR4) &  9.0 &   $-$1.05 &       1300 &       0.0022 &   $-$1.13 &       3200 &       0.012 & N &    G \\
 820 &     Oph & J162624.04$-$242448.0 & YSOc\_star$+$dust(IR2) & 15.9 &   $-$0.59 &        930 &       1.1 &   $-$0.96 &       3000 &       7.8 & N &    G \\
 821 &     Oph & J162624.07$-$241613.4 &                YSOc & 13.3 &   $-$0.71 &        980 &       1.9 &   $-$1.12 &       3000 &       11 & N &    G \\
 822 &     Oph & J162625.46$-$242301.3 & YSOc\_star$+$dust(IR2) &  9.8 &    0.87 & $\leq$130 & $\geq$0.100 &    0.64 & $\leq$280 & $\geq$0.20 & Y &  L\_I \\
 823 &     Oph & J162625.62$-$242428.9 &                 red &  9.8 &    1.65 & $\leq$72 & $\geq$0.039 &    1.54 & $\leq$120 & $\geq$0.066 & Y &  L\_I \\
 824 &     Oph & J162625.99$-$242340.5 &                YSOc &  9.8 &    0.31 &        510 &       0.0064 &    0.22 &        510 &       0.021 & N &    G \\
 825 &     Oph & J162626.42$-$242430.0 &                red1 &  0.0 & ... & ... & ... & ... & ... & ... & N &  O \\
 826 &     Oph & J162627.53$-$244153.6 & YSOc\_star$+$dust(IR4) & 17.3 &   $-$0.51 &        750 &       0.098 &   $-$0.79 &       3100 &       0.73 & N &    G \\
 827 &     Oph & J162627.79$-$242641.7 & YSOc\_star$+$dust(IR2) &  7.3 &   $-$1.20 &       1400 &       0.0085 &   $-$1.35 &       3300 &       0.038 & N &    G \\
 828 &     Oph & J162632.97$-$240016.8 & YSOc\_star$+$dust(IR2) &  2.5 &   $-$0.95 &       1600 &       0.039 &   $-$1.07 &       3200 &       0.100 & N &    G \\
 829 &     Oph & J162636.82$-$241551.7 & YSOc\_star$+$dust(IR1) &  9.8 &    0.08 &        670 &       0.24 &   $-$0.35 &       1100 &       1.0 & N &    G \\
 830 &     Oph & J162637.79$-$243903.1 & YSOc\_star$+$dust(IR3) &  7.1 &   $-$1.10 &       1500 &       0.0043 &   $-$1.15 &       3200 &       0.019 & N &    G \\
 831 &     Oph & J162640.46$-$242714.3 &            YSOc\_red &  9.8 &    0.45 & $\leq$370 & $\geq$0.065 &    0.27 & $\leq$500 & $\geq$0.19 & Y &  L\_I \\
 832 &     Oph & J162640.83$-$243050.8 & YSOc\_star$+$dust(IR1) & 17.8 &   $-$0.52 &        920 &       0.0047 &   $-$0.93 &       3000 &       0.038 & N &    G \\
 833 &     Oph & J162641.25$-$244017.9 & YSOc\_star$+$dust(IR3) &  3.8 &   $-$1.27 &       1700 &       0.11 &   $-$1.35 &       3300 &       0.36 & N &    G \\
 834 &     Oph & J162642.13$-$243102.8 & YSOc\_star$+$dust(IR1) & 25.0 &   $-$0.39 &        790 &       0.035 &   $-$1.00 &       2900 &       0.40 & N &    G \\
 835 &     Oph & J162642.85$-$242029.7 & YSOc\_star$+$dust(IR3) &  9.7 &   $-$0.98 &       1400 &       0.41 &   $-$1.30 &       3200 &       2.4 & N &    G \\
 836 &     Oph & J162644.19$-$243448.4 &              rising &  9.8 &    2.49 &        290 &       1.1 &    2.44 &        440 &       2.6 & N &    G \\
 837 &     Oph & J162645.02$-$242307.6 & YSOc\_star$+$dust(IR1) & 18.5 &   $-$0.64 &        970 &       0.23 &   $-$1.17 &       3100 &       2.1 & N &    G \\
 838 &     Oph & J162646.42$-$241159.9 & YSOc\_star$+$dust(IR3) &  7.4 &   $-$1.39 &       1500 &       0.55 &   $-$1.58 &       3300 &       2.7 & N &    G \\
 839 &     Oph & J162648.47$-$242838.7 &            YSOc\_red &  9.8 &    0.02 &        430 &       0.12 &   $-$0.11 &        650 &       0.35 & Y &    G \\
 840 &     Oph & J162648.64$-$235634.1 & YSOc\_star$+$dust(IR1) &  6.3 &   $-$0.77 &       1200 &       0.32 &   $-$0.85 &       3000 &       1.1 & N &    G \\
 841 &     Oph & J162648.96$-$243825.1 &                YSOc & 14.5 &   $-$0.93 &       1100 &       0.075 &   $-$1.27 &       3100 &       0.55 & N &    G \\
 842 &     Oph & J162651.95$-$243039.4 &                YSOc &  9.8 &   $-$0.15 &        680 &       0.011 &   $-$0.16 &        820 &       0.041 & N &    G \\
 843 &     Oph & J162653.47$-$243236.1 &            YSOc\_red &  9.8 &   $-$0.23 &        640 &       0.014 &   $-$0.26 &        800 &       0.048 & N &    G \\
 844 &     Oph & J162654.29$-$242437.9 &                YSOc &  9.8 &   $-$0.29 &        720 &       0.0091 &   $-$0.22 &        860 &       0.034 & N &    G \\
 845 &     Oph & J162654.43$-$242620.6 & YSOc\_star$+$dust(IR2) & 20.6 &   $-$0.92 &       1100 &       0.076 &   $-$1.51 &       3200 &       0.95 & N &    G \\
 846 &     Oph & J162654.76$-$242702.1 & YSOc\_star$+$dust(IR4) & 21.1 &   $-$0.41 &        820 &       0.0080 &   $-$0.90 &       2600 &       0.060 & N &    G \\
 847 &     Oph & J162656.43$-$243301.5 &                YSOc &  0.0 &   $-$0.44 & $\geq$540 & $\geq$0.0032 &   $-$0.44 & $\geq$540 & $\geq$0.0030 & N & L\_II \\
 848 &     Oph & J162656.76$-$241351.3 & YSOc\_star$+$dust(IR3) & 11.7 &   $-$1.01 &       1300 &       0.13 &   $-$1.31 &       3200 &       0.83 & N &    G \\
 849 &     Oph & J162657.32$-$243538.6 &                YSOc & 24.3 &   $-$0.66 &        940 &       0.0063 &   $-$1.41 &       2800 &       0.078 & N &    G \\
 850 &     Oph & J162658.27$-$243740.7 &                YSOc &  9.8 &   $-$0.29 &        710 &       0.0053 &   $-$0.29 &        870 &       0.019 & N &    G \\
 851 &     Oph & J162658.38$-$242129.9 & YSOc\_star$+$dust(IR3) & 19.8 &   $-$0.84 &       1100 &       0.019 &   $-$1.36 &       3200 &       0.23 & N &    G \\
 852 &     Oph & J162658.42$-$244531.8 & YSOc\_star$+$dust(IR1) & 10.7 &   $-$0.45 &        860 &       1.2 &   $-$0.86 &       2600 &       4.5 & N &    G \\
 853 &     Oph & J162658.62$-$241834.5 & YSOc\_star$+$dust(IR2) & 16.8 &   $-$0.72 &       1100 &       0.018 &   $-$1.18 &       3200 &       0.17 & N &    G \\
 854 &     Oph & J162658.65$-$242455.4 &                YSOc & 17.2 &   $-$0.48 &        820 &       0.0026 &   $-$1.01 &       2300 &       0.012 & N &    G \\
 855 &     Oph & J162659.04$-$243556.8 & YSOc\_star$+$dust(IR4) & 18.2 &   $-$1.01 &       1200 &       0.011 &   $-$1.39 &       3300 &       0.14 & N &    G \\
 856 &     Oph & J162659.10$-$243503.3 &                 red &  9.8 &    1.99 &        110 &       1.5 &    1.91 &        150 &       2.7 & N &    G \\
 857 &     Oph & J162702.32$-$243727.2 &              rising &  9.8 &    1.53 &        320 &       4.8 &    0.58 &        540 &       12 & Y &    G \\
 858 &     Oph & J162702.99$-$242614.6 &                YSOc &  9.8 &   $-$0.19 &        680 &       0.020 &   $-$0.29 &        860 &       0.073 & N &    G \\
 859 &     Oph & J162703.58$-$242005.4 & YSOc\_star$+$dust(IR1) &  9.8 &   $-$0.09 &        750 &       0.0048 &   $-$0.46 &       1200 &       0.021 & N &    G \\
 860 &     Oph & J162704.10$-$242829.9 & YSOc\_star$+$dust(IR2) &  9.8 &    0.04 &        640 &       0.078 &   $-$0.28 &        870 &       0.30 & N &    G \\
 861 &     Oph & J162704.56$-$242715.6 & YSOc\_star$+$dust(IR4) & 23.6 &   $-$0.43 &        830 &       0.036 &   $-$0.97 &       3000 &       0.44 & N &    G \\
 862 &     Oph & J162705.24$-$243629.6 &            YSOc\_red &  9.8 &    1.27 &        110 &       0.15 &    1.14 &        170 &       0.25 & Y &    G \\
 863 &     Oph & J162705.65$-$244013.0 & YSOc\_star$+$dust(IR4) & 20.3 &   $-$0.76 &        880 &       0.0033 &   $-$1.24 &       2200 &       0.019 & N &    G \\
 864 &     Oph & J162705.96$-$242618.4 & YSOc\_star$+$dust(IR4) & 28.6 &   $-$1.07 &       1000 &       0.032 &   $-$1.84 &       3200 &       0.77 & N &    G \\
 865 &     Oph & J162705.96$-$242836.1 & YSOc\_star$+$dust(IR3) & 15.2 &   $-$0.74 &       1100 &       0.0044 &   $-$1.10 &       3200 &       0.037 & N &    G \\
 866 &     Oph & J162706.58$-$244148.8 & YSOc\_star$+$dust(IR2) &  4.6 &   $-$0.87 &       1500 &       0.032 &   $-$0.90 &       3200 &       0.100 & N &    G \\
 867 &     Oph & J162706.75$-$243814.8 &            YSOc\_red &  9.8 &    0.61 &        310 &       0.60 &    0.68 &        430 &       1.5 & Y &    G \\
 868 &     Oph & J162709.07$-$241200.8 & YSOc\_star$+$dust(IR3) &  9.6 &   $-$1.23 &       1400 &       0.065 &   $-$1.51 &       3300 &       0.39 & N &    G \\
 869 &     Oph & J162709.09$-$243408.0 & YSOc\_star$+$dust(IR2) & 15.0 &   $-$0.91 &       1000 &       0.22 &   $-$1.26 &       3100 &       1.6 & N &    G \\
 870 &     Oph & J162709.34$-$244022.3 & YSOc\_star$+$dust(IR3) &  9.8 &   $-$0.09 &        720 &       0.044 &   $-$0.38 &        940 &       0.18 & N &    G \\
 871 &     Oph & J162709.40$-$243718.6 &              rising &  9.8 &    1.69 &        260 &       18 &    0.55 &        350 &       41 & Y &    G \\
 872 &     Oph & J162711.17$-$244046.5 &                YSOc &  9.8 &   $-$0.05 &        570 &       0.23 &   $-$0.17 &        750 &       0.77 & N &    G \\
 873 &     Oph & J162711.70$-$243831.9 &                YSOc & 35.7 &   $-$0.43 &        750 &       0.15 &   $-$2.29 &       3200 &       37 & N &    G \\
 874 &     Oph & J162712.12$-$243449.0 &                YSOc & 17.7 &   $-$0.82 &       1000 &       0.022 &   $-$1.24 &       3100 &       0.19 & N &    G \\
 875 &     Oph & J162713.26$-$244133.4 &                YSOc & 40.9 &   $-$2.01 &       1100 &       0.11 &   $-$3.24 &       3200 &       9.6 & N &    G \\
 876 &     Oph & J162713.71$-$241816.7 & YSOc\_star$+$dust(IR3) & 11.5 &   $-$0.96 &       1300 &       0.13 &   $-$1.23 &       3200 &       0.80 & N &    G \\
 877 &     Oph & J162713.81$-$244331.6 & YSOc\_star$+$dust(IR2) &  9.8 &   $-$0.22 &        830 &       0.093 &   $-$0.85 &       1400 &       0.46 & N &    G \\
 878 &     Oph & J162714.49$-$242645.9 &                YSOc &  9.8 &   $-$0.01 &        660 &       0.034 &   $-$0.05 &        770 &       0.12 & N &    G \\
 879 &     Oph & J162715.11$-$245138.8 & YSOc\_star$+$dust(IR2) &  2.3 &   $-$1.06 &       1700 &       0.11 &   $-$0.99 &       3300 &       0.29 & N &    G \\
 880 &     Oph & J162715.44$-$242639.6 &                YSOc & 30.9 &   $-$0.39 &        760 &       0.11 &   $-$1.20 &       2700 &       1.4 & N &    G \\
 881 &     Oph & J162715.50$-$243053.6 &                YSOc &  9.8 &    0.01 &        650 &       0.019 &   $-$0.05 &        770 &       0.071 & N &    G \\
 882 &     Oph & J162715.87$-$242513.9 & YSOc\_star$+$dust(IR2) &  9.8 &   $-$0.09 &        680 &       0.010 &   $-$0.26 &        870 &       0.038 & N &    G \\
 883 &     Oph & J162715.89$-$243843.2 &      star$+$dust(IR2) & 18.6 &   $-$0.70 &        220 &       0.62 &   $-$0.64 &        220 &       0.62 & Y &    G \\
 884 &     Oph & J162716.39$-$243114.5 &                YSOc &  9.8 &    0.16 &        550 &       0.025 &    0.13 &        590 &       0.081 & N &    G \\
 885 &     Oph & J162717.58$-$242856.2 &                YSOc &  9.8 &    0.25 &         68 &       2.6 &    0.33 &        130 &       3.2 & Y &    G \\
 886 &     Oph & J162717.58$-$240513.6 & YSOc\_star$+$dust(IR1) &  6.4 &   $-$0.75 &       1000 &       0.074 &   $-$0.90 &       2400 &       0.18 & N &    G \\
 887 &     Oph & J162718.37$-$243914.6 &                YSOc &  9.8 &    0.18 &        590 &       0.048 &    0.16 &        690 &       0.17 & N &    G \\
 888 &     Oph & J162718.47$-$242905.8 & YSOc\_star$+$dust(IR1) & 21.9 &   $-$0.59 &        930 &       0.13 &   $-$1.25 &       3000 &       1.5 & N &    G \\
 889 &     Oph & J162719.20$-$242843.8 &                YSOc &  9.8 &   $-$0.03 &        660 &       0.088 &    0.04 &        750 &       0.31 & N &    G \\
 890 &     Oph & J162721.45$-$244143.0 &                YSOc &  9.8 &   $-$0.03 &        600 &       1.2 &   $-$0.10 &        740 &       4.2 & Y &    G \\
 891 &     Oph & J162721.79$-$242953.1 &                YSOc &  9.8 &    0.72 &        410 &       0.88 &    0.98 &        480 &       2.6 & N &    G \\
 892 &     Oph & J162721.82$-$242727.6 &            YSOc\_red &  9.8 &   $-$0.05 &        180 &       0.019 &   $-$0.07 &        420 &       0.035 & Y &    G \\
 893 &     Oph & J162722.96$-$244807.1 & YSOc\_star$+$dust(IR2) &  3.9 &   $-$1.04 &       1600 &       0.11 &   $-$1.19 &       3200 &       0.35 & N &    G \\
 894 &     Oph & J162724.58$-$244103.1 &            YSOc\_red &  9.8 &    1.01 & $\leq$300 & $\geq$0.19 &    1.22 & $\leq$350 & $\geq$0.53 & Y &  L\_I \\
 895 &     Oph & J162724.63$-$242935.2 & YSOc\_star$+$dust(MP1) & 29.1 &   $-$1.45 &       1100 &       0.0069 &   $-$2.21 &       3100 &       0.19 & N &    G \\
 896 &     Oph & J162726.21$-$241923.0 & YSOc\_star$+$dust(IR2) & 14.2 &   $-$0.93 &       1200 &       0.0047 &   $-$1.37 &       3200 &       0.035 & N &    G \\
 897 &     Oph & J162726.27$-$244246.1 & YSOc\_star$+$dust(IR3) &  9.8 &    0.08 &        610 &       0.018 &   $-$0.17 &        810 &       0.065 & N &    G \\
 898 &     Oph & J162726.57$-$242554.2 & YSOc\_star$+$dust(IR1) &  2.0 &   $-$0.76 &       1500 &       0.013 &   $-$0.81 &       3100 &       0.030 & N &    G \\
 899 &     Oph & J162726.91$-$244050.7 &              rising &  9.8 &    1.17 &        160 &       3.8 &    1.03 &        310 &       6.0 & Y &    G \\
 900 &     Oph & J162727.37$-$243116.6 & YSOc\_star$+$dust(IR4) & 11.9 &   $-$0.94 &       1300 &       0.11 &   $-$1.19 &       3200 &       0.77 & N &    G \\
 901 &     Oph & J162727.99$-$243933.4 &              rising &  9.8 &    2.29 &        110 &       15 &    1.96 &        180 &       27 & Y &    G \\
 902 &     Oph & J162728.44$-$242721.0 &                YSOc &  9.8 &   $-$0.03 &        310 &       0.48 &   $-$0.16 &        600 &       1.1 & Y &    G \\
 903 &     Oph & J162729.94$-$243336.4 &                YSOc & 28.9 &   $-$1.38 &       1000 &       0.0099 &   $-$3.12 &       2700 &       0.28 & N &    G \\
 904 &     Oph & J162730.17$-$242743.2 &                YSOc &  9.8 &   $-$0.12 &        530 &       0.93 &   $-$0.12 &        720 &       2.9 & Y &    G \\
 905 &     Oph & J162730.83$-$242455.9 & YSOc\_star$+$dust(IR2) &  9.8 &   $-$0.14 &        850 &       0.097 &   $-$0.74 &       1500 &       0.52 & N &    G \\
 906 &     Oph & J162730.91$-$242733.2 &                YSOc &  9.8 &    0.88 &        460 &       0.037 &    0.86 &        500 &       0.12 & N &    G \\
 907 &     Oph & J162732.12$-$242943.5 & YSOc\_star$+$dust(IR4) & 23.9 &   $-$0.52 &        860 &       0.0063 &   $-$1.07 &       2800 &       0.073 & N &    G \\
 908 &     Oph & J162732.64$-$243323.4 & YSOc\_star$+$dust(IR4) & 23.6 &   $-$0.92 &       1100 &       0.030 &   $-$1.50 &       3200 &       0.54 & N &    G \\
 909 &     Oph & J162732.71$-$244500.3 & YSOc\_star$+$dust(MP1) & 18.0 &   $-$1.48 &       1100 &       0.0033 &   $-$1.88 &       2700 &       0.025 & N &    G \\
 910 &     Oph & J162732.84$-$243234.7 & YSOc\_star$+$dust(IR2) & 23.5 &   $-$0.46 &        880 &       0.046 &   $-$1.22 &       3000 &       0.56 & N &    G \\
 911 &     Oph & J162733.10$-$244115.2 & YSOc\_star$+$dust(IR4) & 14.4 &   $-$0.88 &       1200 &       0.45 &   $-$1.28 &       3200 &       3.9 & N &    G \\
 912 &     Oph & J162736.16$-$240457.5 & YSOc\_star$+$dust(IR3) &  7.5 &   $-$1.26 &       1400 &       0.0077 &   $-$1.44 &       3300 &       0.036 & N &    G \\
 913 &     Oph & J162736.65$-$235826.8 & YSOc\_star$+$dust(IR3) &  4.4 &   $-$1.23 &       1700 &       0.013 &   $-$1.35 &       3400 &       0.046 & N &    G \\
 914 &     Oph & J162737.23$-$244237.9 &            YSOc\_red &  9.8 &    0.13 &        450 &       0.13 &    0.18 &        570 &       0.43 & Y &    G \\
 915 &     Oph & J162737.43$-$241754.8 & YSOc\_star$+$dust(IR2) &  7.5 &   $-$0.89 &       1400 &       0.011 &   $-$1.10 &       3200 &       0.046 & N &    G \\
 916 &     Oph & J162738.31$-$243658.4 & YSOc\_star$+$dust(IR3) & 12.3 &   $-$0.73 &       1100 &       0.36 &   $-$1.06 &       3100 &       2.2 & N &    G \\
 917 &     Oph & J162738.33$-$235732.1 & YSOc\_star$+$dust(IR4) &  6.2 &   $-$1.00 &       1400 &       0.40 &   $-$1.17 &       3200 &       1.6 & N &    G \\
 918 &     Oph & J162738.61$-$243839.1 & YSOc\_star$+$dust(IR2) &  7.4 &   $-$0.49 &       1200 &       0.027 &   $-$0.66 &       3100 &       0.11 & N &    G \\
 919 &     Oph & J162738.93$-$244020.5 & YSOc\_star$+$dust(IR1) &  9.8 &    0.64 &        290 &       0.072 &    0.20 &        510 &       0.20 & N &    G \\
 920 &     Oph & J162739.01$-$235818.3 & YSOc\_star$+$dust(IR3) &  4.8 &   $-$1.09 &       1600 &       0.30 &   $-$1.27 &       3300 &       1.1 & N &    G \\
 921 &     Oph & J162739.41$-$243915.3 & YSOc\_star$+$dust(IR2) &  7.9 &   $-$0.37 &       1000 &       0.38 &   $-$0.60 &       2900 &       1.4 & N &    G \\
 922 &     Oph & J162739.81$-$244315.0 &                YSOc &  9.8 &   $-$0.15 &        570 &       0.71 &   $-$0.15 &        700 &       2.6 & Y &    G \\
 923 &     Oph & J162740.10$-$242636.3 &                YSOc & 19.4 &   $-$0.75 &        860 &       0.0037 &   $-$1.19 &       2500 &       0.024 & N &    G \\
 924 &     Oph & J162740.27$-$242204.0 & YSOc\_star$+$dust(IR1) &  2.3 &   $-$1.07 &       1600 &       0.88 &   $-$1.00 &       3200 &       2.3 & N &    G \\
 925 &     Oph & J162741.48$-$243537.5 & YSOc\_star$+$dust(MP1) & 15.6 &   $-$1.98 &       1400 &       0.027 &   $-$2.34 &       3400 &       0.33 & N &    G \\
 926 &     Oph & J162741.60$-$244644.6 &                YSOc &  9.8 &    0.32 &        350 &       0.022 &    0.18 &        620 &       0.058 & N &    G \\
 927 &     Oph & J162741.74$-$244336.0 & YSOc\_star$+$dust(IR2) &  9.8 &   $-$0.20 &        720 &       0.023 &   $-$0.30 &        880 &       0.090 & N &    G \\
 928 &     Oph & J162741.78$-$244234.6 & YSOc\_star$+$dust(IR4) & 13.8 &   $-$0.33 &        750 &       0.0014 &   $-$0.55 &       2300 &       0.0050 & N &    G \\
 929 &     Oph & J162742.69$-$243850.5 & YSOc\_star$+$dust(IR4) & 10.2 &   $-$1.28 &       1500 &       0.030 &   $-$1.51 &       3400 &       0.21 & N &    G \\
 930 &     Oph & J162743.77$-$244307.8 &                YSOc & 30.9 &   $-$1.78 &       1100 &       0.022 &   $-$3.17 &       3000 &       0.67 & N &    G \\
 931 &     Oph & J162745.00$-$240628.2 & YSOc\_star$+$dust(IR3) &  9.1 &   $-$1.25 &       1400 &       0.025 &   $-$1.43 &       3300 &       0.14 & N &    G \\
 932 &     Oph & J162745.77$-$244453.8 &                YSOc &  9.8 &    0.11 &        450 &       0.055 &    0.10 &        640 &       0.16 & N &    G \\
 933 &     Oph & J162746.28$-$243141.1 & YSOc\_star$+$dust(IR3) &  9.1 &   $-$0.88 &       1400 &       0.017 &   $-$1.15 &       3200 &       0.093 & N &    G \\
 934 &     Oph & J162747.08$-$244535.0 & YSOc\_star$+$dust(IR2) & 20.3 &   $-$0.72 &        990 &       0.031 &   $-$1.29 &       3100 &       0.34 & N &    G \\
 935 &     Oph & J162748.23$-$244225.4 &            YSOc\_red &  9.8 &    1.55 &        260 &       0.014 &    1.12 &        380 &       0.042 & N &    G \\
 936 &     Oph & J162749.77$-$242521.9 & YSOc\_star$+$dust(IR2) &  9.7 &   $-$1.28 &       1400 &       0.050 &   $-$1.55 &       3300 &       0.29 & N &    G \\
 937 &     Oph & J162751.79$-$243145.4 &            YSOc\_red &  9.8 &    0.03 &        500 &       0.79 &   $-$0.26 &        740 &       2.5 & N &    G \\
 938 &     Oph & J162755.24$-$242839.5 & YSOc\_star$+$dust(IR3) &  7.7 &   $-$0.91 &       1400 &       0.029 &   $-$1.13 &       3200 &       0.13 & N &    G \\
 939 &     Oph & J162755.24$-$240215.4 & YSOc\_star$+$dust(IR3) &  4.8 &   $-$1.06 &       1600 &       0.0085 &   $-$1.19 &       3300 &       0.031 & N &    G \\
 940 &     Oph & J162755.57$-$242617.9 & YSOc\_star$+$dust(IR2) &  2.4 &   $-$1.08 &       1600 &       0.18 &   $-$1.17 &       3200 &       0.47 & N &    G \\
 941 &     Oph & J162758.89$-$243514.6 &                YSOc &  6.5 &   $-$0.63 &        900 &       0.0018 &   $-$0.81 &       1800 &       0.0036 & N &    G \\
 942 &     Oph & J162802.58$-$235503.6 & YSOc\_star$+$dust(IR4) &  4.3 &   $-$1.06 &       1800 &       0.043 &   $-$1.12 &       3400 &       0.16 & N &    G \\
 943 &     Oph & J162804.53$-$243448.4 & YSOc\_star$+$dust(IR4) & 26.3 &   $-$0.81 &        880 &       0.010 &   $-$1.44 &       2600 &       0.12 & N &    G \\
 944 &     Oph & J162804.77$-$245035.5 & YSOc\_star$+$dust(IR1) &  4.5 &   $-$0.74 &       1400 &       0.0081 &   $-$0.84 &       3100 &       0.025 & N &    G \\
 945 &     Oph & J162804.78$-$243710.0 & YSOc\_star$+$dust(MP1) & 13.2 &   $-$2.13 &       1500 &       0.033 &   $-$2.44 &       3400 &       0.32 & N &    G \\
 946 &     Oph & J162808.07$-$235304.1 &                YSOc &  6.1 &   $-$2.30 &       1900 &       0.14 &   $-$2.50 &       3500 &       0.71 & N &    G \\
 947 &     Oph & J162812.70$-$241135.5 & YSOc\_star$+$dust(IR3) &  9.2 &   $-$0.88 &       1300 &       0.022 &   $-$1.11 &       3200 &       0.12 & N &    G \\
 948 &     Oph & J162813.69$-$243138.8 & YSOc\_star$+$dust(IR1) &  5.3 &   $-$1.55 &       1500 &       0.0018 &   $-$1.36 &       3200 &       0.0067 & N &    G \\
 949 &     Oph & J162813.78$-$243249.4 & YSOc\_star$+$dust(IR2) &  7.7 &   $-$1.10 &       1400 &       0.055 &   $-$1.39 &       3200 &       0.26 & N &    G \\
 950 &     Oph & J162816.50$-$243657.9 & YSOc\_star$+$dust(IR2) &  6.3 &   $-$0.80 &       1200 &       0.14 &   $-$0.92 &       3100 &       0.48 & N &    G \\
 951 &     Oph & J162816.72$-$240514.2 & YSOc\_star$+$dust(IR2) &  7.1 &   $-$1.33 &       1600 &       0.15 &   $-$1.50 &       3400 &       0.72 & N &    G \\
 952 &     Oph & J162817.73$-$241705.0 & YSOc\_star$+$dust(IR4) &  7.8 &   $-$1.21 &       1500 &       0.0067 &   $-$1.29 &       3300 &       0.033 & N &    G \\
 953 &     Oph & J162821.50$-$242154.9 & YSOc\_star$+$dust(MP1) &  5.9 &   $-$2.27 &       1800 &       0.040 &   $-$2.33 &       3400 &       0.19 & N &    G \\
 954 &     Oph & J162821.61$-$243623.4 &            YSOc\_red &  9.8 &    1.23 &         41 &       0.29 &    1.14 &         49 &       0.34 & Y &    G \\
 955 &     Oph & J162821.69$-$244247.1 & YSOc\_star$+$dust(IR1) & 19.0 &   $-$0.68 &        970 &       0.0095 &   $-$1.13 &       3100 &       0.091 & N &    G \\
 956 &     Oph & J162823.32$-$242240.5 & YSOc\_star$+$dust(IR2) & 12.7 &   $-$1.16 &       1200 &       0.23 &   $-$1.42 &       3200 &       1.6 & N &    G \\
 957 &     Oph & J162832.66$-$242244.8 & YSOc\_star$+$dust(IR2) &  5.8 &   $-$1.70 &       1600 &       1.0 &   $-$1.94 &       3300 &       4.2 & N &    G \\
 958 &     Oph & J162845.26$-$242818.8 & YSOc\_star$+$dust(IR1) &  2.3 &   $-$0.78 &       1300 &       0.58 &   $-$0.85 &       2800 &       1.3 & N &    G \\
 959 &     Oph & J162848.70$-$242631.7 & YSOc\_star$+$dust(IR3) &  3.0 &   $-$1.50 &       1700 &       0.0032 &   $-$1.66 &       3400 &       0.0097 & N &    G \\
 960 &     Oph & J162854.06$-$244744.3 & YSOc\_star$+$dust(IR4) &  5.2 &   $-$0.93 &       1400 &       0.18 &   $-$0.84 &       3200 &       0.62 & N &    G \\
 961 &     Oph & J162856.03$-$233106.9 & YSOc\_star$+$dust(IR3) &  3.3 &   $-$1.23 &       1700 &       0.0092 &   $-$1.28 &       3300 &       0.029 & N &    G \\
 962 &     Oph & J162856.93$-$243109.6 & YSOc\_star$+$dust(IR2) &  2.9 &   $-$0.92 &       1600 &       0.028 &   $-$0.97 &       3200 &       0.077 & N &    G \\
 963 &     Oph & J162857.85$-$244054.9 &            YSOc\_red &  9.8 &    0.67 &        300 &       0.030 &    0.59 &        450 &       0.081 & Y &    G \\
 964 &     Oph & J162903.20$-$242748.9 & YSOc\_star$+$dust(IR2) &  2.4 &   $-$1.32 &       1700 &       0.019 &   $-$1.33 &       3300 &       0.050 & N &    G \\
 965 &     Oph & J162908.22$-$241546.8 & YSOc\_star$+$dust(IR4) &  6.9 &   $-$1.06 &       1500 &       0.018 &   $-$1.06 &       3300 &       0.084 & N &    G \\
 966 &     Oph & J162923.38$-$241356.7 & YSOc\_star$+$dust(MP1) & 10.4 &   $-$1.81 &       1400 &       0.82 &   $-$2.06 &       3300 &       5.4 & N &    G \\
 967 &     Oph & J162935.09$-$243610.4 & YSOc\_star$+$dust(MP1) &  4.2 &   $-$2.09 &       1800 &       0.068 &   $-$2.21 &       3400 &       0.25 & N &    G \\
 968 &     Oph & J162944.28$-$244121.8 & YSOc\_star$+$dust(MP1) &  0.8 &   $-$1.67 &       1900 &       0.13 &   $-$1.55 &       3400 &       0.30 & N &    G \\
 969 &     Oph & J162948.31$-$233103.3 & YSOc\_star$+$dust(IR4) &  1.7 &   $-$1.54 &       1800 &       0.0095 &   $-$1.45 &       3300 &       0.024 & N &    G \\
 970 &     Oph & J162954.58$-$245846.1 & YSOc\_star$+$dust(MP1) &  0.0 &   $-$2.44 & $\geq$2200 & $\geq$0.78 &   $-$2.44 & $\geq$2200 & $\geq$0.78 & N & L\_II \\
 971 &     Oph & J163002.21$-$242007.3 & YSOc\_star$+$dust(MP1) &  4.4 &   $-$2.39 &       1900 &       0.93 &   $-$2.54 &       3500 &       3.7 & N &    G \\
 972 &     Oph & J163019.76$-$240256.3 & YSOc\_star$+$dust(MP1) &  5.4 &   $-$1.89 &       1800 &       0.013 &   $-$1.80 &       3400 &       0.055 & N &    G \\
 973 &     Oph & J163020.04$-$233108.3 & YSOc\_star$+$dust(IR4) &  2.7 &   $-$1.79 &       1900 &       0.053 &   $-$1.83 &       3400 &       0.16 & N &    G \\
 974 &     Oph & J163023.39$-$245416.1 & YSOc\_star$+$dust(IR2) &  4.2 &   $-$0.63 &       1300 &       0.14 &   $-$0.73 &       3000 &       0.41 & N &    G \\
 975 &     Oph & J163026.73$-$235908.7 & YSOc\_star$+$dust(IR2) &  1.9 &   $-$0.79 &       1600 &       0.017 &   $-$0.80 &       3200 &       0.042 & N &    G \\
 976 &     Oph & J163033.90$-$242806.2 & YSOc\_star$+$dust(IR4) &  2.5 &   $-$1.25 &       1800 &       0.041 &   $-$1.30 &       3400 &       0.12 & N &    G \\
 977 &     Oph & J163041.47$-$241320.6 & YSOc\_star$+$dust(MP1) &  9.8 &   $-$0.17 &       1600 &       0.0018 &   $-$0.78 &       2300 &       0.020 & N &    G \\
 978 &     Oph & J163053.48$-$242453.9 & YSOc\_star$+$dust(IR3) &  2.4 &   $-$1.12 &       1700 &       0.023 &   $-$1.18 &       3300 &       0.063 & N &    G \\
 979 &     Oph & J163102.39$-$240843.1 & YSOc\_star$+$dust(IR1) &  2.0 &   $-$1.49 &       1700 &       0.030 &   $-$1.64 &       3300 &       0.078 & N &    G \\
 980 &     Oph & J163105.15$-$240440.2 & YSOc\_star$+$dust(IR3) &  3.8 &   $-$1.23 &       1600 &       0.22 &   $-$1.33 &       3300 &       0.70 & N &    G \\
 981 &     Oph & J163115.73$-$243402.0 & YSOc\_star$+$dust(IR4) &  2.3 &   $-$1.05 &       1700 &       0.85 &   $-$1.05 &       3300 &       2.3 & N &    G \\
 982 &     Oph & J163129.23$-$240431.1 &                YSOc &  9.8 &   $-$0.16 &        770 &       0.024 &   $-$0.27 &       1100 &       0.100 & N &    G \\
 983 &     Oph & J163130.87$-$242439.5 &                YSOc & 11.3 &   $-$0.57 &        980 &       0.60 &   $-$0.92 &       3000 &       2.9 & N &    G \\
 984 &     Oph & J163131.24$-$242627.9 & YSOc\_star$+$dust(IR4) &  1.8 &   $-$0.38 &        750 &       0.014 &   $-$0.24 &       2100 &       0.022 & N &    G \\
 985 &     Oph & J163133.44$-$242737.1 & YSOc\_star$+$dust(IR1) &  4.4 &   $-$0.61 &       1200 &       0.76 &   $-$0.68 &       2900 &       2.1 & N &    G \\
 986 &     Oph & J163133.82$-$240446.5 & YSOc\_star$+$dust(IR2) &  9.8 &    0.13 &        730 &       0.12 &   $-$0.60 &       1400 &       0.59 & N &    G \\
 987 &     Oph & J163134.08$-$240059.7 &                YSOc & 20.4 &   $-$0.32 &        860 &       0.0033 &   $-$1.56 &       2600 &       0.026 & N &    G \\
 988 &     Oph & J163134.29$-$240325.2 &                YSOc &  9.8 &   $-$0.08 &        700 &       0.25 &   $-$0.12 &        870 &       0.88 & N &    G \\
 989 &     Oph & J163135.65$-$240129.3 &                YSOc &  9.8 &    0.14 &        300 &       1.4 &    0.09 &        530 &       3.3 & Y &    G \\
 990 &     Oph & J163136.77$-$240419.8 & YSOc\_star$+$dust(MP1) &  9.8 &   $-$0.27 &         77 &       0.18 &   $-$0.33 &        300 &       0.24 & Y &    G \\
 991 &     Oph & J163143.75$-$245524.6 &                YSOc &  9.8 &    0.23 &        500 &       0.28 &    0.13 &        720 &       0.93 & Y &    G \\
 992 &     Oph & J163144.57$-$240213.0 & YSOc\_star$+$dust(IR3) & 14.1 &   $-$0.54 &        930 &       0.11 &   $-$0.94 &       3100 &       0.72 & N &    G \\
 993 &     Oph & J163145.39$-$244307.2 & YSOc\_star$+$dust(IR3) &  5.0 &   $-$1.33 &       1600 &       0.054 &   $-$1.44 &       3300 &       0.20 & N &    G \\
 994 &     Oph & J163145.81$-$243909.0 & YSOc\_star$+$dust(IR2) &  6.7 &   $-$0.86 &       1400 &       0.024 &   $-$1.05 &       3200 &       0.099 & N &    G \\
 995 &     Oph & J163148.93$-$245429.5 &                YSOc & 17.8 &   $-$0.78 &        990 &       0.012 &   $-$1.28 &       3100 &       0.100 & N &    G \\
 996 &     Oph & J163152.06$-$245726.0 &            YSOc\_red &  9.8 &    0.82 & $\leq$120 & $\geq$0.0093 &    0.82 & $\leq$190 & $\geq$0.018 & Y &  L\_I \\
 997 &     Oph & J163152.11$-$245615.8 &                YSOc &  9.8 &   $-$0.17 &        720 &       1.2 &   $-$0.56 &       1100 &       4.9 & N &    G \\
 998 &     Oph & J163152.45$-$245536.2 &            YSOc\_red &  9.8 &    1.07 &        240 &       0.13 &    0.82 &        340 &       0.33 & Y &    G \\
 999 &     Oph & J163153.44$-$245505.2 &                YSOc & 23.8 &   $-$0.36 &        800 &       0.041 &   $-$1.09 &       2900 &       0.41 & N &    G \\
1000 &     Oph & J163154.42$-$250349.3 & YSOc\_star$+$dust(IR3) &  5.8 &   $-$1.19 &       1500 &       0.062 &   $-$1.38 &       3300 &       0.25 & N &    G \\
1001 &     Oph & J163154.73$-$250324.0 & YSOc\_star$+$dust(IR3) &  8.5 &   $-$0.63 &       1200 &       0.55 &   $-$0.80 &       3100 &       2.5 & N &    G \\
1002 &     Oph & J163159.33$-$245440.7 & YSOc\_star$+$dust(IR2) &  4.2 &   $-$0.92 &       1500 &       0.037 &   $-$1.05 &       3200 &       0.12 & N &    G \\
1003 &     Oph & J163200.99$-$245642.6 &              rising &  9.8 &    1.39 &        130 &       4.0 &    1.54 &        220 &       7.7 & Y &    G \\
1004 &     Oph & J163205.53$-$250236.3 & YSOc\_star$+$dust(IR4) &  4.8 &   $-$1.08 &       1600 &       0.059 &   $-$1.04 &       3300 &       0.22 & N &    G \\
1005 &     Oph & J163211.81$-$244021.5 & YSOc\_star$+$dust(IR4) &  2.8 &   $-$1.66 &       1800 &       0.37 &   $-$1.68 &       3400 &       1.1 & N &    G \\
1006 &     Oph & J163221.04$-$243035.8 & YSOc\_star$+$dust(IR1) & 15.5 &   $-$0.39 &        790 &       0.41 &   $-$0.77 &       2900 &       2.4 & N &    G \\
1007 &     Oph & J163221.92$-$244214.8 & YSOc\_star$+$dust(IR2) &  2.8 &   $-$0.85 &       1500 &       0.15 &   $-$0.92 &       3100 &       0.40 & N &    G \\
1008 &     Oph & J163222.63$-$242831.8 &                 red &  9.8 &    5.03 &         47 &       16 &    4.89 &         48 &       19 & Y &    G \\
1009 &     Oph & J163227.10$-$244843.2 & YSOc\_star$+$dust(IR4) &  7.3 &   $-$2.31 &       1800 &       1.7 &   $-$2.60 &       3500 &       9.6 & N &    G \\
1010 &     Oph & J163227.87$-$252501.8 & YSOc\_star$+$dust(IR2) &  1.9 &   $-$0.94 &       1600 &       0.013 &   $-$0.99 &       3200 &       0.033 & N &    G \\
1011 &     Oph & J163301.55$-$240355.5 &                YSOc & 14.6 &   $-$1.49 &       1100 &       0.062 &   $-$1.92 &       2900 &       0.38 & N &    G \\
1012 &     Oph & J163346.21$-$242752.9 & YSOc\_star$+$dust(MP1) &  8.8 &   $-$2.22 &       1700 &       0.30 &   $-$2.48 &       3400 &       1.9 & N &    G \\
1013 &     Oph & J163355.60$-$244205.0 & YSOc\_star$+$dust(MP1) &  4.6 &   $-$1.22 &       1500 &       0.17 &   $-$1.07 &       3300 &       0.61 & N &    G \\
1014 &     Oph & J163519.46$-$241540.3 & YSOc\_star$+$dust(IR2) &  6.9 &   $-$0.63 &       1300 &       0.14 &   $-$0.96 &       3000 &       0.52 & N &    G \\
1015 &     Oph & J163603.94$-$242344.3 & YSOc\_star$+$dust(MP1) &  5.8 &   $-$2.14 &       1800 &       0.13 &   $-$2.31 &       3400 &       0.61 & N &    G \\
1016 &     Oph & J163744.22$-$242805.2 & YSOc\_star$+$dust(MP1) &  9.2 &   $-$2.20 &       1700 &       0.54 &   $-$2.46 &       3400 &       3.7 & N &    G \\
1017 &     Oph & J163759.94$-$242146.6 & YSOc\_star$+$dust(MP1) &  8.6 &   $-$2.14 &       1700 &       0.25 &   $-$2.39 &       3400 &       1.6 & N &    G \\
1018 &     Oph & J163945.43$-$240203.9 & YSOc\_star$+$dust(IR1) &  9.3 &   $-$0.73 &       1100 &       0.77 &   $-$0.93 &       2900 &       3.2 & N &    G \\
1019 &     Oph & J163952.91$-$241931.4 & YSOc\_star$+$dust(IR1) &  9.8 &   $-$0.28 &        950 &       0.0011 &   $-$0.45 &       1600 &       0.0064 & N &    G \\
1020 &     Oph & J164424.27$-$240124.6 &         YSOc\_PAH$-$em &  9.8 &    0.76 &        260 &       0.019 &    0.27 &        810 &       0.049 & N &    G \\
1021 &     Oph & J164428.83$-$241224.0 & YSOc\_star$+$dust(MP1) &  0.0 &   $-$2.31 & $\geq$2000 & $\geq$0.45 &   $-$2.31 & $\geq$2000 & $\geq$0.45 & N & L\_II \\
1022 &     Oph & J164429.32$-$241555.5 & YSOc\_star$+$dust(MP1) &  6.2 &   $-$1.99 &       1700 &       0.52 &   $-$2.14 &       3500 &       2.5 & N &    G \\
1023 &     Oph & J164526.65$-$240305.4 &            YSOc\_red &  9.8 &    0.50 &        500 &       0.0028 &    0.37 &       1000 &       0.012 & N &    G \\
1024 &     Oph & J164535.46$-$241422.4 & YSOc\_star$+$dust(IR2) &  4.7 &   $-$1.48 &       1800 &       0.23 &   $-$1.62 &       3500 &       0.93 & N &    G \\
\enddata \\
\tablenotetext{a}{Value of A$_{\rm V}$ used for dereddening, as explained in the text.}
\tablenotetext{b}{Indicates whether or not the source is associated with an envelope as traced by extended millimeter emission (based primarily on the sample of Enoch et al. [2008]).}
\tablenotetext{c}{Indicates the quality of the calculated \lbol\ and \tbol\ values.\\
``G'': existing photometry provides sufficient spectral coverage for reliable calculations.  Other flags mark sources without sufficient coverage:\\
``L\_I'': the source is associated with an envelope and thus likely an embedded source, but lacks spectral coverage between 24 \um\ and 1 mm.  The calculated values of \lbol\ and \tbol\ are thus considered lower and upper limits, respectively.\\
``L\_II'': the source is not associated with an envelope and has an observed $\alpha \leq$ $-$0.3, thus is not likely an embedded source, but no extinction correction could be derived based on available data, usually because of a lack of sufficient coverage in the near-infrared.  The calculated values of \lbol\ and \tbol\ are thus considered lower limits.\\
``O'':  Other.  These three sources were added to the list of YSOs based on the searches for embedded protostars presented by J{\o}rgensen et al. (2007) (for Perseus) and J{\o}rgensen et al. (2008) (for Ophiuchus), but they are not associated with envelopes according to Enoch et al. (2008).  They are only detected at one wavelength (24 \um), thus calculations of $\alpha$, \tbol, and \lbol\ are not possible.  They are counted as Class I objects when classifying by $\alpha$ and $\alpha^{\prime}$; they are not counted at all when classifying by \tbol\ and \tbol$^{\prime}$.}
\end{deluxetable}
\end{landscape}


==> tab9.tex <==
\begin{landscape}
\begin{deluxetable}{rcccccccc}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\tablecaption{\label{tabysolist2}$0.36-0.96$ \um\ Flux Densities, in mJy, of YSOs in the c2d Clouds}
\tablehead{
                & \colhead{\emph{U}} & \colhead{\emph{B}} & \colhead{\emph{V}} & \colhead{\emph{R}}    & \colhead{H$\alpha$12}    & \colhead{\emph{I}}    & \colhead{\emph{m}914}    & \colhead{\emph{z}}  \\
\colhead{Index} & \colhead{0.36 \um} & \colhead{0.44 \um} & \colhead{0.55 \um}       & \colhead{0.64 \um} & \colhead{0.665 \um} & \colhead{0.79 \um} & \colhead{0.915 \um} & \colhead{0.96 \um}}
\startdata
   1 &             ... &      0.48 $\pm$     0.12 &       4.2 $\pm$      1.0 &       12 $\pm$      2.8 &       16 $\pm$      1.9 &      510 $\pm$      19 &             ... &             ... \\
   2 &             ... &      0.16 $\pm$    0.040 &      0.65 $\pm$     0.16 &       3.6 $\pm$    0.030 &       2.4 $\pm$     0.29 &       33 $\pm$     0.60 &       90 $\pm$      6.6 &       49 $\pm$      2.3 \\
   3 &             ... &   0.00100 $\pm$   0.0020 &      0.14 $\pm$   0.0040 &      0.83 $\pm$  0.00100 &      0.78 $\pm$    0.100 &       6.7 $\pm$    0.060 &       17 $\pm$      1.2 &       19 $\pm$     0.36 \\
   4 &             ... &             ... &             ... &   0.00100 $\pm$  0.00100 &   0.00100 $\pm$  0.00100 &     0.040 $\pm$   0.0020 &     0.090 $\pm$  0.00100 &      0.11 $\pm$  0.00100 \\
   5 &             ... &      0.40 $\pm$  0.00100 &       1.3 $\pm$    0.040 &       4.4 $\pm$    0.040 &       4.0 $\pm$     0.48 &       14 $\pm$     0.12 &       22 $\pm$      1.6 &       22 $\pm$     0.20 \\
   6 &       2.8 $\pm$     0.18 &       5.3 $\pm$     0.15 &       7.5 $\pm$     0.21 &       8.8 $\pm$      1.2 &       1.0 $\pm$      1.2 &       11 $\pm$    0.100 &       11 $\pm$     0.81 &       11 $\pm$    0.100 \\
   7 &             ... &      0.95 $\pm$     0.23 &       8.2 $\pm$      2.0 &       11 $\pm$    0.100 &       14 $\pm$      1.6 &       35 $\pm$     0.64 &       59 $\pm$      4.3 &       63 $\pm$      1.2 \\
   8 &             ... &             ... &             ... &    0.0030 $\pm$  0.00100 &             ... &     0.040 $\pm$   0.0020 &      0.18 $\pm$    0.020 &      0.18 $\pm$  0.00100 \\
   9 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  10 &             ... &      0.21 $\pm$    0.050 &             ... &       27 $\pm$      6.4 &       37 $\pm$      4.4 &      270 $\pm$      7.5 &             ... &             ... \\
  11 &             ... &      0.41 $\pm$  0.00100 &       1.6 $\pm$    0.040 &       5.3 $\pm$    0.050 &       5.4 $\pm$     0.65 &       25 $\pm$     0.23 &       41 $\pm$      3.0 &       43 $\pm$     0.78 \\
  12 &             ... &             ... &             ... &      0.11 $\pm$  0.00100 &     0.090 $\pm$  0.00100 &      0.86 $\pm$  0.00100 &       1.9 $\pm$     0.24 &       1.7 $\pm$    0.020 \\
  13 &      0.65 $\pm$  0.00100 &       3.3 $\pm$    0.090 &       6.3 $\pm$     0.17 &       13 $\pm$     0.23 &       19 $\pm$      2.3 &       28 $\pm$     0.26 &       46 $\pm$      3.4 &       49 $\pm$     0.91 \\
  14 &             ... &     0.030 $\pm$  0.00100 &             ... &      0.24 $\pm$   0.0020 &      0.22 $\pm$    0.040 &       1.6 $\pm$  0.00100 &       4.1 $\pm$     0.30 &       4.0 $\pm$    0.040 \\
  15 &             ... &     0.030 $\pm$   0.0020 &      0.15 $\pm$   0.0040 &      0.54 $\pm$   0.0050 &      0.49 $\pm$    0.060 &       2.6 $\pm$    0.020 &       6.5 $\pm$     0.48 &       5.8 $\pm$    0.050 \\
  16 &             ... &       1.8 $\pm$     0.43 &       14 $\pm$      3.4 &       15 $\pm$     0.81 &       18 $\pm$      2.3 &       41 $\pm$      1.5 &       60 $\pm$      4.4 &       65 $\pm$      1.2 \\
  17 &             ... &      0.21 $\pm$    0.050 &      0.73 $\pm$     0.18 &       1.1 $\pm$  0.00100 &      0.96 $\pm$     0.12 &       5.3 $\pm$    0.050 &       9.5 $\pm$     0.79 &       12 $\pm$     0.11 \\
  18 &             ... &      0.34 $\pm$  0.00100 &      0.91 $\pm$    0.030 &       1.8 $\pm$    0.030 &       1.9 $\pm$     0.31 &       7.1 $\pm$    0.070 &       6.2 $\pm$     0.46 &       14 $\pm$     0.13 \\
  19 &       2.0 $\pm$    0.020 &       13 $\pm$     0.36 &       38 $\pm$      1.1 &       72 $\pm$      1.3 &       10 $\pm$      12 &      140 $\pm$      1.3 &      150 $\pm$      20 &      170 $\pm$      67 \\
  20 &             ... &     0.040 $\pm$  0.00100 &      0.32 $\pm$    0.080 &      0.27 $\pm$   0.0020 &      0.30 $\pm$    0.030 &      0.58 $\pm$    0.041 &      0.68 $\pm$    0.060 &      0.80 $\pm$  0.00100 \\
  21 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  22 &             ... &             ... &             ... &      0.11 $\pm$  0.00100 &      0.11 $\pm$    0.020 &      0.90 $\pm$  0.00100 &       2.2 $\pm$     0.16 &       2.6 $\pm$      1.0 \\
  23 &             ... &      0.21 $\pm$    0.050 &      0.80 $\pm$     0.19 &       1.1 $\pm$  0.00100 &       1.3 $\pm$     0.16 &       4.7 $\pm$    0.040 &       8.5 $\pm$     0.63 &       9.9 $\pm$      4.2 \\
  24 &      0.32 $\pm$   0.0030 &      0.91 $\pm$    0.030 &       3.5 $\pm$    0.100 &       10 $\pm$     0.19 &       17 $\pm$      2.1 &       28 $\pm$     0.26 &       53 $\pm$      3.9 &       66 $\pm$      26 \\
  25 &             ... &     0.020 $\pm$   0.0040 &             ... &     0.080 $\pm$  0.00100 &     0.050 $\pm$  0.00100 &      0.62 $\pm$  0.00100 &       1.5 $\pm$     0.11 &       1.7 $\pm$     0.70 \\
  26 &      0.31 $\pm$   0.0030 &      0.74 $\pm$    0.020 &       2.4 $\pm$    0.070 &             ... &             ... &       24 $\pm$     0.22 &             ... &       56 $\pm$      22 \\
  27 &             ... &      0.33 $\pm$    0.033 &       1.0 $\pm$    0.100 &       6.2 $\pm$     0.62 &             ... &       47 $\pm$      4.7 &             ... &      110 $\pm$      11 \\
  28 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  29 &             ... &       24 $\pm$      2.4 &       53 $\pm$      5.3 &       90 $\pm$      9.0 &             ... &      130 $\pm$      13 &             ... &      170 $\pm$      17 \\
  30 &             ... &             ... &             ... &       4.8 $\pm$     0.48 &             ... &       24 $\pm$      2.4 &             ... &       57 $\pm$      5.7 \\
  31 &             ... &             ... &             ... &             ... &             ... &     0.047 $\pm$   0.0047 &             ... &      0.11 $\pm$    0.011 \\
  32 &             ... &     0.052 $\pm$   0.0052 &             ... &      0.17 $\pm$    0.017 &             ... &       3.6 $\pm$     0.36 &             ... &       14 $\pm$      1.4 \\
  33 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  34 &             ... &      0.13 $\pm$    0.013 &             ... &      0.14 $\pm$    0.014 &             ... &             ... &             ... &             ... \\
  35 &             ... &      0.18 $\pm$    0.018 &      0.30 $\pm$    0.030 &      0.37 $\pm$    0.037 &             ... &       2.0 $\pm$     0.20 &             ... &             ... \\
  36 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  37 &             ... &             ... &             ... &     0.099 $\pm$   0.0099 &             ... &             ... &             ... &             ... \\
  38 &             ... &      0.45 $\pm$    0.045 &       1.2 $\pm$     0.12 &             ... &             ... &             ... &             ... &             ... \\
  39 &             ... &      0.27 $\pm$    0.027 &             ... &      0.35 $\pm$    0.035 &             ... &             ... &             ... &             ... \\
  40 &             ... &             ... &             ... &     0.094 $\pm$   0.0094 &             ... &      0.49 $\pm$    0.049 &             ... &      0.90 $\pm$    0.090 \\
  41 &             ... &             ... &             ... &     0.100 $\pm$    0.010 &             ... &      0.18 $\pm$    0.018 &             ... &      0.40 $\pm$    0.040 \\
  42 &             ... &       3.2 $\pm$     0.32 &       13 $\pm$      1.3 &       10 $\pm$      1.0 &             ... &       26 $\pm$      2.6 &             ... &       50 $\pm$      5.0 \\
  43 &             ... &       1.3 $\pm$     0.13 &       5.6 $\pm$     0.56 &       7.0 $\pm$     0.70 &             ... &       17 $\pm$      1.7 &             ... &       29 $\pm$      2.9 \\
  44 &             ... &      0.18 $\pm$    0.018 &             ... &      0.44 $\pm$    0.044 &             ... &       1.4 $\pm$     0.14 &             ... &       3.1 $\pm$     0.31 \\
  45 &             ... &       1.1 $\pm$     0.11 &       5.6 $\pm$     0.56 &       6.1 $\pm$     0.61 &             ... &       21 $\pm$      2.1 &             ... &       31 $\pm$      3.1 \\
  46 &             ... &      0.57 $\pm$    0.057 &       2.8 $\pm$     0.28 &       4.5 $\pm$     0.45 &             ... &       32 $\pm$      3.2 &             ... &       96 $\pm$      9.6 \\
  47 &             ... &             ... &             ... &    0.0053 $\pm$  0.00053 &             ... &     0.027 $\pm$   0.0027 &             ... &     0.082 $\pm$   0.0082 \\
  48 &             ... &             ... &             ... &     0.054 $\pm$   0.0054 &             ... &       1.3 $\pm$     0.13 &             ... &       9.5 $\pm$     0.95 \\
  49 &             ... &      0.69 $\pm$    0.069 &      0.59 $\pm$    0.059 &      0.63 $\pm$    0.063 &             ... &       4.8 $\pm$     0.48 &             ... &       11 $\pm$      1.1 \\
  50 &             ... &       2.0 $\pm$     0.20 &       15 $\pm$      1.5 &       8.6 $\pm$     0.86 &             ... &       40 $\pm$      4.0 &             ... &      100 $\pm$      10 \\
  51 &             ... &             ... &             ... &      0.19 $\pm$    0.019 &             ... &       8.0 $\pm$     0.80 &             ... &       26 $\pm$      2.6 \\
  52 &             ... &       5.0 $\pm$     0.50 &       16 $\pm$      1.6 &       10 $\pm$      1.0 &             ... &       47 $\pm$      4.7 &             ... &       31 $\pm$      3.1 \\
  53 &             ... &             ... &             ... &     0.083 $\pm$   0.0083 &             ... &      0.27 $\pm$    0.027 &             ... &      0.53 $\pm$    0.053 \\
  54 &             ... &       1.4 $\pm$     0.14 &       5.4 $\pm$     0.54 &       4.2 $\pm$     0.42 &             ... &       17 $\pm$      1.7 &             ... &       29 $\pm$      2.9 \\
  55 &             ... &       4.2 $\pm$     0.42 &       13 $\pm$      1.3 &       64 $\pm$      6.4 &             ... &       84 $\pm$      8.4 &             ... &      130 $\pm$      13 \\
  56 &             ... &       2.6 $\pm$     0.26 &       1.5 $\pm$     0.15 &       2.2 $\pm$     0.22 &             ... &       5.5 $\pm$     0.55 &             ... &       11 $\pm$      1.1 \\
  57 &             ... &      0.93 $\pm$    0.093 &       2.5 $\pm$     0.25 &       3.2 $\pm$     0.32 &             ... &       14 $\pm$      1.4 &             ... &       31 $\pm$      3.1 \\
  58 &             ... &             ... &             ... &       7.7 $\pm$     0.77 &             ... &       29 $\pm$      2.9 &             ... &       57 $\pm$      5.7 \\
  59 &             ... &       1.3 $\pm$     0.13 &       1.6 $\pm$     0.16 &       2.2 $\pm$     0.22 &             ... &       1.4 $\pm$     0.14 &             ... &       1.5 $\pm$     0.14 \\
  60 &             ... &             ... &             ... &       2.6 $\pm$     0.26 &             ... &       14 $\pm$      1.4 &             ... &       25 $\pm$      2.5 \\
  61 &             ... &             ... &       3.0 $\pm$     0.30 &       8.0 $\pm$     0.80 &             ... &       9.5 $\pm$     0.95 &             ... &       18 $\pm$      1.8 \\
  62 &             ... &             ... &             ... &       3.1 $\pm$     0.31 &             ... &       3.5 $\pm$     0.35 &             ... &       5.1 $\pm$     0.51 \\
  63 &             ... &      0.49 $\pm$    0.049 &       1.4 $\pm$     0.14 &       2.1 $\pm$     0.21 &             ... &       13 $\pm$      1.3 &             ... &       27 $\pm$      2.7 \\
  64 &             ... &             ... &             ... &      0.25 $\pm$    0.025 &             ... &       4.5 $\pm$     0.45 &             ... &       13 $\pm$      1.3 \\
  65 &             ... &      0.82 $\pm$    0.082 &             ... &       1.4 $\pm$     0.14 &             ... &       5.1 $\pm$     0.51 &             ... &       12 $\pm$      1.2 \\
  66 &             ... &             ... &             ... &     0.080 $\pm$   0.0080 &             ... &      0.14 $\pm$    0.014 &             ... &      0.18 $\pm$    0.018 \\
  67 &             ... &       3.2 $\pm$     0.32 &       5.6 $\pm$     0.56 &       10 $\pm$      1.0 &             ... &       31 $\pm$      3.1 &             ... &       38 $\pm$      3.8 \\
  68 &             ... &      0.40 $\pm$    0.040 &       1.1 $\pm$     0.11 &       2.2 $\pm$     0.22 &             ... &       1.0 $\pm$    0.100 &             ... &       18 $\pm$      1.8 \\
  69 &             ... &             ... &             ... &    0.0063 $\pm$  0.00063 &             ... &     0.080 $\pm$   0.0080 &             ... &      0.29 $\pm$    0.029 \\
  70 &             ... &      0.47 $\pm$    0.047 &             ... &      0.39 $\pm$    0.039 &             ... &       2.0 $\pm$     0.20 &             ... &       4.4 $\pm$     0.44 \\
  71 &             ... &      0.93 $\pm$    0.093 &       2.6 $\pm$     0.26 &       3.8 $\pm$     0.38 &             ... &       17 $\pm$      1.7 &             ... &       33 $\pm$      3.3 \\
  72 &             ... &      0.43 $\pm$    0.043 &      0.95 $\pm$    0.095 &      0.68 $\pm$    0.068 &             ... &       3.5 $\pm$     0.35 &             ... &       7.7 $\pm$     0.77 \\
  73 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  74 &             ... &             ... &             ... &     0.061 $\pm$   0.0061 &             ... &      0.44 $\pm$    0.044 &             ... &       1.4 $\pm$     0.14 \\
  75 &             ... &      0.70 $\pm$    0.070 &       2.8 $\pm$     0.28 &       3.0 $\pm$     0.30 &             ... &       10 $\pm$      1.0 &             ... &       12 $\pm$      1.2 \\
  76 &             ... &       3.0 $\pm$     0.30 &       8.5 $\pm$     0.85 &       5.6 $\pm$     0.56 &             ... &       25 $\pm$      2.5 &             ... &       54 $\pm$      5.4 \\
  77 &             ... &      0.73 $\pm$    0.073 &       2.4 $\pm$     0.24 &       2.8 $\pm$     0.28 &             ... &       14 $\pm$      1.4 &             ... &       25 $\pm$      2.5 \\
  78 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
  79 &             ... &      0.19 $\pm$    0.019 &       1.0 $\pm$    0.100 &       2.1 $\pm$     0.21 &             ... &       32 $\pm$      3.2 &             ... &      130 $\pm$      13 \\
  80 &             ... &       1.9 $\pm$     0.19 &       5.5 $\pm$     0.55 &       6.4 $\pm$     0.64 &             ... &       28 $\pm$      2.8 &             ... &       35 $\pm$      3.5 \\
  81 &             ... &      0.19 $\pm$    0.019 &      0.66 $\pm$    0.066 &      0.70 $\pm$    0.070 &             ... &       2.5 $\pm$     0.25 &             ... &       17 $\pm$      1.7 \\
  82 &             ... &      0.47 $\pm$    0.047 &             ... &      0.78 $\pm$    0.078 &             ... &       2.0 $\pm$     0.20 &             ... &       4.6 $\pm$     0.46 \\
  83 &             ... &             ... &             ... &      0.33 $\pm$    0.033 &             ... &       9.7 $\pm$     0.97 &             ... &       77 $\pm$      7.7 \\
  84 &             ... &      0.18 $\pm$    0.018 &      0.41 $\pm$    0.041 &      0.21 $\pm$    0.021 &             ... &       2.0 $\pm$     0.20 &             ... &       6.0 $\pm$     0.60 \\
  85 &             ... &             ... &             ... &     0.067 $\pm$   0.0067 &             ... &      0.27 $\pm$    0.027 &             ... &      0.44 $\pm$    0.044 \\
  86 &             ... &      0.19 $\pm$    0.019 &      0.84 $\pm$    0.084 &      0.66 $\pm$    0.066 &             ... &       3.4 $\pm$     0.34 &             ... &       7.1 $\pm$     0.71 \\
  87 &             ... &      0.46 $\pm$    0.046 &             ... &      0.61 $\pm$    0.061 &             ... &       1.5 $\pm$     0.15 &             ... &       3.5 $\pm$     0.35 \\
  88 &             ... &             ... &             ... &    0.0063 $\pm$  0.00063 &             ... &     0.050 $\pm$   0.0050 &             ... &      0.12 $\pm$    0.012 \\
  89 &             ... &      0.41 $\pm$    0.041 &       1.1 $\pm$     0.11 &       1.5 $\pm$     0.15 &             ... &       7.0 $\pm$     0.70 &             ... &       11 $\pm$      1.1 \\
  90 &             ... &      0.18 $\pm$    0.018 &      0.52 $\pm$    0.052 &       2.9 $\pm$     0.29 &             ... &       53 $\pm$      5.3 &             ... &      180 $\pm$      18 \\
  91 &             ... &      0.42 $\pm$    0.042 &       1.9 $\pm$     0.19 &       5.5 $\pm$     0.55 &             ... &       56 $\pm$      5.6 &             ... &      160 $\pm$      16 \\
  92 &             ... &      0.22 $\pm$    0.022 &             ... &      0.40 $\pm$    0.040 &             ... &       6.6 $\pm$     0.66 &             ... &       25 $\pm$      2.5 \\
  93 &             ... &      0.41 $\pm$    0.041 &             ... &      0.43 $\pm$    0.043 &             ... &      0.97 $\pm$    0.097 &             ... &       1.3 $\pm$     0.13 \\
  94 &             ... &       1.8 $\pm$     0.18 &       6.1 $\pm$     0.61 &       5.2 $\pm$     0.52 &             ... &       16 $\pm$      1.6 &             ... &       26 $\pm$      2.6 \\
  95 &             ... &      0.35 $\pm$    0.035 &       2.3 $\pm$     0.23 &       8.0 $\pm$     0.80 &             ... &             ... &             ... &             ... \\
  96 &             ... &      0.22 $\pm$    0.022 &      0.37 $\pm$    0.037 &       1.1 $\pm$     0.11 &             ... &       27 $\pm$      2.7 &             ... &       65 $\pm$      6.5 \\
  97 &             ... &      0.13 $\pm$    0.013 &             ... &       1.3 $\pm$     0.13 &             ... &       3.8 $\pm$     0.38 &             ... &       6.8 $\pm$     0.68 \\
  98 &             ... &      0.42 $\pm$    0.042 &             ... &      0.44 $\pm$    0.044 &             ... &       3.3 $\pm$     0.33 &             ... &       7.2 $\pm$     0.72 \\
  99 &             ... &      0.63 $\pm$    0.063 &       2.1 $\pm$     0.21 &       1.6 $\pm$     0.16 &             ... &       2.6 $\pm$     0.26 &             ... &       3.0 $\pm$     0.30 \\
 100 &             ... &      0.22 $\pm$    0.022 &      0.91 $\pm$    0.091 &      0.98 $\pm$    0.098 &             ... &       5.0 $\pm$     0.50 &             ... &       9.5 $\pm$     0.95 \\
 101 &             ... &      0.20 $\pm$    0.020 &       1.7 $\pm$     0.17 &       3.3 $\pm$     0.33 &             ... &       70 $\pm$      7.0 &             ... &      120 $\pm$      12 \\
 102 &             ... &             ... &             ... &     0.066 $\pm$   0.0066 &             ... &     0.086 $\pm$   0.0086 &             ... &      0.21 $\pm$    0.021 \\
 103 &             ... &      0.25 $\pm$    0.025 &             ... &      0.39 $\pm$    0.039 &             ... &       3.2 $\pm$     0.32 &             ... &       5.8 $\pm$     0.58 \\
 104 &             ... &      0.52 $\pm$    0.052 &       2.2 $\pm$     0.22 &       4.7 $\pm$     0.47 &             ... &       48 $\pm$      4.8 &             ... &      130 $\pm$      13 \\
 105 &             ... &       4.1 $\pm$     0.41 &       16 $\pm$      1.6 &       14 $\pm$      1.4 &             ... &       58 $\pm$      5.8 &             ... &       53 $\pm$      5.3 \\
 106 &             ... &      0.53 $\pm$    0.053 &       2.5 $\pm$     0.25 &       7.3 $\pm$     0.73 &             ... &             ... &             ... &             ... \\
 107 &             ... &      0.42 $\pm$    0.042 &       2.5 $\pm$     0.25 &       6.3 $\pm$     0.63 &             ... &      100 $\pm$      10 &             ... &      180 $\pm$      18 \\
 108 &             ... &       1.4 $\pm$     0.14 &       13 $\pm$      1.3 &       16 $\pm$      1.6 &             ... &             ... &             ... &             ... \\
 109 &             ... &      0.20 $\pm$    0.020 &       6.5 $\pm$     0.65 &       13 $\pm$      1.3 &             ... &       61 $\pm$      6.1 &             ... &      100 $\pm$      10 \\
 110 &             ... &             ... &             ... &      0.93 $\pm$    0.093 &             ... &             ... &             ... &             ... \\
 111 &             ... &      0.97 $\pm$    0.097 &      0.99 $\pm$    0.099 &       1.6 $\pm$     0.16 &             ... &       7.7 $\pm$     0.77 &             ... &       15 $\pm$      1.5 \\
 112 &             ... &       1.9 $\pm$     0.19 &       4.9 $\pm$     0.49 &       12 $\pm$      1.2 &             ... &       26 $\pm$      2.6 &             ... &       33 $\pm$      3.3 \\
 113 &             ... &       36 $\pm$      3.6 &       51 $\pm$      5.1 &      120 $\pm$      12 &             ... &             ... &             ... &             ... \\
 114 &             ... &      0.18 $\pm$    0.018 &      0.82 $\pm$    0.082 &       2.0 $\pm$     0.20 &             ... &       16 $\pm$      1.6 &             ... &       32 $\pm$      3.2 \\
 115 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 116 &             ... &      0.21 $\pm$    0.021 &      0.97 $\pm$    0.097 &       1.7 $\pm$     0.17 &             ... &       12 $\pm$      1.2 &             ... &       23 $\pm$      2.3 \\
 117 &             ... &      0.26 $\pm$    0.026 &       1.2 $\pm$     0.12 &       2.6 $\pm$     0.26 &             ... &       27 $\pm$      2.7 &             ... &       55 $\pm$      5.5 \\
 118 &             ... &      0.26 $\pm$    0.026 &       1.4 $\pm$     0.14 &       6.2 $\pm$     0.62 &             ... &       92 $\pm$      9.2 &             ... &      270 $\pm$      27 \\
 119 &             ... &      0.30 $\pm$    0.030 &             ... &      0.20 $\pm$    0.020 &             ... &      0.20 $\pm$    0.020 &             ... &      0.35 $\pm$    0.035 \\
 120 &             ... &             ... &             ... &      0.26 $\pm$    0.026 &             ... &       3.4 $\pm$     0.34 &             ... &       10 $\pm$      1.0 \\
 121 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 122 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 123 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 124 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 125 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 126 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 127 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 128 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 129 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 130 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 131 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 132 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 133 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 134 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 135 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 136 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 137 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 138 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 139 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 140 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 141 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 142 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 143 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 144 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 145 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 146 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 147 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 148 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 149 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 150 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 151 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 152 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 153 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 154 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 155 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 156 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 157 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 158 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 159 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 160 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 161 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 162 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 163 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 164 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 165 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 166 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 167 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 168 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 169 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 170 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 171 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 172 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 173 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 174 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 175 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 176 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 177 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 178 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 179 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 180 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 181 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 182 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 183 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 184 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 185 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 186 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 187 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 188 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 189 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 190 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 191 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 192 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 193 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 194 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 195 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 196 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 197 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 198 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 199 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 200 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 201 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 202 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 203 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 204 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 205 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 206 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 207 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 208 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 209 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 210 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 211 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 212 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 213 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 214 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 215 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 216 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 217 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 218 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 219 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 220 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 221 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 222 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 223 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 224 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 225 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 226 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 227 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 228 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 229 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 230 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 231 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 232 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 233 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 234 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 235 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 236 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 237 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 238 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 239 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 240 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 241 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 242 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 243 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 244 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 245 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 246 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 247 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 248 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 249 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 250 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 251 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 252 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 253 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 254 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 255 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 256 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 257 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 258 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 259 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 260 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 261 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 262 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 263 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 264 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 265 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 266 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 267 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 268 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 269 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 270 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 271 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 272 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 273 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 274 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 275 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 276 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 277 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 278 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 279 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 280 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 281 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 282 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 283 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 284 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 285 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 286 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 287 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 288 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 289 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 290 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 291 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 292 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 293 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 294 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 295 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 296 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 297 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 298 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 299 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 300 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 301 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 302 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 303 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 304 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 305 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 306 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 307 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 308 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 309 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 310 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 311 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 312 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 313 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 314 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 315 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 316 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 317 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 318 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 319 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 320 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 321 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 322 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 323 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 324 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 325 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 326 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 327 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 328 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 329 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 330 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 331 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 332 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 333 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 334 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 335 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 336 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 337 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 338 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 339 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 340 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 341 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 342 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 343 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 344 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 345 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 346 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 347 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 348 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 349 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 350 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 351 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 352 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 353 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 354 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 355 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 356 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 357 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 358 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 359 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 360 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 361 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 362 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 363 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 364 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 365 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 366 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 367 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 368 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 369 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 370 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 371 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 372 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 373 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 374 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 375 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 376 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 377 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 378 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 379 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 380 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 381 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 382 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 383 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 384 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 385 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 386 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 387 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 388 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 389 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 390 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 391 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 392 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 393 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 394 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 395 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 396 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 397 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 398 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 399 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 400 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 401 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 402 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 403 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 404 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 405 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 406 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 407 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 408 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 409 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 410 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 411 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 412 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 413 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 414 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 415 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 416 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 417 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 418 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 419 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 420 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 421 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 422 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 423 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 424 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 425 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 426 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 427 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 428 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 429 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 430 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 431 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 432 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 433 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 434 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 435 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 436 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 437 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 438 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 439 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 440 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 441 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 442 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 443 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 444 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 445 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 446 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 447 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 448 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 449 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 450 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 451 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 452 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 453 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 454 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 455 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 456 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 457 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 458 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 459 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 460 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 461 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 462 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 463 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 464 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 465 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 466 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 467 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 468 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 469 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 470 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 471 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 472 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 473 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 474 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 475 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 476 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 477 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 478 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 479 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 480 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 481 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 482 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 483 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 484 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 485 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 486 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 487 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 488 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 489 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 490 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 491 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 492 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 493 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 494 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 495 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 496 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 497 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 498 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 499 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 500 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 501 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 502 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 503 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 504 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 505 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 506 &             ... &             ... &             ... &             ... &             ... &       10 $\pm$      1.0 &             ... &             ... \\
 507 &             ... &             ... &             ... &             ... &             ... &       9.7 $\pm$     0.97 &             ... &             ... \\
 508 &             ... &     0.015 $\pm$   0.0015 &             ... &     0.069 $\pm$   0.0069 &             ... &       1.6 $\pm$     0.16 &             ... &             ... \\
 509 &             ... &             ... &             ... &             ... &             ... &       17 $\pm$      1.7 &             ... &             ... \\
 510 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 511 &             ... &             ... &             ... &             ... &             ... &      0.71 $\pm$    0.071 &             ... &             ... \\
 512 &             ... &             ... &             ... &             ... &             ... &       5.5 $\pm$     0.55 &             ... &             ... \\
 513 &             ... &             ... &             ... &             ... &             ... &       3.0 $\pm$     0.30 &             ... &             ... \\
 514 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 515 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 516 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 517 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 518 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 519 &             ... &             ... &             ... &             ... &             ... &       1.5 $\pm$     0.15 &             ... &             ... \\
 520 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 521 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 522 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 523 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 524 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 525 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 526 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 527 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 528 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 529 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 530 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 531 &             ... &             ... &             ... &             ... &             ... &      0.66 $\pm$    0.066 &             ... &             ... \\
 532 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 533 &             ... &             ... &             ... &     0.098 $\pm$   0.0098 &             ... &             ... &             ... &             ... \\
 534 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 535 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 536 &             ... &             ... &             ... &             ... &             ... &      0.13 $\pm$    0.013 &             ... &             ... \\
 537 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 538 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 539 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 540 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 541 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 542 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 543 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 544 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 545 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 546 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 547 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 548 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 549 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 550 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 551 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 552 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 553 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 554 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 555 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 556 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 557 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 558 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 559 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 560 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 561 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 562 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 563 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 564 &             ... &             ... &             ... &     0.069 $\pm$   0.0069 &             ... &             ... &             ... &             ... \\
 565 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 566 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 567 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 568 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 569 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 570 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 571 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 572 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 573 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 574 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 575 &             ... &             ... &             ... &             ... &             ... &       1.9 $\pm$     0.19 &             ... &             ... \\
 576 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 577 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 578 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 579 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 580 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 581 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 582 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 583 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 584 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 585 &             ... &             ... &             ... &             ... &             ... &       2.2 $\pm$     0.22 &             ... &             ... \\
 586 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 587 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 588 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 589 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 590 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 591 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 592 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 593 &             ... &             ... &             ... &     0.098 $\pm$   0.0098 &             ... &             ... &             ... &             ... \\
 594 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 595 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 596 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 597 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 598 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 599 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 600 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 601 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 602 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 603 &             ... &             ... &             ... &             ... &             ... &      370 $\pm$      37 &             ... &             ... \\
 604 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 605 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 606 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 607 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 608 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 609 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 610 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 611 &             ... &             ... &             ... &     0.070 $\pm$   0.0070 &             ... &             ... &             ... &             ... \\
 612 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 613 &             ... &             ... &             ... &     0.099 $\pm$   0.0099 &             ... &             ... &             ... &             ... \\
 614 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 615 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 616 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 617 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 618 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 619 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 620 &             ... &             ... &             ... &     0.088 $\pm$   0.0088 &             ... &             ... &             ... &             ... \\
 621 &             ... &             ... &             ... &     0.075 $\pm$   0.0075 &             ... &             ... &             ... &             ... \\
 622 &             ... &             ... &             ... &     0.075 $\pm$   0.0075 &             ... &             ... &             ... &             ... \\
 623 &             ... &             ... &             ... &     0.075 $\pm$   0.0075 &             ... &             ... &             ... &             ... \\
 624 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 625 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 626 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 627 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 628 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 629 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 630 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 631 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 632 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 633 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 634 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 635 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 636 &             ... &       1.1 $\pm$     0.11 &       5.5 $\pm$     0.55 &       8.7 $\pm$     0.87 &             ... &             ... &             ... &             ... \\
 637 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 638 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 639 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 640 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 641 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 642 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 643 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 644 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 645 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 646 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 647 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 648 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 649 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 650 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 651 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 652 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 653 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 654 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 655 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 656 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 657 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 658 &             ... &             ... &             ... &      0.11 $\pm$    0.011 &             ... &             ... &             ... &             ... \\
 659 &             ... &             ... &             ... &      0.11 $\pm$    0.011 &             ... &             ... &             ... &             ... \\
 660 &             ... &             ... &             ... &      0.11 $\pm$    0.011 &             ... &             ... &             ... &             ... \\
 661 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 662 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 663 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 664 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 665 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 666 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 667 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 668 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 669 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 670 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 671 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 672 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 673 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 674 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 675 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 676 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 677 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 678 &             ... &     0.032 $\pm$   0.0032 &             ... &      0.43 $\pm$    0.043 &             ... &             ... &             ... &             ... \\
 679 &             ... &     0.032 $\pm$   0.0032 &             ... &      0.43 $\pm$    0.043 &             ... &             ... &             ... &             ... \\
 680 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 681 &             ... &     0.032 $\pm$   0.0032 &             ... &      0.43 $\pm$    0.043 &             ... &             ... &             ... &             ... \\
 682 &             ... &     0.032 $\pm$   0.0032 &             ... &      0.43 $\pm$    0.043 &             ... &             ... &             ... &             ... \\
 683 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 684 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 685 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 686 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 687 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 688 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 689 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 690 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 691 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 692 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 693 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 694 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 695 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 696 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 697 &             ... &     0.036 $\pm$   0.0036 &             ... &      0.14 $\pm$    0.014 &             ... &             ... &             ... &             ... \\
 698 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 699 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 700 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 701 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 702 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 703 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 704 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 705 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 706 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 707 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 708 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 709 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 710 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 711 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 712 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 713 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 714 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 715 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 716 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 717 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 718 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 719 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 720 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 721 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 722 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 723 &             ... &             ... &             ... &     0.076 $\pm$   0.0076 &             ... &             ... &             ... &             ... \\
 724 &             ... &             ... &             ... &     0.076 $\pm$   0.0076 &             ... &             ... &             ... &             ... \\
 725 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 726 &             ... &     0.014 $\pm$   0.0014 &             ... &     0.097 $\pm$   0.0097 &             ... &             ... &             ... &             ... \\
 727 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 728 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 729 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 730 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 731 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 732 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 733 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 734 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 735 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 736 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 737 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 738 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 739 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 740 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 741 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 742 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 743 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 744 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 745 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 746 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 747 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 748 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 749 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 750 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 751 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 752 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 753 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 754 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 755 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 756 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 757 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 758 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 759 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 760 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 761 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 762 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 763 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 764 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 765 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 766 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 767 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 768 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 769 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 770 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 771 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 772 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 773 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 774 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 775 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 776 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 777 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 778 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 779 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 780 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 781 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 782 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 783 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 784 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 785 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 786 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 787 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 788 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 789 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 790 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 791 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 792 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 793 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 794 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 795 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 796 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 797 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 798 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 799 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 800 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 801 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 802 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 803 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 804 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 805 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 806 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 807 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 808 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 809 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 810 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 811 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 812 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 813 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 814 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 815 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 816 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 817 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 818 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 819 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 820 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 821 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 822 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 823 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 824 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 825 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 826 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 827 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 828 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 829 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 830 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 831 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 832 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 833 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 834 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 835 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 836 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 837 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 838 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 839 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 840 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 841 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 842 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 843 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 844 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 845 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 846 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 847 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 848 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 849 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 850 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 851 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 852 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 853 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 854 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 855 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 856 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 857 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 858 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 859 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 860 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 861 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 862 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 863 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 864 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 865 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 866 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 867 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 868 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 869 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 870 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 871 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 872 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 873 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 874 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 875 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 876 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 877 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 878 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 879 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 880 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 881 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 882 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 883 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 884 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 885 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 886 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 887 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 888 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 889 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 890 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 891 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 892 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 893 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 894 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 895 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 896 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 897 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 898 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 899 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 900 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 901 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 902 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 903 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 904 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 905 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 906 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 907 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 908 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 909 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 910 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 911 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 912 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 913 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 914 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 915 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 916 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 917 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 918 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 919 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 920 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 921 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 922 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 923 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 924 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 925 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 926 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 927 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 928 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 929 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 930 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 931 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 932 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 933 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 934 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 935 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 936 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 937 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 938 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 939 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 940 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 941 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 942 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 943 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 944 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 945 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 946 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 947 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 948 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 949 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 950 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 951 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 952 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 953 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 954 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 955 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 956 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 957 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 958 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 959 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 960 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 961 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 962 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 963 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 964 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 965 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 966 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 967 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 968 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 969 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 970 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 971 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 972 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 973 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 974 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 975 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 976 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 977 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 978 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 979 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 980 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 981 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 982 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 983 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 984 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 985 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 986 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 987 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 988 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 989 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 990 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 991 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 992 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 993 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 994 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 995 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 996 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 997 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 998 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
 999 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1000 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1001 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1002 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1003 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1004 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1005 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1006 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1007 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1008 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1009 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1010 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1011 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1012 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1013 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1014 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1015 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1016 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1017 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1018 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1019 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1020 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1021 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1022 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1023 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
1024 &             ... &             ... &             ... &             ... &             ... &             ... &             ... &             ... \\
\enddata \\
\end{deluxetable}
\end{landscape}

